Decoupling DNS Update Timing from TTL Values

A relatively simple safety-belt mechanism for improving DNS system availability and efficiency is proposed here. While it may seem ambitious, a careful examination shows it is both feasible and beneficial for the DNS system. The mechanism called "DNS Real-time Update" (DNSRU), a service that facilitates real-time and secure updates of cached domain records in DNS resolvers worldwide, even before the expiration of the corresponding Time To Live (TTL) values. This service allows Internet domain owners to quickly rectify any erroneous global IP address distribution, even if a long TTL value is associated with it. By addressing this critical DNS high availability issue, DNSRU eliminates the need for short TTL values and their associated drawbacks. Therefore, DNSRU DNSRU reduces the traffic load on authoritative servers while enhancing the system's fault tolerance. In this paper we show that our DNSRU design is backward compatible, supports gradual deployment, secure, efficient, and feasible.

==> cwc-macs.tex <==
%\newcommand{\boaz}[1]{\hl{\textbf{BPS}: #1}}
%\newcommand{\yehuda}[1]{{\color{red}{\bfseries\{YA: #1\}}}}
%\newcommand{\gal}[1]{{\color{blue}{\bfseries\{GG: #1\}}}}
%\newcommand{\todo}[1]{{\color{violet}{\bfseries\{TODO: #1\}}}}
%\newcommand\ignore[1]{}
%
%
%\newcommand{\namedref}[2]{\hyperref[#2]{#1~\ref*{#2}}}
%\newcommand{\sectionref}[1]{\namedref{Section}{#1}}
%\newcommand{\appendixref}[1]{\namedref{Appendix}{#1}}
%\newcommand{\theoremref}[1]{\namedref{Theorem}{#1}}
%\newcommand{\defref}[1]{\namedref{Definition}{#1}}
%\newcommand{\figref}[1]{\namedref{Figure}{#1}}
%\newcommand{\lemmaref}[1]{\namedref{Lemma}{#1}}
%\newcommand{\tableref}[1]{\namedref{Table}{#1}}
%\newcommand{\corollaryref}[1]{\namedref{Corollary}{#1}}
%\newcommand{\remarkref}[1]{\namedref{Remark}{#1}}
%\newcommand{\appref}[1]{\namedref{Appendix}{#1}}
%\newcommand{\propref}[1]{\namedref{Proposition}{#1}}
%\newcommand{\algref}[1]{\namedref{Algorithm}{#1}}
%\newcommand{\lineref}[1]{\namedref{Line}{#1}}
%\newcommand{\equalityref}[1]{\hyperref[#1]{Eq.~\ref*{#1}}}
%\newcommand{\inequalityref}[1]{\hyperref[#1]{Inequality~(\ref*{#1})}}
%\newcommand{\factref}[1]{\namedref{Fact}{#1}}
%\newcommand{\stepref}[1]{\hyperref[#1]{Step~(\ref*{#1})}}
%
%\def\blackslug{\hbox{\hskip 1pt \vrule width 4pt height 8pt
%		depth 1.5pt \hskip 1pt}}
%\def\QED{\quad\blackslug\lower 8.5pt\null\par}
%\def\Qed{\QED}
%\def\inQED{~~~~~\quad\blackslug\lower 8.5pt\null}
%\def\Proof{\noindent{\bf Proof:~}}
%\def\ProofOf#1#2{\noindent{\bf Proof of #1 \ref{#2}:~}}
%\def\Prooff#1#2{\noindent{\bf Proof of \namedref{#1}{#2}:~}}
%\def\proof{\Proof}
%
%\def\Sketch{\noindent{\bf Proof Sketch}: }
%
%\newcommand{\Unit}{\tilde{\mathbf{1}}}
%\newcommand{\Int}{\mathrm{int}}
%\newcommand{\Val}{\mathrm{val}}
%
%
%\newcommand{\OO}[1]{O\left( #1\right)}
%\newcommand{\OM}[1]{\Omega\left( #1 \right)}
%\newcommand{\Set}[1]{\left\{ #1 \right\}}
%\newcommand{\Seq}[1]{\left\langle #1 \right\rangle}
%\newcommand{\Range}[1]{\left\{1,\ldots, #1 \right\}}
%\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
%\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
%%\newcommand{\ignore}[1]{}
%\newcommand{\Exp}[1]{\mathbf{E}\left[#1\right]}
%\newcommand{\Var}[1]{\mathbf{Var}\left[#1\right]}
%\newcommand{\Prob}[1]{\Pr\left[ #1 \right]}
%\def\DEF{\stackrel{\rm def}{=}}
%\newcommand{\Eqr}[1]{\equalityref{#1}}  %{Eq.~\ref{#1}}
%\newcommand{\diff}{\ne}
%\newcommand{\sO}{\tilde{O}}
%
%\newcommand\cwc{\textrm{CWC}\xspace}
%\def\CWC{\cwc}
%\newcommand\argmin{\operatorname*{argmin}}
%\newcommand\argmax{\operatorname*{argmax}}
%\newcommand\WLOG{{w.l.o.g.}\xspace}
%%%%%%%%%%%%%%%%%%%%
%\newcommand\bl{b_\ell}
%\newcommand\bc{b_c}
%\newcommand\blmin{\phi}
%%%%%%%%%%%%%%%%%%%%
%\newcommand\bC[1]{\bc({#1})}
%\newcommand\bL[2]{w({{#1}, {#2}})}
%%%%%%%%%%%%%%%%%%%%
%%\newcommand\kR[1]{k^+({v_{#1}})}
%\newcommand\kR[1]{k(#1)}
%\newcommand\IR[1]{I_{#1}}
%\newcommand\ZR[1]{Z_{#1}}
%\newcommand\kL[1]{k^-({v_{#1}})}
%\newcommand\interval[2]{[{#1}, {#2}]}
%%\newcommand\kCR[1]{k_C^+({v_{#1}})}
%\newcommand\kCR[1]{k_c(#1)}
%%\newcommand\kLR[1]{k_L^+({v_{#1}})}
%\newcommand\kLR[1]{k_\ell(#1)}
%\newcommand\bLminR[1]{\blmin\left(\IR{#1} \right)}
%\newcommand\bLminL[1]{b_{L \min}^-({v_{#1}})}
%\newcommand\bLmin{b_{L \min}}
%%%%%%%%%%%%%%%%%%%%
%\newcommand\uploadproblem{\text{Upload-Problem}\xspace}
%\newcommand\twouploadproblem{\text{2-Upload-Problem}\xspace}
%\newcommand\twotransferproblem{\text{2-File-Tranfer-Problem}\xspace}
%\newcommand\VAproblem{\text{Vector-Addition-Problem}\xspace}
%\newcommand\MMproblem{\text{Matrix-Multiplication-Problem}\xspace}
%%%%%%%%%%%%%%%%%%%%
%\newcommand{\CR}{\textbf{Cloud-Read}\xspace}
%\newcommand{\CW}{\textbf{Cloud-Write}\xspace}
%\newcommand{\CCR}{\textbf{Cloud-Cast}\xspace}
%\newcommand{\CAW}{\textbf{Cloud-All-Write}\xspace}
%\newcommand{\CCW}{\textbf{Cloud-Combined-Write}\xspace}
%\newcommand\gread{\text{group-read}\xspace}
%\newcommand\gwrite{\text{group-write}\xspace}
%\newcommand\twointervaladdition{\text{2-Interval-Addition}\xspace}
%\newcommand\vectoradditionstage{\text{Vector-Addition-Single-Stage}\xspace}
%\newcommand\vectoraddition{\text{Vector-Addition}\xspace}
%\newcommand{\para}[1]{\par\noindent$\rhd$~\emph{#1}}
%
%\usepackage{graphicx,accents}
%
%\makeatletter
%\DeclareRobustCommand{\cev}[1]{%
%  \mathpalette\do@cev{#1}%
%}
%\newcommand{\do@cev}[2]{%
%  \fix@cev{#1}{+}%
%  \reflectbox{$\m@th#1\vec{\reflectbox{$\fix@cev{#1}{-}\m@th#1#2\fix@cev{#1}{+}$}}$}%
%  \fix@cev{#1}{-}%
%}
%\newcommand{\fix@cev}[2]{%
%  \ifx#1\displaystyle
%    \mkern#23mu
%  \else
%    \ifx#1\textstyle
%      \mkern#23mu
%    \else
%      \ifx#1\scriptstyle
%        \mkern#22mu
%      \else
%        \mkern#22mu
%      \fi
%    \fi
%  \fi
%}
%
%
%%%% Local Variables:
%%%% mode: latex
%%%% TeX-master: "cwc"
%%%% End:

==> extension.tex <==
\section{\DNSUD{}-\MakeLowercase{ext}}
\label{sec:extension}

%%%%\subsection{Overview}
\label{sec:ext}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DNSUD{} heavily relies on the traditional DNS system and in particular on the authoritative servers.
\ignore{%%%%%%%%%%%%%%%%%
In case the authoritative server is unavailable and its domain name updates (to fix an erroneous update, or a required good update \cite{facebook}) the \DNSUD{} is futile.
In some cases \cite{facebook}, clients lost access to an Internet service because the TTL associated with the DNS record has expired since the corresponding authoritative server became inaccessible. The \DNSUD{} method provides a solution by extending the TTL indefinitely. 
This way, clients may receive the correct IP address of a domain name from the resolver since its TTL does not expire. However, if the authoritative server is inaccessible and a record update is required, or the record has been evicted from the resolver's cache, the basic version of \DNSUD{} is not enough. 
Here we extend \DNSUD{} to handle this case as follows:
}%%%%%%%%%%%%%%
Here we extend \DNSUD{} to provide remediation even if some authoritative servers are unavailable while their domain name updates.
To this end we store in every record in the \UpdateDBext{} the updated information, e.g., the new IP address for the domain. 
Of course, the \Extension{} service does not replace the current DNS system, it must be used only for emergencies and not routinely. Notice that the extension is compatible with \DNSUD{} without the extension and with the traditional DNS system, thus all three variants are compatible and may be used at the same time.

\begin{figure}[h!]
    \centering
    \includegraphics[width=8.4cm]{saveupdates-biggraph2.PNG}
    \caption{\Extension{} events and messages flow (We \underline{underline} the details that differ from \DNSUD, Figure \ref{fig:dnsud}): \newline
    1. InsertDomain - The authoritative server may become unavailable hence, upon updating a record, the owner of the faulty authoritative server sends the new record signed with a DNSSEC signing key to the \UpdateDBext. \newline 
    2. UpDNS request - The recursive resolver queries the \UpdateDBext{} every $\Delta$ time units.  \newline
    3. UpDNS-ext response - The \UpdateDBext{} responds with the list of domain names that have been updated in the last $\Delta$ time. In this extension some of these domain names come together with their corresponding update information.\newline
    4. UpdateCache - The recursive resolver removes the domain in the list from its cache and updates the cache with the domains in the list that come with their updated information. \newline
    5. DNS request - When a client sends a request to resolve a domain name, a cache hit may occur on the resolver. \newline
    6. DNS response - The recursive resolver responds to the client with the updated IP address for a domain name.
    }
    \label{fig:saveupdates}
\end{figure}
\ignore{%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!b]
    \centering
    \includegraphics[width=\textwidth]{saveupdates-biggraph}
    \caption{\Extension{} flow chart (We underlined the changes from \DNSUD{} flow chart): \newline
    1. InsertDomain - The authoritative servers may become inaccessible, so upon updating a record, the authoritative server owners sends the new record to the \UpdateDBext. It inserts the record with the DNSSEC signing.\newline 
    2. UpDNS request - The recursive resolver queries the \UpdateDBext{} every $\Delta$ time units.  \newline
    3. ListUpdateDNS response - The recursive resolver receives the list of domains with their corresponding updates that have been updated in the last epoch.\newline
    4. StoreDNS - The recursive resolver updates the domains in its local cache with their corresponding updates. \newline
    5. DNS request - When a client sends a request to resolve a domain name, a cache hit occurs on the resolver. \newline
    6. DNS response - The recursive resolver responds to the client with the updated IP address for a domain name.
    }
    \label{fig:saveupdates}
\end{figure*}
}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ignore{%%%%%%%%%%%%%%%%
The next time the resolver receives a request for an updated domain name, it checks for the domain in its local cache and returns the correct DNS record to the client. Therefore, if \Extension{} is available, we can ensure IP updates for records. Of course, \Extension{} does not replace the current DNS network, so it must be used for emergencies, not as routine.
}%%%%%%%%%%%%%%%%%%%

\subsection{\UpdateDBext{} structure and messages}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\UpdateDBext{} holds two types of records: records as in the \UpdateDB{} besides new records with the following fields:
\begin{itemize}%%[leftmargin=0.12in]\setlength\itemsep{0.25em}
    \item Domain - The domain whose record has been recently updated.
    \item Subdomains - A flag indicating whether the domain's subdomains should also be removed from the resolvers' cache.
    \item \underline{DNS record} - Entire new DNS record.
    \item \underline{Signature} - Signing with DNSSEC, see Section \ref{sec:ext-security}.
    \item Timestamp - The time in which the record was inserted into the \UpdateDBext.
\end{itemize}

Upon receiving an InsertDomain request from an authoritative server owner (the authoritative server is down) the \Extension{}
first, verifies the request as explained in the security section \S\ref{sec:security}, and then inserts a new record into the \UpdateDBext{} with the above five fields.
\Extension{} handles the UpDNS request as in the original \DNSUD{} service, see Figure \ref{fig:saveupdates}.

Notice that unlike \DNSUD{}, \Extension{} does not 
allow Internet services to use unicast DNS services \cite{unicast}, i.e., to provide different IP addresses for different resolvers.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Adding a new resolver to the extension and the extension security }
Due to space limitation these and more \DNSUD{}-ext material are moved to Appendix \ref{sec:ApExt}

\ignore{%%%%%%%%%%  Remove from CoNEXT submission

\subsection{Adding a new resolver to the extension}
\label{sec:ext-joining-process}
Resolvers that recover from a crash for less than $MaxHistory$ time perform a sequence of UpDNS requests-replies until obtaining all the records in the \UpdateDBext{} up to the current time, see Section \ref{sec:update-process}.
However a new resolver or one that lost its network connection for more than $MaxHistory$ time performs the joining process, as in Section \ref{sec:joining-process}. 
In that process the resolver clears its cache and queries the \UpdateDBext{} to receive only records that have been inserted after it has started the joining process. Thus, in the peculiar case that an authoritative server crashes before a resolver starts the joining process (after being down for more than $MaxHistory$ time), this resolver does not receive the updated information that corresponds to the crashed authoritative server. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Security of the \Extension{}}
\label{sec:ext-security}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The additional threat on \Extension{} on top of the threats on the \DNSUD{} is the cache poisoning attack \cite{cache-injection-study, poison1, poison2, poison3} since the \UpdateDBext{} stores also record updates. To mitigate the attack, each authoritative server owner sends a DNSSEC \cite{rfc4035, dnssec-view, dnssec-view2} signature with the record in the InsertDomain request. Then, upon receiving the UpDNS response by the resolver, it verifies the signature of the record and then inserts the new DNS record to its local cache.
\ignore{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{enumerate}[leftmargin=0.15in]\setlength\itemsep{0.25em}
    \item Integrity of records stored by \UpdateDB{} - An attacker can cause a DNS cache poisoning attack\cite{poison1, poison2, poison3} by injecting the updated DNS records with incorrect values. The possible damage is high since Internet services may increase their TTLs indefinitely.
    \item DoS/DDoS on the \Extension{} that affects its availability - This becomes more severe since it prevents website owners from updating their DNS records if their authoritative server became inaccessible.
\end{enumerate}
}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nsdionly{%%%%%%%%%%%%%%%%%%%%%%%
\subsection{DNS unicast routing support} 
\label{sec:ext-unicast}
\delete{
Unlike the \DNSUD{} service, \Extension{} does not allow Internet services to use unicast DNS services after a record update, since the authoritative server owner can send only one record to the \UpdateDBext, which distributes to all resolvers. Thus, Internet service owners may use anycast DNS services or wait until their authoritative servers become available again.
}
}

\ignore{%%%%%%%%%%%%%%%%%%%%%%%%%%
We suggest the following mitigation to deal with this threat:\newline
Signing DNS records and not only the communication. Authoritative servers should sign them with DNSSEC  to prevent the injection of an incorrect records. Then, each resolver verifies the signature of a record, and only after the verification, it stores the received new IP address for a domain name in its local cache.
}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

}%%%%%%%%%%  Remove from CoNEXT submission

==> implications.tex <==
\section{Discussion}
\label{sec:implications}
Here we discuss possible implications that may result from using \DNSUD{}.



==> intro-old.tex <==
\section{Introduction}
\label{sec:intro}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
While being very critical for the Internet operation, the DNS system \cite{rfc1034} is unforgiving, it has no CTRL-Z, i.e., no undo command.
For example, several Microsoft services like Azure and others were not available for a few hours in 2019 due to an erroneous DNS update that could not be quickly corrected or undone \cite{azure}. 
Furthermore, when using short TTLs the system is very sensitive to authoritative server failures or crashes due to e.g., DDoS or other attacks \cite{facebook}.
In this paper, we examine \DNSUD{}, a method to add an undo command to the DNS system for a reasonable price in resources.
\DNSUD{} also increases the fault tolerant of the DNS system to name server crashes.

Internet domain name owners and managers have to set the TTL value associated with their domain records in the DNS system \cite{rfc1034} to dictate the maximum time a record may be stored in resolvers, stub resolvers, and client caches before they should obtain a fresh copy from the authoritative server \cite{rfc1035}.
Associating short TTL values with domain names is the current remediation for the DNS unforgiveness however it is expensive \cite{moura2019cache} in terms of futile DNS traffic (resulting from refreshing a popular domain record in different resolvers every TTL time). 
On the other hand, two major risks are associated with large TTL values \cite{choose-ttl-values}; first, if inadvertently a domain name is announced with the wrong IP, then the corresponding service is inaccessible for the duration of this large value; secondly, if a service has to change its IP address (e.g., for maintenance, load balancing or any other reason) then again the clients have to wait for the expiration of the TTL before the change takes effect. 
In this paper \DNSUD{} is suggested to provide the benefits of both: an undo command for quick recovery from erroneous updates and large TTL values to reduce the load on DNS authoritative servers. Both increase the robustness of the DNS system.

\ignore{%%%%%%%%%%%%%%%%%
As a result, the TTL value of many domains is very short ($1-5$ minutes), even though most domains change their IP address infrequently (less than once a month). Content distribution networks (CDNs) \cite{kazunori2012cdn, centralized-dns} use even shorter TTLs ($\sim$ tens of seconds) to achieve high availability, load balancing, and frequent updates but only some of them indeed change their IP quite often.

The main consequence of choosing short TTL values is that most DNS requests receive the same response over and over, resulting in extra traffic to learn that there is nothing new.
}%%%%%%%%%%%%%%%%%%

There are two major observations on which \DNSUD{} is based; First, the method is backward compatible and adaptive. That is, any portion of the DNS system may use \DNSUD{} while other parts continue operating in the traditional DNS method. 
Secondly, according to our measurements about $80\%$ of the domains on the Internet change their IP address less than once a month on average.
Let us define domain update time, $T^D_{update}$ as the average inter update time for domain $D$. We say domain $D$ is \emph{stable} if $T^D_{update} > 1$ month, and \emph{erratic} otherwise. \DNSUD{} is designed under the assumption that only \emph{stable} domains use the service, while \emph{erratic} domains keep using the traditional system.
The observation is that \emph{stable} domains have a very high ratio of domain update time to TTL length.
As a typical example, consider the popular Microsoft \emph{stable} domain office.com whose TTL is $5$ minutes, but its IP address has not been updated for $3$ years.
Thus, at least every $5$ minutes, office.com is evicted from the resolvers' cache, and upon receiving a DNS request, the resolvers issue a new query to the authoritative server holding office.com.  That is, short TTL values are a significant cause of futile traffic between clients and resolvers as well as between resolvers and authoritative servers.

As stated above, our motivation comes from incidents in which the wrong IP address was inadvertently associated with a domain, resulting in service disruption for the duration of the corresponding TTL value, which sometimes was several hours, as in the Microsoft incident from 2019 \cite{azure}. Where 
Microsoft services like Azure, Microsoft 365 umbrella, Dynamics, and DevOps were down for more than 2 hours due to an incorrect DNS update.
Microsoft published: "During the migration of a legacy DNS system to Azure DNS, some domains for Microsoft services were incorrectly updated." In another incident, in 2021, SiteGround services \cite{siteground} were not accessible to Google crawlers for several hours due to an incorrect DNS update.
The company explained: "We have implemented a fix for the Google bot crawling issue experienced by some sites... Please allow a few hours for the DNS changes to take effect".
Other similar incidents have occurred, such as Zoho\cite{zoho}, Slack \cite{slack}, Microsoft \cite{win-update}, and Akami \cite{akami}.

\ignore{%%%%%%%%%%%%%%%%%%%%%%%%% 
We estimate this excess traffic by calculating the ratio between the average time between IP address updates for a domain and its corresponding TTL value. In addition, our analysis indicates that more than $80\%$ of the $500,050$ most popular domains change their IP address less than once a month and more than $60\%$ less than once a year. \footnote{We combined an up to date top $500$ domains list of moz.com with the top $500,050$ list of Alexa from $2021$. Due to the constrains of SecurityTrails \cite{securitytrails} we sampled $200$ domains from this list.  See Section \ref{sec:freq-updates}.} For these domains we found that at most $0.2\%$ of DNS responses contain a DNS record that has been changed since the previous response, \ariel{e.g., the IP address of the domain "Office.com" has not changed for more than $3$ years, but its TTL value is $300$ seconds.
Thus, every $300$ seconds at most, the domain is evicted from the resolver's cache, and upon receiving a DNS request, the resolvers issue it to the authoritative server.} As a result, short TTL values are a significant cause of excess traffic between clients and resolvers as well as between resolvers and authoritative servers.
This excessive traffic also causes client latency and server performance impairment \cite{moura2019cache}. In addition, website owners expose themselves to another availability problem - if there is no access to their authoritative servers, when their short TTL expires, the access to their website is disabled \cite{facebook}.

As stated above, our motivation comes from incidents in which the wrong IP address was inadvertently associated with a domain, resulting in service disruption for the duration of the corresponding TTL value, which sometimes was several hours, as in the Microsoft incident from 2019:
\begin{itemize}[leftmargin=0.12in]\setlength\itemsep{0em}
    \item Microsoft \cite{azure} - In 2019, Microsoft services like Azure, Microsoft 365 umbrella, Dynamics, and DevOps were down for more than 2 hours due to an incorrect DNS update. Microsoft published: "During the migration of a legacy DNS system to Azure DNS, some domains for Microsoft services were incorrectly updated."
    \item SiteGround \cite{siteground} - In 2021, SiteGround services were not accessible to Google crawlers for several hours due to an incorrect DNS update. The company explained: "We have implemented a fix for the Google bot crawling issue experienced by some sites... Please allow a few hours for the DNS changes to take effect".
\end{itemize}
Similar incidents have occurred, such as Zoho\cite{zoho}, Slack \cite{slack}, Microsoft \cite{win-update}, and Akami \cite{akami}.

}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nsdionly{%%%%%%%%%%%%%%%%%%%%
Many people rightfully describe the DNS as the phone book of the Internet.
In both, when clients need the IP address of a domain or the phone number of another person or business, they query either the DNS system or use a search engine to query for the desired phone number. However, there is a difference; IP addresses sometimes change frequently, while the phone number of people change quit infrequently. Thus using a contact-list (cache) on mobile devices is helpful for phone books but requires much more care and sophistication in the DNS system due to the dynamic nature of IP addresses associated with endpoints. Still, the DNS system relies on caches with a TTL value attached to each record. However, suppose, for some reason, the cache contains the wrong IP address for a domain. In that case, there is no automatic mechanism to query the authoritative server again to get a fresh record. As a result, clients query the DNS system regularly, regardless of whether record updates have occurred, unlike updates of a phone contact list when the mentioned person updates her phone number.

Internet service owners compromise on any choice of TTL: large TTL values cause slow recovery from an IP address change, while short TTLs generate excess traffic and load.
}%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this paper, we propose \DNSUD{}, a mechanism to update a record in resolver caches before the associated TTL has expired.
In a nutshell, \DNSUD{} updates the resolvers about domains whose records were recently updated.
After that, the resolvers remove the corresponding records from their cache.
Upon receiving a subsequent request for a removed domain, the resolver performs a new resolution in the standard DNS system to get a fresh update.
\DNSUD{} is secure, efficient, and fully compatible with the current DNS system. 

Furthermore, \DNSUD{} enables Internet services to significantly increase the TTL values associated with their domain names in resolvers' cache (client caches are discussed in the sequel). Thus, we add an additional second and larger TTL value, called \DNSUD-TTL while preserving the traditional TTL.
To achieve backward compatibility, the additional \DNSUD-TTL is included in an optional field (in the ADDITIONAL section \cite{rfc1035}) of DNS responses.
\ignore{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Domain names with short TTL values (less than $10$ minutes) benefit from \DNSUD{} since larger TTL values reduce their DNS traffic and the average latencies experienced by clients. Furthermore, for domain names with large TTL values, \DNSUD{} provides quick recovery from IP address changes.
To achieve the backward compatibility of the \DNSUD, we added an additional TTL value, an optional field, used by clients and resolvers that are not yet using the \DNSUD, besides the traditional TTL value (used by the clients).
} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this way, an authoritative server that uses \DNSUD{} can communicate with resolvers that implemented or did not the method, and a resolver that uses \DNSUD{} can communicate with both authoritative servers that implemented or did not the method.
In Section \ref{sec:beyond}, we discuss methods to expand \DNSUD{} to enable clients to use the additional larger TTLs and reduce the futile DNS traffic also between clients and resolvers.
\ignore{While the method could be applicable also for clients and stub resolvers, in their case efficiency and complexity of the method, as well as their small cache size, needs to be considered, see Section \ref{sec:beyond}.}
\nsdionly{%%%%%%%%%%%%%%%%%%
Unlike the phone book, the trigger in \DNSUD{} is initiated by the authoritative server rather than the client, i.e., some kind of a pull method initiated by a push.
}%%%%%%%%%%%%%%%%%%

Related work and alternative methods are presented in Section \ref{sec:background}. Description of the \DNSUD{} service with the primary implication of increasing TTL values and how we preserve the backward compatibility of \DNSUD{} is provided in Section \ref{sec:solution}.
In section \ref{sec:measurements}, we measure the parameters that produce the current drawbacks of the DNS system.   
In section \ref{sec:analysis}, we analyze the relevancy and feasibility of the method. 
Detailed description of the \DNSUD{} is provided in Section \ref{sec:drill-down}.
In section \ref{sec:security} we introduce the threat analysis of the method.
In Section \ref{sec:beyond}, we discuss ways to expand the method also to the clients -- resolvers communication, that is, updating stale records in browsers and other client applications before the corresponding TTL has expired.
In Section \ref{sec:extension} an extension is presented to provide fast recovery when an authoritative server is unavailable.
Finally, conclusions are given in Section \ref{sec:conclusion}.

\ignore{Our analysis indicates that more than $80\%$ of the $50$ most popular domains and the $450-500$ most popular, change their IP address less than once a month, and more than $50\%$ less than once a year. Domain names with short TTL values (less than $10$ minutes) benefit from \DNSUD, by using much larger TTL values and reducing their DNS traffic and the average latencies experienced by clients. Also, \DNSUD{} could ensure a constant and quick recovery from IP address changing for domain names with large TTL values.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cwc"
%%% End:


==> model-body.tex <==
The CWC model is a synchronous network whose underlying
topology is described by a weighted directed graph $G=(V, E, w)$. The node set
consists of two disjoint subsets: $V=V_p\cup V_c$, where $V_p$ is the
set of \emph{processing nodes}, and $V_c$ is the set of \emph{cloud
	nodes}.
Cloud nodes are passive nodes that function as shared storage: they
	support read and write requests, and do not perform any other computation.  
	Cloud nodes represent storage clouds (such as Dropbox) and not
	computation clouds (such as EC2).	
	% that serve only as storage nodes.  
	A processing node may be 
connected to any node, but there
are no links between different cloud nodes\ignore{, i.e.,
  $E\cap(V_c\times V_c)=\emptyset$}.
We use $n$ to denote the number of processing nodes (the number of
cloud nodes is typically constant).
	
% Let $E_L$ (``local links"), denote the set of links that
% connect two processing nodes and $E_C$ (``cloud
% links") the set of links that connect processing nodes to cloud nodes. 
% Each link $e\in E=E_L\cup E_C$ has a prescribed bandwidth $w(e)$.

We denote the set of links that
connect two processing nodes by $E_L$ (``local links''), and by $E_C$ (``cloud
links'') the set of links that connect processing nodes to cloud nodes. 
Each link $e\in E=E_L\cup E_C$ has a prescribed bandwidth $w(e)$.
We denote by $G_p\DEF(V_p,E_L)$ the graph $G-V_c$, i.e., the graph spanned by the processing nodes.

Our execution model is the standard synchronous network model,
%derived from CONGEST \cite{Peleg:book}.
%Executions proceed in synchronous rounds,
where each round consists of processing nodes receiving messages sent
in the previous round, doing an arbitrary local computation, and then
sending messages.  The size of a message sent over a link $e$ in a
round is at most $w(e)$ bits.
 
% Cloud nodes 
% %
% In this paper we focus on time complexity, i.e., number of rounds
% required to execute a task.


Cloud nodes do not perform any computations: they can only receive requests we denote by \FR
and \FW , to which they respond in the following round. More
precisely, each cloud node has unbounded storage; to write, a
processing node $v_i$ invokes $\FW$ with arguments that describe the
cloud node $v_c$, a filename $f$, a bit string $S$, and the location
(index) within $f$ that $S$ needs to be written in. It is assumed that
$|S|\le w(v_i,v_c)$ bits (longer writes can be broken to a series of
\FW operations). To read, a processing node $v_i$ invokes $\FR$ with
arguments that describe the cloud node $v_c$, a filename $f$ and the
range of indices to fetch from $f$. Again, we assume that the size of
the range in any single \FR invocation by node $v_i$ is at most
$w(v_i,v_c)$.

For both the \FW and \FR operations we ignore the metadata
(i.e., $v_c$'s descriptor, the filename $f$ and the indices)
and assume that the total size of metadata in a single round
is negligible and can fit
within $w(v_i,v_c)$.%
\footnote{
	Otherwise, processing nodes may use the metadata parameters to exchange information
	that exceeds the bandwidth limitations
	(for example, naming a file with the string representation of a message whose length is
	larger than the bandwidth). 
}

\FW operations are exclusive, i.e., no other operation (read or
write) to the same file location is
allowed to take place simultaneously.
Concurrent \FR operations from the same location are allowed.


%to complete a task.

% Examples for that may be shared memory between processors in the
% same computer, or cloud storage such as Dropbox, Google Drive,
% shared folders, and Git.

% assume the cloud model in this paper to be that way, to avoid conflicting writes to the cloud, and to simplify the cloud as an atomic node that allows distributed reading and writing.\\
% We allow the cloud storage to be infinite, because in this paper the
% limitations on the cloud will come from the limited bandwidth of the
% links to it.

% \boaz{how to fix this?}  We mark the bandwidth of node $v_i$ to the
% cloud, i.e. the bandwidth of the cloud edge $(v_i, v_c)$, as
% $\bC{i}$.

% We mark the bandwidth between two nodes $v_i, v_j$, i.e. the
% bandwidth of the local edge $(v_i, v_j)$, as $\bL{i}{j}$.



==> old/app-comb.tex <==
\section{Proofs for Section~\ref{sec:va}}
\label{app-combining}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ProofOf{Theorem}{thm-ccw-gen}
% \Proof
By algorithm. The idea is to do the combining over a binary
``computation tree'' by
using the cloud to store the partial results.
%calculating partial combining results and using files in the cloud as relay stations.
%writing node values in the cloud.
The computation tree is defined as follows (see
\figref{fig-tree}).
Let $X_i^j$ denote the $i$-th node at level $j$, as well as the
value of that node.
The leaves $X_i^0$ are the input values, and the value of
an internal node $X_{i}^{j+1}$ at level $j+1$ with left child
$X_{2i}^{j}$ and right child $X_{2i+1}^{j}$ is $X_{2i}^{j}\otimes
X_{2i+1}^{j}$. Pseudocode is provided in
\algref{alg:caw-flow}. Correctness of the algorithm follows from the
observation that after each execution of Step \ref{alg:caw-flow:caw},
there are 
$m$ files of size $s$ written in the cloud, whose product is the
required output, and that $m$ is halved in every iteration.
% Afterwards, each of the first $\ceil{m/2}$ nodes
% read two of the files from the cloud (while maintaining their order),
% and calculate their product, while maintaining the fact that each of
% the $m$ files is read exactly once.  
If at any iteration $m$ is odd,
then node $\ceil{m/2}-1$ only needs to read one file, and therefore we
set the other file that it reads to be $\Unit$.
%, i.e., of size $0$.
%For all other nodes we set their input to be $\epsilon$ too.
When $m$ reaches $1$, there is only $1$ file left, which is the
required result. % product of all inputs by induction.
% The algorithm is finished by writing said last file to the cloud, and by that completing
% \CAW.

% See \figref{fig-tree} for an example of the values held in each node in every iteration.
% Note that every non-leaf node in the tree reads $2$ values and writes $1$ value to the
% cloud, which corresponds to $2$ invocations of \CAR and $1$ invocation of \CAW in
% every layer.

%Let $X_i^j$ denote the $s$-bit file that node $i$ has in iteration $j$
%(for every $i$, $X_i^0 = S_i$).
As for the time analysis: Clearly, a single iteration of the \textbf{while} loop %in Step \ref{alg:caw-flow:loop}
takes $3T_s = O(T_s)$ rounds.
Note that when writing $\Unit$ to the cloud, it can be encoded as a $0$-bit string,
which can only improve the runtime.
%(note that if some of the input files
%are of size $0$, the runtime can only be improved, and thus $T$ remains an upper bound).
There are $\ceil{\log n}$ rounds due to Step \ref{alg:caw-flow:advance},
and Step \ref{alg:caw-flow:last-caw} is also completed in $O(T_s)$ rounds,
and thus the total runtime of the algorithm is $O(T_s \log{n})$.
\QED

\begin{figure}[htb]
	%\small
  \begin{center}
    \begin{tikzpicture}[scale=0.8]
      \node [draw]{$X_0^3$} [level distance=10mm,sibling distance=50mm]
      child {
        node [draw]{$X_0^2$} [level distance=10mm ,sibling distance=25mm]
        child {
          node [draw] {$X_0^1$} [level distance=10mm ,sibling distance=12mm]
          child {node [draw] {$X_0^0$}}
          child {node [draw]{$X_1^0$}}
        }
        child {
          node [draw]{$X_2^1$} [level distance=10mm ,sibling distance=12mm]
          child {node [draw] {$X_2^0$}}
          child {node [draw] {$X_3^0$}}
        }
      }
      child {
        node [draw]{$X_4^2$} [level distance=10mm ,sibling distance=25mm]
        child {
          node [draw] {$X_4^1$} [level distance=10mm ,sibling distance=12mm]
          child {node [draw] {$X_4^0$}}
          child {node [draw]{$X_5^0$}}
        }
        child {
          node [draw]{$X_6^1$} [level distance=10mm ,sibling distance=12mm]
          child {node [draw] {$X_6^0$}}
          child {node [draw] {$X_7^0$}}
        }
      };
    \end{tikzpicture}
  \end{center}
  \caption{\em Computation tree  with $n=8$.
    $X_i^j$ denotes the result stored in node $i$ in iteration $j$.}
  \label{fig-tree}
\end{figure}

\ProofOf{Theorem}{thm-ccr-gen}
First note that if there were $n$ copies of the input file
$S$ in the cloud, then \CCR and \CAR would have been the exact same
problem.  Now, any algorithm for \CAR with $n$ inputs of size
$s$ in the cloud can be modified so that each invocation of $\FR$ for
file $S_i$, is converted to \FR for file $S$,  the input of \CCR. This
change is legal by our assumption that concurrent reads are allowed,
and by assumption that $S$ cannot be written to during \CCR.
%\todo{when did we make that assumption?}.

Clearly the modified algorithm solves \CCR,
and requires $T_s$ rounds.  \QED

\ProofOf{Theorem}{theorem:CW_UB}
The algorithm broadcasts all $s$ bits to all nodes in $\BR i$,
and then each node writes a subrange of the data whose size is
proportional to its cloud bandwidth. Correctness is obvious.
As for the time analysis:
Steps \ref{cw-alg-BFS-tree}-\ref{cw-alg-send-local} require $O(\kR i)$ rounds.
In the loop of steps \ref{cw-alg-node-write}-\ref{cw-alg-ack},
$\bc(\BR i)$ bits are sent in every round, and thus it terminates in
$O({s}/{\bc(\BR i)})$ rounds. The theorem follows from the definition of $\ZR i$.
\QED

\ProofOf{Theorem}{theorem:CW_LB}
By definition, $\ZR{i} = \kR{i} + {s}/{\bc(\BR{i})}$.
\lemmaref{lemma:cluster_diameter} and \lemmaref{lemma-cluster-bc} show
that each term of $\ZR{i}$ is a lower bound on the running time of any
algorithm for $\CW_i$.  \QED
\begin{lemma}
	\label{lemma:cluster_diameter}
	$\CW_i$ in a fat-links \CWC system   requires
	$\Omega \left( \kR{i}\right)$
	rounds.
\end{lemma}
\Proof Let $A$ be an algorithm for $\CW_i$ that writes string $S$  in
$t_A$ rounds. 
If $t_A \ge \Diam(G_p)$ then $t_A \ge \kR{i}$ and we are
done. Otherwise, we count the number of bits of $S$ that can get to
the cloud in $t_A$ rounds.  Since $S$ is initially stored in $i$, % in
% round $t$ only the nodes of $\Br{t-1}{i}$ can write to the cloud parts
% of $S$.  It follows that
in a given round $t$, only nodes in $\Br{t-1}{i}$ can write pieces of
$S$ to the cloud. %  at most
% $\bc(\Br{t-1}{i})$ bits of information can be sent to the cloud
% and
Therefore, overall, $A$ writes to the cloud at most
$\sum_{t=1}^{t_A}\bc(\Br{t-1}{i}) \le t_A\cdot\bc(\Br{t_A-1}{i})$
bits. Hence, by assumption that $A$ solves $\CW_i$, we must have
$t_A\cdot\bc(\Br{t_A-1}{i}) \ge s$. The lemma now follows from
definition of $\kR{i}$ as
the minimal integer
% 
% \footnote{ $\kCR{i}$ may be $\Diam(V_p)$ if no such integer exists,
%   but $t_A$ is an integer that satisfies the $\kCR{i}$ formula so this
%   is not the case.  } 
$\ell \le \Diam(G_p)$ such that
$(\ell \tp 1) \cdot \bc( \Br{\ell}{i} ) \ge s$ if it exists
(otherwise, $\kCR{i}=\Diam(G_p)$ and $t_A>\Diam(G_p)$). Either way,
we are done.
%\boaz{rephrased}
\QED


\begin{lemma}\label{lemma-cluster-bc}
	$\CW_i$ in a fat-links \CWC system   requires
	$\Omega \left({s}/{\bC{\BR{i}}} \right)$ rounds.
\end{lemma}

\Proof Let $A$ be an algorithm that solves $\CW_i$ in $t_A$ rounds.
If $\kR{i}=\Diam(G_p)$ then $\BR{i}$ contains all processing nodes
$V_p$, and the claim is obvious, as no more than $\bC{V_p}$ bits can
be written to the cloud in a single round.  Otherwise,
$\kR{i} \ge {s}/{\bC{\BR{i}}} - 1$ by \defref{def-Bi}, and we are done
since $t_A = \Omega(\kR{i})$ by \lemmaref{lemma:cluster_diameter}.
%Otherwise, $\kR{i} = \kLR{i}$. Let us denote $w_R=\bL{i\tp
%	\kR{i}}{i\tp \kR{i}\tp1}$. In this case we have
%$w_R < \bc(\IR{i})$.  We count how many
%bits can leave $\IR{i}$.  Similarly to \lemmaref{lemma:interval_BN},
%in a single round, at most $\bC{\IR{i}}$ bits can leave through the
%cloud links, and at most $w_R$ bits can leave through
%the local links. Since $A$ solves $\CW_i$, we must have
%$
%s
%~\le~t_A\cdot\left(\bC{\IR{i}} +w_R\right)
%~\le~ 2t_A \cdot \bC{\IR{i}} ~,$
%and hence $t_A = \Omega\left({s}/{\bC{\IR{i}}} \right)$.
\QED

From \theoremref{theorem:CW_LB}, we get the following lemma:
\begin{lemma} \label{lemma:cloud-cluster-timespan}
	For every node $i$, $Z(\BR{i}) \le Z_{\BR{i}}(i) = O(Z_i)$.
\end{lemma}

\begin{lemma} \label{lemma:alg:ccw-high:node}
	\algref{alg:ccw-high:node} computes $\bigotimes_{i=1}^m{P_i}$
	%  with each cluster $B\in \cC$ operating for at most
	in $O(\ZC(\CC) \cdot \log{|\CC|})$ rounds,
	assuming that all clusters operate in complete parallelism.
\end{lemma}
\Proof Computing all values in a tree layer requires a constant number
of \CW and \CR invocations in a cluster, i.e., by
\defref{def-covers},
%\theoremref{theorem:CW_UB}, \theoremref{theorem:CR_UB},
%every cluster $B\in \CC$ has to work for 
at most $O(\ZC(\CC))$ rounds of work in every layer.
%a layer is computed in
%$O\left(\ZC(\CC)\right)$ rounds.
The number of layers is  $\ceil{\log|\CC|}$.
the result follows.
\QED

From %\lemmaref{lemma:alg:ccw-high:overlap} and
\lemmaref{lemma:alg:ccw-high:node},
considering the multiplexing of Step \ref{ccw-1},
we get the following result:

\begin{lemma}\label{ccw-lem-hi}
	Line \ref{ccw-high} of \algref{alg:ccw-hi} is completed in
	$O(\ZC(\CC) \cdot \load(\CC) \cdot \log |\CC|)$ rounds.
\end{lemma}
We can therefore conclude:
\par\smallskip\noindent\textbf{Proof of \theoremref{thm-ccw-covers-ub}:~} By \lemmaref{ccw-lem-lo} and
\lemmaref{ccw-lem-hi}. 
\QED
%noting that $|C|\le n$ and $|I_{j_{\max}}|\le n$.
% \gal{This line that completes the proof is too hidden and easy to miss}


\ProofOf{Theorem}{theorem:CCW-LB}
By reduction from \CW.
Let $i$ be any processing node.
Given $S$, assign $S_i=S$ as the input of node $i$ in \CCW, and for every 
other node $j \ne i$, assign $S_j = \Unit$. Clearly, any algorithm for \CCW
that runs with these inputs solves $\CW_i$ with input $S$.
the result follows from \theoremref{theorem:CW_LB}.
\QED




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cwc"
%%% End:


==> old/applications.tex <==
\def\XX{\mathbf{x}}
\def\YY{\mathbf{y}}
\def\ZZ{\mathbf{z}}

\section{\CWC Applications}
\label{sec:applications}

%Here we consider the implementation of basic Federated Learning and Deduplication  (\sectionref{sec:dedup}) operations in the CWC model.

In this \dsection we briefly explore some of the possible applications
of the results shown in this \paper to
% While file transfer operations and combining operators
% such as vector addition and matrix multiplication
% are already useful in their own right,
% here we consider the implementation of 
two slightly more
involved applications, namely Federated Learning (\subsectionref{sec:federated})
and File Deduplication (\subsectionref{sec:dedup}).

%We consider the implementation of basic Federated Learning (\sectionref{sec:federated})
%and Deduplication  (\sectionref{sec:dedup}) operations in the CWC model.
% \gal{I feel like there should be some more selling sentences here, about the usefulness of the model etc.
% I liked the old sentence about the fact that matrix multiplication and vector addition are good applications in their own right}

\ignore{%%%%%
	In this \dsection we briefly explore some of the possible applications
	of the results shown in this \paper.
	% We believe that the \CWC framework
	% can be useful in many real-world applications,
	% and more specifically that the \CW, \CR, \CCW and \CCR
	% problems may be useful as primitives for that matter.
	Before we start, we note that %matrix multiplication and
	matrix (or vector) addition over a finite field satisfy the requirements of
	the combining operator analyzed in \sectionref{sec:va} (we need the
	finite field assumption so that the length of the encoding of the
	result of applying the operation
	is the same as the encoding length of each operand). 
	Furthermore, the addition operator is modular, with grain size which is
	the number of bits required to encode an element in the underlying field.
	In the remainder of this section, we describe two slightly more
	involved applications, namely federated learning (\sectionref{sec:federated})
	and file deduplication (\sectionref{sec:dedup}).
}%%%%%%%%%



\subsection{Federated Learning in CWC}
\label{sec:federated}
\ignore{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	Here we explain how can the \cwc framework be used in the
	context of federated learning, abbreviated FL henceforth.
}%%%%%%%%%%
Federated Learning (FL) \cite{federated-17,federated-cacm} is a distributed Machine Learning
training algorithm,
by which an ML model for some concept is acquired.
The idea is to train over a huge data set that is distributed across many devices such as mobile phones and user PCs, % \gal{is 'users PCS' correct english?},
without requiring the edge devices to explicitly exchange their data. Thus it gives the end devices some sense of privacy and data protection.
Examples of such data is personal pictures, medical data, hand-writing or speech recognition, etc. 


\ignore{%%%%%%%%%%%%
	First, let us briefly review the concept of FL (see
	\cite{federated-17,federated-cacm} for a more detailed description; we
	concentrate on the \emph{horizontal} flavor of FL here). The
	premise is that while labeled data is abundant, much of it is
	private and the owners are not happy to share it (e.g.,
	medical or financial information, or personal photographs). On the other hand,
	effective learning by neural networks 
	requires massive samples of labeled data. To bridge over this gap,
	FL is a framework wherein each user applies the learning process to
	its private data, and the parameters of their
	learned networks are sent to a central trusted server which computes a weighted average 
	of the
	results and sends the combined values back to the users, %\gal{This can be done with CloudCast }
	who proceed to the next iteration (see \cite{federated-17} for more details).
	The goal is to ensure that the only
	information that leaks is the resulting combined network: no
	individually generated information is shared with others.
}%%%%%%%%%

In \cite{federated-secure}, a cryptographic protocol for FL
is presented, under the assumption that any two users can
communicate directly. The protocol of \cite{federated-secure} is
engineered to be
robust against malicious users, and uses cryptographic machinery such as
Diffie-Hellman key agreement and threshold secret sharing.  
We propose a way to do FL without using an active trusted central server, but only a passive storage 
server, namely cloud storage.
Here, we describe
a simple scheme
%that is tailored to the wheel topology of \figref{fig-ring},
that is tailored to the fat-links scenario,
assuming that
users are ``honest but curious,'' %\gal{what does it mean?} 
but not malicious.

%In a nutshell,
The idea is as follows.
Each of the users has a vector of $m$ weights.  Weights are represented
by non-negative integers from $\Set{0,1,\ldots,M-1}$, so that user
input is simply a vector in $(\mathbb{Z}_M)^m$. Let $\XX_i$ be the vector of user $i$.
The goal of the computation is to compute $\sum_{i=0}^{n-1}\XX_i$ (using addition over $\mathbb Z_M$) and store the result in the cloud.
We assume that $M$ is large enough so that no coordinate in the vector-sum exceeds $M$, i.e., that
$\sum_{i=0}^{n-1}\XX_i=\left(\sum_{i=0}^{n-1}\XX_i\bmod M\right)$.

To compute this sum securely, {we use basic multi-party computation in the \CWC model}.
Specifically, each user $i$
chooses a private random vector $\ZZ_{i,j}\in(\mathbb{Z}_M)^m$ uniformly,
for each of her neighbors $j$,
and sends $\ZZ_{i,j}$ to user $j$.
Then each user $i$ computes
$\YY_i=\XX_i- \sum_{(i,j)\in E} \ZZ_{i,j}+ \sum_{(j,i)\in E} \ZZ_{j,i}$,
where addition is modulo $M$. 
Clearly, $\YY_i$ is uniformly distributed even if $\XX_i$ is known.
Also note that $\sum_i\YY_i=\sum_i\XX_i$. Therefore all that remains
to do is to compute $\sum_i\YY_i$, which can be done by invoking \CCW,
where the combining operator is vector addition over $(\mathbb{Z}_M)^m$.
We obtain the following theorem from \theoremref{thm-ccw-ub}.

\begin{theorem}\label{thm-FL}
	In a fat-links network,
	an FL
	iteration with vectors in $(\mathbb{Z}_M)^m$ can be computed in
	$O(\Zmax \log^2 n)$ rounds.
\end{theorem}


Since the grain size of this operation is $O(\log M)$ bits, 
we can apply the pipelined version (\corollaryref{cor:modular-combining}) of \CCW
in case that the underlying topology is a cycle,
to obtain the following. % result.
\begin{theorem}\label{thm-FL=wheel}
	In the uniform $n$-node wheel,  an FL
	iteration with vectors in $(\mathbb{Z}_M)^m$ can be computed in
	$O(\sqrt{(m\log M)/\bc}+\log n)$ rounds, assuming that
	$\bc m\log M\le\bl^2$ and $\bc\ge\log M$.
\end{theorem}
\Proof Using the notation of \sectionref{sec:va} and \subsectionref{sec:wheel}, the assumption implies that $s=m\log M$, and $Z_{\max}=O(\sqrt{s/\bc})=O(\sqrt{(m\log M)/\bc})$. The result follows
from \theoremref{thm-aw-modular} and \corollaryref{cor:modular-combining}.
\QED
% From
% that point on, computation proceeds as usual using the $\YY_i$ values
% instead of the $\XX_i$ values. It is easy to see that
% $\sum_{i=1}^n\YY_i=\sum_{i=1}^n\XX_i$ because the $\ZZ_i$ vectors cancel
% out. It is also clear that any partial sum of the $\ZZ_i$s is a random vector in
% $(\mathbb{Z}_M)^m$. 

% While homomorphic encryption can be used in principle,
% The observation that makes FL work is that the weights vectors are
% additive: if the data is split over $n$ agents, with agent $i$ owning
% data $D_i$, and applying an iteration of the network $N$ results in
% improvement vector $v_i=N(D_i)$, then the global improvement vector
% $v=N(\bigcup_{i=1}^nv_i)$ satisfies $v=\sum_{i=1}^nv_i$.
% This additivity allows each user to apply the current network to her
% private data, send the resulting vector to a \emph{trusted central
%   server}, which combines the results, updates the network, and sneds
% the updated description to the users for another iteration, without
% any user compromising the privacy of her data. Another advantage of
% FL is that the computation load is shared among the users, relieving
% the demand on the server by some amount.

% Our \cwc paradigm can be used by FL in case where user-cloud bandwidth
% is an issue, while local communication enjoys high bandwidth. The idea
% is that users can locally--and privately--add 
% weight vectors using local links, and upload the resulting vector
% collectively. This way iteration time can be cut down considerably.

\def\dcup{\widetilde{\cup}}

\subsection{File Deduplication With the Cloud}
\label{sec:dedup}

Deduplication, or Single-Instance-Storage (SIS), is a central problem
for storage systems (see, e.g., \cite{dedup,
	dedup-performance,bolosky2000single}). 
%\textbf{(GG: is \cite{dedup} legitimate? also, something in the bib \dsection of it is kinda messed up)}
Grossly simplifying, the motivation is the following: Many of the
files (or file parts) in a storage system may be unknowingly
replicated. The general goal of deduplication (usually dubbed dedup)
is to identify such replications and possibly discard
redundant copies.  Many cloud storage systems use a dedup mechanism
internally to save space. Here we show how the processing nodes can cooperate to
carry out dedup without active help from the cloud, when the files
are stored locally at the nodes (cf.\
serverless SIS~\cite{serverless-SIS}). We ignore privacy
and security concerns here.


% Here we focus on file-based deduplication, but the results can be
% adjusted to block-based deduplication as well.

% is to calculate a hash value of each file,
% and compare it against some hash table of files that are already stored in the cloud.
% If the file already exists in the cloud, there is no need to upload the entirety
% of its content again. Otherwise the file is uploaded to the cloud
% and the hash value is added to said hash table.
% We are suggesting a solution to two variations of the SIS problem
% %As is the premise of t   his \paper, we are suggesting a method
% %to implement SIS
% in the \CWC model, namely on the \emph{wheel} topology,
% by distributing computation to the nodes that can use the cloud,
% rather than doing the computation in the cloud
% (a similar concept of Serverless SIS is described in \cite{serverless-SIS}).
% Therefore, for systems that already implement deduplication solutions in
% their cloud storage, our solutions will probably be obsolete.
% In addition, we do not consider privacy implications of our approach,
% and do not attempt to make it private nor secure.

%Note that many cloud infrastructures are already implementing or providing 
%a deduplication approach. Our solutions are beneficial on systems that do not
%have a built-in implementation for dedup.

%\subsection{Local File Deduplication}
%\label{local-file-dedup}
We  consider the following setting. 
Each node $i$ has a set of local files
$F_i$ (and their hash values), and the goal is to identify, for each
unique file $f\in\bigcup_i F_i$, a single owner user $u(f)$.
(Once the operation is done,  users may delete any file they do not
own.)
% which we call \textbf{the file set} of $i$. 
% Let $h:\Set{0,1}^\star\rightarrow\Set{0,1}^H$, be a
% \emph{hash function}, with $H$ being the size of the hashed values.
% We consider two files $f, f'$ to be the same file, if $h(f)=h(f')$.
% %Some files may be in more than one file group.
% Let $m$ be the total number of unique files in $F_0 \cup \ldots \cup F_{n-1}$.
% The goal is to delete duplicate files, so that every file would be
% in exactly one file group.

This is easily done with the help of \CCW, as follows.
Let
$h$ %h:\Set{0,1}^*\to\Set{0,1}^H$
be a has function. 
For file $f$ and processing node $i$, call the pair $(h(f),i)$ a
\emph{tagged hash}. Let the set
$S_i=\Set{(h(f), i) \mid f\in F_i}$ of tagged hashes of $F_i$ be the input of processing node $i$.
We define the associative operation $S_i\,\dcup\, S_j$ that takes two sets $S_i$
and $S_j$ of tagged hashes, and returns a set of tagged hashes without duplicate hash values, i.e., if $(x,i)$ and $(x,j)$ are both in the union $S_i\cup S_j$,
then only $(x, \min(i,j))$ will be in $S_i\,\dcup\,S_j$.
Intuitively, $\dcup$ is a binary dedup operation.  Clearly
$\dcup$ is associative and commutative, and %has a neutral operand ($\emptyset$), and
therefore can be used in the \CCW algorithm.
Note that if  the total number of unique files in the system is $m$, then
$s=m\cdot (H+\log{n})$.
Applying \CCW with operation $\dcup$ to inputs $S_i$, 
we obtain  a set of tagged hashes $S$ for all files in the system,
where $(h(f),i) \in S$ means that user $i$ is the owner of file $f$.
Then we invoke \CCR %algorithm presented in \theoremref{thm-AR},
to disseminate the ownership information to all nodes.
% Each node $i$ looks for the hash values of all files in its file set,
% and deletes files whose hash value is not mapped to $i$.
Thus dedup can be done in \cwc in $O(\Zmax \log^2 n)$ rounds.

\ignore{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\subsection{Cloud File Deduplication}
	% Although in the aforementioned task we managed to remove all duplications,
	% any node whose file have been removed will have no access to the remaining copy
	% of its deleted file afterwards.
	% We now discuss a similar problem, perhaps more suitable to
	% the world of cloud infrastructures:
	Next, assume that a \emph{multiset} $F$ of files is
	stored in the cloud, 
	% $m$ of which are unique,
	and
	% and each is mapped to its hash value (we assume that
	% upon uploading of a file, its hash value is written as well).
	%While some of the files may contain the exact same content.
	the goal is to replace each duplicate file by
	a reference to  its remaining copy.
	To do so, we partition the files among the users so that  each node
	$i$ is assigned a subset, $F_i\subseteq F$ whose size $|F_i$ is
	proportionate to 
	$\bc(i)$ (we assume that for all $i$,  $\bc(i)\ge H$).
	\boaz{how is this done?!}
	Then  each node $i$ reads $h(f)$ for all $f\in F_i$ from the cloud,
	and proceed to the algorithm described in \ref{local-file-dedup}
	with the following difference: instead of tagging the hash of a file
	with a node identifier, hashes are tagged by a reference to its storage
	in the cloud.
	After computing the result $S$,  each user $i$
	deletes from the cloud the files of $F_i$  files whose hashes in $S$
	are  not tagged by their location in $F_i$, and we are done.
}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%% Local variables:
%%% TeX-master: "cwc"
%%% End:

==> old/combining.tex <==

\section{Computing \& Writing Combined Values}
\label{sec:va}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ignore{Combining values en-route to the destination is one of the most useful 
operations in computer networks (e.g., convergecast \cite{Peleg:book}).
In the \CWC model, we propose the following \CCW abstraction.}
% In this \dsection we show how to implement it. First we give
% an implementation for the general case using straight-forward reductions to the primitives of \sectionref{sec-multiple}, and then a near-optimal algorithm for the case of fat-links networks.
% We also mention
% \CCR, which is analogous to broadcast.
%
%Specifically,
%In \CCW, 
\ignore{ %%%%%
Each node $i\in\Set{0,1,\ldots,n-1}$ has an
input $S_i$ of size $s$ 
bits, and the requirement is to write the combined value
$\bigotimes_{i=0}^{n-1}S_i$ to a given cloud node $v_c$, where
$\otimes$ is a given associative binary
operator that takes two $s$-bits operands and returns an
$s$-bits result.  Borrowing from Group Theory, we call the operation
$\otimes$ \emph{multiplication}, and $S_1\otimes S_2$ is
the \emph{product} of $S_1$ by $S_2$. In general, $\otimes$ is not
necessarily commutative. % unless explicitly stated otherwise.
We assume the existence of a
unit element for $\otimes$, denoted $\Unit$, such that
$\Unit\otimes S=S\otimes\Unit=S$ for all $s$-bits strings $S$. The
unit element is represented by a string of $O(1)$ bits.
%We note that $\otimes$ need not be
%commutative.


%\todo{Should I add here some examples for operators? such as vector addition,
%	bitwise operations, leader election ($s=\log n$), finding the maximal $k$ elements, etc.
%	Same goes for non-commutative operators: matrix multiplication,
%	pointer jumping, permutation combining}

Examples for commutative operators include
vector and matrix addition (over a finite field),
bitwise operations such as \texttt{and}, \texttt{or} and \texttt{xor},
leader election (with operand size $s = \log n$),
and the top-$k$ problem (with operand size $s= k\log n$).
Examples for non-commutative operators may be
matrix multiplication (over a finite field) and
function composition such as permutation combining
(with $s$ being the size of the domains and codomains of all functions).
}%%%%%

Observe that flow-based techniques are not applicable in the case
of writing a combined value, because the very essence of combining
violates conservation constraints. However, in
\subsectionref{sec-ccw-flow} we explain how to implement \CCW in the
general case using \CAW and \CAR. While simple and generic, these
implementations can have time complexity much larger than optimal.
%(see \remarkref{remark-alg-compare} in \subsectionref{ssec:case-studies}
%for an example of a topology
%where the round complexity of the flow-based \CCW algorithm is larger than the optimal
%round complexity by a power of $2$).
We offer partial remedy in \subsectionref{sec-fat-combining}, where we
present our main result: an algorithm for \CCW 
when $\otimes$ is commutative and the local network has ``fat
links,'' i.e., all local links have capacity at least $s$.
%where $s=|S_i|$ for every node $i$.
For this
special but important case, we show how to complete the task in
time larger than the optimum by an $O(\log^2n)$ factor.
% that works in
% $O(Z_{\max}\log^2 n)$ rounds, where $Z_{\max}$ is the maximal timespan
% of cloud clusters (cf.\ \defref{def:intervals2} and \theoremref{thm-aw-ub}),
% in case that $\otimes$ is commutative, for graphs in which all local links are sufficiently
% large to send an entire message of size $s$ (see \defref{def:locally-wide}).



\subsection{Combining in General Graphs}
\label{sec-ccw-flow}
%%%%%%%%%%%%%%%%%%%%%%%%%%%

We now present algorithms for \CCW %for any combining operator $\otimes$, 
and for \CCR on general graphs, using
the primitives constructed in \sectionref{sec:rw} and \appref{app:multiple}. For combining, we consider a general
associative operator. Note that with a
non-commutative operator, the operands must be ordered; we assume
w.l.o.g.\ that in such cases
the nodes are indexed by the same order of their operands.

% \boaz{to the end of this \dsection or to wheel section}
% For example, in any instance of the uniform wheel model,
% \CCW requires $\Omega(s/b_c)$ time, since there are
% $n\cdot s$ bits of input that need to cross the cloud-links cut that
% has $n\cdot \bc$ bandwidth altogether.  However, if the links are fat
% (i.e., $\bl\ge s$), \CCW can solved in  $O(\sqrt{s/b_c})$ rounds.





\begin{theorem}
	\label{thm-ccw-gen}
	%Given a \CWC system, % $G=(V,E,w)$,
	Let $T_s$ be the running time  of \CAW (and \CAR)
	for input size $s_i=s$ for all processing nodes $i$.  Then \algref{alg:caw-flow} solves \CCW 
	in $O(T_s \log{n})$ rounds.
\end{theorem}


\ignore{%%%%  moving the figure to the appendix
\begin{figure}[t]
	%\small
  \begin{center}
    \begin{tikzpicture}[scale=0.8]
      \node [draw]{$X_0^3$} [level distance=10mm,sibling distance=50mm]
      child {
        node [draw]{$X_0^2$} [level distance=10mm ,sibling distance=25mm]
        child {
          node [draw] {$X_0^1$} [level distance=10mm ,sibling distance=12mm]
          child {node [draw] {$X_0^0$}}
          child {node [draw]{$X_1^0$}}
        }
        child {
          node [draw]{$X_2^1$} [level distance=10mm ,sibling distance=12mm]
          child {node [draw] {$X_2^0$}}
          child {node [draw] {$X_3^0$}}
        }
      }
      child {
        node [draw]{$X_4^2$} [level distance=10mm ,sibling distance=25mm]
        child {
          node [draw] {$X_4^1$} [level distance=10mm ,sibling distance=12mm]
          child {node [draw] {$X_4^0$}}
          child {node [draw]{$X_5^0$}}
        }
        child {
          node [draw]{$X_6^1$} [level distance=10mm ,sibling distance=12mm]
          child {node [draw] {$X_6^0$}}
          child {node [draw] {$X_7^0$}}
        }
      };
    \end{tikzpicture}
  \end{center}
  \caption{\em Computation tree  with $n=8$.
    $X_i^j$ denotes the result stored in node $i$ in iteration $j$.}
  \label{fig-tree}
\end{figure}
}%%%%%%%%


\begin{algorithm}[t]%\small
  \caption{High-level algorithm for \CCW using \CAW and \CAR}
  \label{alg:caw-flow}
  \begin{algorithmic}[1]
    \STATE $m := n$, $j := 0$
    \STATE for all $i<n$ set $X_i^0=S_i$, and for all $i > n$, $X_i^0=\Unit$
    \WHILE {$m > 1$} \label{alg:caw-flow:loop}
    \STATE run \CAW with inputs $S_i=X_i^j$
    \label{alg:caw-flow:caw}
    \STATE run \CAR with inputs $S_i=X_{2i}^j$
    \STATE run \CAR with inputs $S_i=X_{2i+1}^j$
    \STATE $m := \ceil{m/2}$ \label{alg:caw-flow:advance}
    \STATE for all $i<m$ set $X_i^{j+1}=X_{2i}^j \otimes X_{2i+1}^j$,
    and for all $i>m$, $X_i^{j+1}=\Unit$
    \STATE for all $i < m$, in parallel, node $i$ calculates $X_i^{j+1}$ locally
    \STATE $j := j+1$
    \ENDWHILE
    \STATE run \CW from node $0$ to write $X_0^j$ to the cloud
    \label{alg:caw-flow:last-caw}
  \end{algorithmic}
\end{algorithm}



\ignore{In \CCR there is a single $s$-bit input file $S$ stored in the
cloud, and the goal is to disseminate it to all processing nodes.}
In a way, \CCR is the ``reverse'' problem of \CCW, since it starts
with $s$ bits in the cloud and ends with $s$ bits of output
in every node. However, \CCR is easier than \CCW because our model allows for
concurrent reads and disallows concurrent writes.
We have the following result.
% in \CAW there are many possible operators to merge
% two $s$-bit operands, whereas in \CCR we split one $s$-bit operands in
% two $s$-bit results just by replication.


\begin{theorem}
	\label{thm-ccr-gen}
	Let $T_s$ be the time required to solve \CAR %on graph $G=(V,E)$ 
	with
	all input sizes $s_i=s$.  Then \CCR can be solved in $T_s$ rounds as
	well. %\boaz{why not the time of \CR?}
\end{theorem}







%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cwc"
%%% End:


==> old/combiningwheel.tex <==

\section{Multiple Cloud-Read/Writes With Combining}
\label{OLD:sec:va}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section we consider the task of \CCW, in which each node
$i$ has an input $S_i$ of size $s$ bits, and the requirement is to write the combined
value $\bigotimes_{i=0}^{n-1}S_i$ to the cloud, for some given associative
operator $\otimes$ that takes two $s$-bits operands and returns an
$s$-bits result.
Somewhat abusing terminology,  we call the operation of applying $\otimes$
\emph{multiplication}, and the result of $S_1\otimes S_2$ the
\emph{product} of $S_1$ by $S_2$. We assume the existence of a unit
element for $\otimes$, denoted $\Unit$, such that $\Unit\otimes
S=S\otimes\Unit=S$ for all $s$-bits strings $S$. We note that $\otimes$ need not be
commutative.

Our main result in this section is an algorithm for \CCW that works in
$O(Z_{\max}\log n)$ rounds, where $Z_{\max}$ is the maximal timespan
of cloud intervals (cf.\ \defref{def:intervals2} and \theoremref{thm-aw-ub}). We note that by using
standard methods \cite{LadnerF-80}, the algorithm can be extended to
compute, with the same asymptotic time complexity, all prefix sums,
i.e., compute, for each $0\le j<n$, $\bigotimes_{i=0}^jS_i$.

We distinguish between \emph{holistic} and
\emph{modular} combining operators, defined as follows.
In holistic combining,
no part of the product can be computed without both operands being
% the product can be computed only when both operands are
known in the entirety.
This is the case, for example, with matrix
multiplication. In modular combining, one can apply the combining
operator to aligned, equal-length parts of operands to get the output
corresponding to that part. For example, this is the case with vector
(or matrix) addition: to compute any entry in the sum, all that is
needed is the corresponding entries in the summands. It turns out that
in the modular case, a logarithmic factor can be shaved off the
running time (\theoremref{thm-aw-modular}).


In \sectionref{sec-aw-upper} we present our algorithm for \CCW. In
\sectionref{sec-aw-pipeline}, we explain how to speed up the algorithm
in the case of modular combining.






\subsection{\CCW}
\label{OLD:sec-aw-upper}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ignore{%%%%%%%%%%
Our algorithm and analysis of \CCW use the
interval-related concepts from \sectionref{sec:rw}.
Before we state the upper bound, we introduce notations regarding
multiple cloud intervals  (cf.~\defref{def-Ii}).
Unlike \sectionref{sec:rw}, the
definitions are not limited solely for right-intervals or left-intervals,
but rather they are defined for the ``best'' (i.e., with the smaller timespan) one-sided interval of each node,
i.e. the one-sided interval for which the upper bound was minimal
in \defref{def-Ii-2-sided}.
}%%%%%%%%

We assume the interval-related definitions from \sectionref{sec:rw}.

\begin{definition}\label{OLD:def:intervals2}
  Given an $n$-node wheel, let  $\IR{i}$ be the  cloud interval of $i$
  with the smaller timespan (cf.\ \defref{def-Ii}).
  We define $j_{\max} = \argmax_i\Set{|\IR{i}|}$,
  $j_c = \argmin_i \Set{\bC{\IR{i}}}$, and
  $j_\ell = \argmin_i \Set{\bLminR{i}}$.
  Finally, we define
  $Z_{\max} = {|\IR{j_{\max}}| + \frac{s}{\bLminR{j_\ell}} +
\frac{s}{\bC{\IR{j_c}}} }$.
\end{definition}
In words: $j_{\max}$ is the node with the longest cloud interval,
$j_c$ is the node whose cloud interval has the least cloud bandwidth, and
$j_\ell$ is the node whose cloud interval has the narrowest bottleneck.

% \begin{corollary}
% 	The upper bound presented in \theoremref{thm-aw-ub} is optimal up to a log factor.
% \end{corollary}



\noindent
We now turn to the upper bound.


\begin{theorem}\label{OLD:thm-aw-ub}
  % Let $Z_{\max} = {|\IR{j_{\max}}| + \dfrac{s}{\bLminR{j_\ell}} +
  %   \dfrac{s}{\bC{\IR{j_c}}} }$. Then
  \CCW can be solved in
  $O(Z_{\max}\log n)$ rounds.
%   If $\otimes$ allows for modular combining,
% then \CCW can be solved in $O(Z_{\max}+\log n)$ rounds.
\end{theorem}
\begin{figure}[t]
\small
\begin{center}
\begin{tikzpicture}
  \node [draw]{$S_0^7$} [level distance=10mm,sibling distance=50mm]
  child { node [draw]{$S_0^3$} [level distance=10mm ,sibling distance=25mm]
    child {node [draw] {$S_0^1$} [level distance=10mm ,sibling distance=12mm]
      child {node [draw] {$S_0^0$}}
      child {node [draw]{$S_1^1$}}}
    child {node [draw]{$S_2^3$} [level distance=10mm ,sibling distance=12mm]
      child {node [draw] {$S_2^2$}}
      child {node [draw] {$S_3^3$}}}
  }
  child { node [draw]{$S_4^7$} [level distance=10mm ,sibling distance=25mm]
    child {node [draw] {$S_4^5$} [level distance=10mm ,sibling distance=12mm]
      child {node [draw] {$S_4^4$}}
      child {node [draw]{$S_5^5$}}}
    child {node [draw]{$S_6^7$} [level distance=10mm ,sibling distance=12mm]
      child {node [draw] {$S_6^6$}}
      child {node [draw] {$S_7^7$}}}
  };
\end{tikzpicture}
\end{center}
\caption{\em Computation tree example, with $n=8$.
	$S_i^j$ denotes $\bigotimes_{k=i}^jS_k$.}
\label{OLD:fig-tree}
\end{figure}

The basic strategy to solve \CCW is to construct a virtual
multiplication tree inductively as follows (see \figref{fig-tree}).
Let $S_i^j$ denote the product of $S_i,\ldots,S_j$, and assume for now
that $n$ and all interval lengths are powers of $2$.  The individual
inputs are at the leaves of a complete binary tree, and given two
children holding $S_i^k$ and $S_{k+1}^j$, their parent node holds
$S_i^j=S_i^k\otimes S_{k+1}^j$. The algorithm computes the tree layer
by layer in a bottom-up fashion, and terminates when the root is
computed.  % This idea is rather standard; the novelty is in the
% implementation.
We use two different methods to compute internal nodes:
In the lower levels of the tree  we compute
the combined values of some cloud intervals without using the cloud,
and then we compute the higher levels nodes using \CR and \CW.


A  high-level
description is given in \algref{alg:aw-hi}.
The algorithm consists of a preprocessing part (lines
\ref{aw-1}--\ref{aw-3}), and the runtime part. The preprocessing part
produces a plan (schedule) for the actual execution. 
% Note that the intervals used in the lower levels
% should have as little overlap as possible because the local link
% bandwidth is limited: to this end, in steps \ref{aw-1}--\ref{aw-3} of the
% algorithm, which are executed off-line in preprocessing,
% we choose a \emph{cover} from all
% possible cloud intervals. We first explain these steps, and then
% explain how are the runtime steps (\ref{aw-colors}--\ref{aw5}) implemented.






% , whose We elaborate next.
% in a centralized approach, and the algorithm would assume that each vector knows in which intervals it is.




\subsubsection{Preprocessing}
\label{OLD:sec:prep}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In line \ref{aw-1}, the cloud intervals of all nodes are computed
according to \defref{def-Ii}.  Clearly
computing the intervals can be done in polynomial time.  From these
intervals, in line \ref{aw-2} we select a cover $C$ such that every
node is a member of either one or two intervals of $C$.  It is
straightforward to find such a cover, say, by a greedy
algorithm. Concretely, a cover with a minimal \emph{number of intervals} is
found by the algorithm in \cite{min-circle-cover} (in $O(n\log n)$
sequential time). The covers produced by \cite{min-circle-cover}  are sufficient
for line \ref{aw-2} of our algorithm, as the following lemma states.
\begin{lemma}
  \label{OLD:lem-coverload}
  Let $\mathcal I$ be a collection of intervals and denote
  $U=\bigcup_{I\in\mathcal I}I$.  Let $C\subseteq\mathcal I$
  be a minimal-cardinality cover of $U$, and let $\textrm{load}(i)=
  |\{I\in C : I\ni i\}|$. Then for all
  $i\in U$, $1\le \textrm{load}(i)\le 2$.
\end{lemma}
\Proof Clearly $\textrm{load}(i)\ge1$ for all $i\in U$ since $C$ is
a cover of $U$. For the upper bound, first note that by
the minimality of $|C|$, there are no intervals $I,I'\in
C$ such that $I\subseteq I'$,  because in this case $I$ could have
been discarded. This implies that the right-endpoints of intervals in $C$
are all distinct, as well as the left-endpoints.
Now, assume for 
contradiction, that there exist three intervals
$I,I',I''\in C$ such that $I\cap I'\cap I''\ne\emptyset$
(i.e., there is at least one node which is a member of each of the three).
Then $I\cup I'\cup I''$ is a contiguous interval.
Let $l=\min(I\cup I'\cup I'')$ and $r=\max(I\cup I'\cup I'')$.%
\footnote{
  The notation $\max(I)$ for an interval $I$ refers to the
  clockwise-end node of the interval.
  }
By counting, one of the three intervals, say  $I$,
has no endpoint in $\Set{l,r}$. But this means
that $I\subseteq I'\cup I''$, i.e., 
we can discard $I$, in contradiction to the minimality of $|C|$.
\QED
\begin{corollary}\label{OLD:cor-intersect}
  Any interval in $C$ intersects at most two other intervals in $C$.
\end{corollary}
In line \ref{aw-3}, the algorithm  partitions the cover to $3$ subsets.
\begin{lemma}
  \label{OLD:lem-3col}
   $C$ can be partitioned into three subsets such that the
  intervals within a subset are pairwise disjoint.
\end{lemma}
\Proof Consider a graph $G_C$
whose nodes are the intervals in $C$, and
there is an edge connecting any two nodes whose corresponding
intervals intersect. By \corollaryref{cor-intersect},
each interval in $C$ 
intersects at most two other intervals in $C$, the maximum degree in
$G_C$ is 2, and therefore the nodes of $G_C$ can be colored by 3
colors. Since there is no edge connecting two nodes of the same color,
we obtain the desired partition by defining $C_l$, for $l=1,2,3$, to be the
set of all intervals whose corresponding nodes in $G_C$ are colored
$l$.
\QED

\begin{algorithm}[t]%[H]\small
  \caption{High-level algorithm for \CCW}
  \label{OLD:alg:aw-hi}
  \begin{algorithmic}[1]
    \STATE For each processing node $i$: Compute its cloud interval $I_i$.
    \label{OLD:aw-1} 
    \STATE\label{OLD:aw-2} Compute a set of intervals $C\subseteq\Set{I_1, \ldots, I_n}$
    such that $C$ covers the ring i.e., $\bigcup_{I\in C}I=\Set{0,\ldots,n-1}$ and such that no
    node is a member of more than two intervals of $C$.
    \STATE\label{OLD:aw-3} Partition $C=C_1\cup C_2\cup C_3$, such that the intervals
    in each subset $C_i$ are pairwise disjoint.
    \FOR{$l:=1$ \textbf{to} 3 (sequentially) }
    \label{OLD:aw-colors}
    \FORALL{$I\in C_l$, in parallel}
    \STATE\label{OLD:aw-4}{compute $P_I=\bigotimes_{j\in I}S_j$
      using local links
      \hfill$\rhd$~\textit{
      the input of each node is combined exactly once in all $3$ iterations
    %   nodes in two intervals are combined once
      }
      }
    \ENDFOR
    \ENDFOR
    \label{OLD:aw-endloop}
    \STATE\label{OLD:aw5} Compute the result $\bigotimes_{I\in C}P_I$ using
    \algref{alg:aw-node}
  \end{algorithmic}
\end{algorithm}    

% As input, we have a set of intervals $S$, such that $S$ is a cover
% of $\Set{1,\ldots,n}$, and such that every node $i$ may be in two
% intervals of $S$ at most. The goal is to find a partition of $S$ to
% $3$ subsets $S_1, S_2, S_3$ such that each subset is pairwise
% disjoint.  More formally, we require that $S_1\cup S_2 \cup S_3 = S$
% and that for every subset $S_i$,
% $\forall_{I,J\in S_i} I\cap J = \emptyset$.

% One can easily see, that each interval $I\in S$ may intersect with
% $2$ intervals in $S$, at most.  We can build a graph $G=(V,E)$, in
% which the nodes are the intervals in $S$ and there is an edge
% connecting every two intersecting intervals, i.e. $V=S$,
% $E=\{(I, J) \mid I\cap J \ne \emptyset\}$.

% As mentioned, each interval in $S$ may intersect with $2$ intervals
% at most, and thus the maximal degree in $G$ is at most
% $\Delta(G) \le 2$. Using a greedy coloring algorithm on graph $G$,
% we can color the vertices of $G$ with $3$ colors. Taking
% $S_1, S_2, S_3$ as the subsets of each color of the coloring, would
% yield the desired partition.

% \textbf{TODO1: find a reference for the greedy coloring?}

% \textbf{TODO2: add some figures?}



\subsubsection{Low levels: Combining within a single interval}
\label{OLD:ssec-inetrval-combining}
We now explain how to implement line \ref{aw-4} of
\algref{alg:aw-hi}. Essentially, we build a computation tree within
each interval $I\in C$.
Before we explain the tree computation, we make, w.l.o.g., two simplifying
assumptions.


First, we require %assume
%\yehuda{why is this an assumption?}\gal{because it will not be the case for nodes that are in two intervals, but we show how we can make this assumption work}\yehuda{so what?  still why is this an assumption}
that each input $S_i$ is associated with a single
interval in $C$. To this end, we use the rule that if a node $i$ is a member
in two intervals 
$I$ and $I'$,
then its input $S_i$ is associated with the interval $I$ satisfying
$\max(I)<\max(I')$, and a unit input $\Unit$ is associated with $i$ in
the  context of $I'$, where $\Unit$ is  the unit (neutral) operand for
$\otimes$.
Intuitively, this rule means that the overlapping regions in an
interval are associated with the ``left'' (counterclockwise) interval.
% Furthermore, in order to compute \CCW with a non-commutative operator, 
% we need to have an interval that starts with node $0$. If this is not the case in $C$, we break the interval $I$ that contains $S_0$ in two $I=I_L\cup I_R$, where 
% $I_L$ is the part up to node $n-1$,  and $I_R$ is the part that starts with $0$.


% associate each node with a single interval: if a node $i$ is a
% member of two intervals, we associate$ S_i$ with the interval with the
% smaller leftpoint. In the other interval, we use a dummy value $S'_i$
% such that $S'_i\otimes S=S$ for any value $S$.

Second, we assume that the interval size, and therefore the number
of leaves in its computation tree, is a power of $2$. Otherwise, let
$p=2^{\ceil{\log|I|}}$ (i.e., $p$ is $|I|$ rounded 
up to the next power of $2$). When doing tree computation over an interval
$I$, we extend it (virtually) to a complete binary tree with $p$
leaves, where all the leftmost $p-|I|$ leaves have the unit input
$\Unit$. These leaves are emulated by the leftmost node of $I$ (the
emulation is trivial).


Assume now that we wish to compute the combined value of an interval
$I$ whose length is a power of $2$.  Computation of the combined value
of interval $I$ whose length is a power of $2$ proceeds in {stages},
where each stage $\ell$ computes all level-$\ell$ products in
parallel.  The algorithm maintains the invariant that after $S_i^j$ is
computed, it is stored in node $j$ (by definition, for all
$0\le i< n$, $S_i^i$ is initially stored at node $i$).  The
computation of a stage is performed as follows.

Let $S_i^{j}=S_i^k\otimes S_{k+1}^j$ be a product we wish to compute
at level $\ell$, and let $S_i^k, S_{k+1}^j$ be the values held by its
children. Note that $k+1-i=j-k=2^{\ell-1}$.  The algorithm forwards
$S_{i}^k$ from node ${k}$ to node $j$, which multiplies it by (the
locally stored) $S_{k+1}^j$, thus computing $S_i^j$, which is stored
in node $j$ for the next level. This way, the number of communication
rounds is just the time required to forward $s$ bits from ${k}$ to
$j$. Using pipelining, this is done in
$j-k+{s\over\phi([k,j])}=2^{\ell-1}+{s\over\phi([k,j])} \le
2^{\ell-1}+{s\over\phi(I)}$
rounds,
%\footnote{\interval{k}{j} is contained within some cloud interval,
%	therefore its bottleneck can not exceed $\phi(I_{j_\ell})$.}
and hence the total time required to compute the product
of all inputs of any interval $I$ is at most
\begin{equation}
  \label{OLD:eq:aw4}
  \sum_{\ell=1}^{\ceil{\log|I|}}\left(2^{\ell-1}+{s\over\phi(I)} \right)
  ~\le~ 2\left(|I|+\log|I|\cdot{s\over\phi(I)}\right)~.
\end{equation}
%
We therefore have the following result.
\begin{lemma}\label{OLD:lem-lo}
  Steps \ref{aw-colors}--\ref{aw-endloop} % \ref{aw-4}
  of the algorithm terminate in
  $O\left(|I_{j_{\max}}|+\log|I_{j_{\max}}|\cdot{s\over\phi(I_{j_\ell})}\right)$
  rounds, with $P_I$ stored in the rightmost node of $I$ for each
  interval $I\in C$. 
\end{lemma}
\Proof
Correctness is obvious. For the complexity analysis,
consider iteration $l$ of the loop of Step
\ref{aw-colors}. In this iteration, only intervals from $C_l$ apply in
line \ref{aw-4}, and since they are disjoint, their executions are
independent.
By \Eqr{eq:aw4},   all intervals in $C_l$ complete line
\ref{aw-4} in
% $I$ from , we have by \defref{def:intervals2}
% that all intervals in $C_l$, and hence iteration $l$, complete in
at most
$O\left(|I_{j_{\max}}|+\log|I_{j_{\max}}|\cdot{s\over\phi(I_{j_\ell})}\right)$
rounds. Summing this bound over $l=1,2,3$, we conclude that the loop of
line \ref{aw-colors} completes after
$O\left(|I_{j_{\max}}|+\log|I_{j_{\max}}|\cdot{s\over\phi(I_{j_\ell})}\right)$
rounds.
\QED


% \boaz{distinguish holistic from pipelined}

% Consider an interval $I = \interval{L}{R}$. \algref{alg:aw-step6}
% computes the combined value $\bigotimes_{i\in I}S_i$ of all the inputs
% of nodes in $I$: it simply sends the input from $L$ toward $R$, 
% combining the inputs along the way, and then $R$ sends the result back 
% to all nodes in $I$.
% \begin{lemma}\label{OLD:lem-interval} Let $Y(I)=|I| + \dfrac{s}{\phi{I}}$.
% 	After $O(Y(I))$ rounds, 
% \algref{alg:aw-step6} terminates, and all nodes in $I$
% 	have $\bigotimes_{j\in I}S_j$  locally stored.
% \end{lemma}
% \Proof The correctness is obvious by induction on $|I|$. 
% The running time follows from For the 
% running time, note that
% by the partition of the
% cover, intervals running concurrently are disjoint, and therefore
% their executions do
% not interfere. Since the execution time of each interval $I$ is
%  $O\left(  \right)$ by
% \theoremref{theorem:one_sided_UB}, we have that each iteration of the 
% loopthe execution of 
% \algref{alg:aw-step6} is $O(\max\Set{Z_i\mid i\in V_p})=O(Z_{\max})$. 
% \QED


\subsubsection{High levels:  Combining using the cloud}
\label{OLD:VA:UB:disjoint-intervals-addition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}[t]%[H]\small
  \caption{Computing a high level tree-node $y$ with children
    $y_\ell,y_r$ by an interval $I\in C$ with leader $h(I)$}
  \label{OLD:alg:aw-node}
  \begin{algorithmic}[1]
    \IF {$y$ is not a leaf}

    \STATE $h(I)$ invokes \CR for $y_\ell$
%    \hfill$\rhd$~~\emph{if the left child is missing, $y_\ell:= \Unit$}
    \STATE $h(I)$ invokes \CR for $y_r$
%    \hfill$\rhd$~~\emph{if the right child is missing, $y_r:= \Unit$}
    \STATE $h(I)$ computes $y:=y_\ell\otimes y_r$
    \ENDIF
        \hfill$\rhd$~~\emph{if $y$ is a leaf its value is already stored at $h(I)$}
    \STATE $h(I)$ invokes $\CW$ for $y$
  \end{algorithmic}
\end{algorithm}    




We now explain how the algorithm implements line \ref{aw5}. The computation is complete within each interval of $C$ and proceeds to 
combine the partial results obtained for each interval. Again, this is
done by filling in the values of a computation tree defined over the intervals. Now the
leaves of the tree are
the combined values of the intervals of $C$, as computed in line
\ref{aw-4} of \algref{alg:aw-hi}. To fill in the values of other nodes
in the computation tree, we use the intervals of $C$: Each node in the
tree is assigned an interval which computes its value using the \CR and \CW
primitives, as described in \algref{alg:aw-node}.
Let $h(I)$, the rightmost node of an interval $I$, be the
\emph{leader} of the interval.


Specifically, we consider a binary tree %\yehuda{need to explain it is not a full binary tree. How is it constructed? 
% Also need to tell which $I \in C$ is the left most etc.}
with $|C|$ leaves, height $\ceil{\log |C|}$, where each non-leaf node
has exactly two children.  This is easily done by constructing a
complete binary tree with $2^{\ceil{\log|C|}}$ leaves, deleting the
rightmost $2^{\ceil{\log|C|}}-|C|$ leaves, and if $|C|$ is odd, then
we ``fold'' the rightmost leaf into its parent (that leaf is the only
child of that parent). 
%
%The leftmost $2^{\ceil{\log|C|}}-|C|$ leaves are
%dummy nodes.
Each node $y$ in the computation tree is associated with
an interval in $C$ called $\Int(y)$, and a value $\Val(y)$: the
processors in $\Int(y)$ are responsible to computing $\Val(y)$.
The assignment of intervals to tree nodes is done as follows.
Intervals are  assigned to leaves in
order: The leftmost leaf is associated with the interval that contains
node $0$, the second leaf from the left is associated with the next
interval clockwise etc.
For internal nodes, we assign the intervals arbitrarily except that we
ensure that no
interval is assigned to more than one internal node (this is possible
because in a tree where every node has two or no children, the number
of internal nodes is smaller than the number of leaves).
% All dummy leaves $x$ are associated with the leftmost interval in
% $C$. Formally, for a dummy $y$, we have $\Int(y)=I_{\min}$, where
% $I_{\min}$ is the interval containing the smallest endpoint in $C$.
% An internal node is associated with the interval associated
% with its right child. 


Having assigned intervals to tree nodes, the values are computed as
follows (see \algref{alg:aw-node}).
The value associated with a leaf $y_I$ corresponding to interval $I$ is
$\Val(y_I)=\bigotimes_{i\in I}S_i$, i.e., the
combined value of $I$, as computed in line \ref{aw-4}. This way, every
leaf $x$ has $\Val(x)$, stored in the leader of $\Int(x)$.
For an internal node $y$ 
with children $y'$ and $y''$,  the leader of
$\Int(y)$ obtains $\Val(y')$ and $\Val(y'')$ using \CR, computes
their product $\Val(y)=\Val(y')\otimes\Val(y'')$ and invokes $\CW$ to
write it to the cloud. %\yehuda{should it be written to $h(Iy)$}

The scheduling of the computations is done layer by layer, bottom up.
Using the coloring of the
intervals of $C$ from line \ref{aw-3}: in each level, we first compute
values of 
nodes $y$ with $\Int(y)\in C_1$, then values of nodes $y$ with
$\Int(y)\in C_2$ and then the  values of nodes $y$ with
$\Int(y)\in C_3$. With this strategy, we have the following result.

\begin{lemma}\label{OLD:lem-hi}
  The execution of line \ref{aw5} is completed in
  $O(\log|C| \cdot Z_{\max})$ rounds.
\end{lemma}
\Proof
Similarly to \lemmaref{lem-lo}, all the values of any level $\ell$ are
computed in $O(Z_{\max})$ rounds, because following \theoremref{theorem:two_sided_UB} and \theoremref{theorem:CR_UB} \CR and \CW are computed in
$O(Z_{\max})$ rounds each.
Since there are $\ceil{\log|C|}$ levels the result follows.
\QED

\theoremref{thm-aw-ub} follows from \lemmaref{lem-lo} and
\lemmaref{lem-hi}, noting that $|C|\le n$ and $|I_{j_{\max}}|\le n$.


We close this subsection with the lower bound.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{lemma}
	\label{OLD:lemma:AR-LB-i}
	Any algorithm for \CCW requires at least $\Omega(\ZR{i})$ rounds
	for every node $i$.
\end{lemma}

\Proof By reduction from $\CW_i$.
%in which $i$ has some message $S$ of size $s$ bits as its input,
%and the goal is to write this message to the cloud.
%
Given $S$, assign $S_i=S$ as the input of node $i$ in \CCW, and for every 
other node $j \ne i$, assign $S_j = \Unit$. Clearly, any algorithm for \CCW
that runs with these inputs, results with $S_i=S$ written to the cloud,
and thus solves $\CW_i$ with input $S$.
The lemma follows from \theoremref{theorem:two_sided_LB}. \QED

\begin{theorem}\label{OLD:thm-aw-lb}
	Any algorithm for \CCW requires 
	$\Omega(Z_{\max})$
	% $ = \Omega \left({|\IR{j_{\max}}| + {{s}\over{\bLminR{j_\ell}}}
	% 	+ {{s}\over{\bC{\IR{j_c}}}} }\right)$
	rounds. 
\end{theorem}

\Proof From \lemmaref{lemma:AR-LB-i}, $\Omega(Z_i)$ is a
lower bound for every node $i$, and recall that
$\ZR{i} = {|\IR{i}| + {{s}\over{\bLminR{i}}} + {{s}\over{\bC{\IR{i}}}}}$.
For index $j_{\max}$ we get a lower bound of
$\Omega(Z_{j_{\max}}) \in \Omega(|\IR{j_{\max}}|)$.
For index $j_\ell$ we get a lower bound of
$\Omega(Z_{j_N}) \in \Omega({{s}/{\bLminR{j_\ell}}})$.
For index $j_c$ we get a lower bound of
$\Omega(Z_{j_C}) \in \Omega\left( {s}/{\bC{\IR{j_c}} }\right)$.
%
Summing them all up, gives the desired lower bound. \QED

\paragraph{Remark: Non-commutative operators.}  In the case that
$\otimes$ is not commutative, the cover $C$ (computed in line \ref{aw-2} of
\algref{alg:aw-hi}) needs to be patched: In this case, we require that
the interval that contains node $0$ does not contain node $n-1$.
If this is not the case after computing the cover, let $I$ be an interval
that contains both. Partition $I$ 
in two subintervals $I=I_L \cup I_R$, where $I_L$ is the part up to
node $n-1$, and 
$I_R$ is the part that starts with node $0$. $I_L$ and $I_R$ replace
$I$ in the cover $C$ for all purposes, except work: any work assigned
to either 
$I_L$ or $I_R$ will be executed by all nodes of $I$. This may incur an
additional  constant slowdown due to multiplexing.


\subsection{Modular Combining}
\label{OLD:sec-aw-pipeline}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Intuitively, an operator is a modular combining operator if it can
be applied to aligned pieces of the operands and obtain the
corresponding piece of the result. For example, bit-wise operations
are modular, as is vector addition. Formally, we have the
following.
\begin{definition}
	\label{OLD:def:modular-op}
  An operator $\otimes:\Set{0,1}^s\times\Set{0,1}^s\to\Set{0,1}^s$  is
  called \emph{modular} if there exists a partition
  $s=g_1+g_2+\cdots+g_K$, and  $K$ operators
  $\otimes_i:\Set{0,1}^{g_i}\times\Set{0,1}^{g_i}\to\Set{0,1}^{g_i}$
  such that for any $x,y\in\Set{0,1}^s$, $x\otimes y$ is equal to the
  concatenation $(x_1\otimes_1y_1)(x_2\otimes_2 y_2)\cdots 
  (x_K\otimes_K y_K)$ with $x=x_1 x_2 \cdots x_K$, $y=y_1 y_2 \cdots y_K$ and
  $|x_i|=|y_i|=g_i$ for every $i$.
  The \emph{grain size
  of $\otimes$ in the given partition} is $\max\Set{g_i\mid 1\le i\le
    K}$, and the \emph{grain size of $\otimes$} is the minimal grain
  size of $\otimes$ over all partitions.
  %\yehuda{Dont you want $\min$ instead of $\max$ in the grain def}\gal{no, if there is a grain of size $1$ and a grain of size $s-1$, the latter would be more dominant} \yehuda{it does not work with the way it is used in the next pages}.
\end{definition}
Note that any $s$-bits binary operator is trivially modular with grain
size at most $s$. However, small grain size facilitates parallelism
and pipelining by applying the operation on small parts of the operands
independently. Note also that the grain size depends on the way we
break down the operands; the best breakdown is the one that minimizes
the grain size.
%
% Modular operators allow for applying their sub-operators in a
% pipelined fashion. 
In any case, given such a breakdown, we can use pipelining to
push the
logarithmic factor of \theoremref{thm-aw-ub} to the grain size, as the following theorem states.
\begin{theorem}\label{OLD:thm-aw-modular}
    Let $Z_{\max} = {|\IR{j_{\max}}| + {s}/{\bLminR{j_\ell}} +
    {s}/{\bC{\IR{j_c}}} }$, and suppose that $\otimes$ is modular with
  grain size $g$. Then \CCW can be solved in
  $O\left(Z_{\max}+|I_{j_{\max}}|\ceil{g\over\phi(I_{j_{\ell}})}+\ceil{g\over\bC{\IR{j_c}}}\log n\right)$ rounds.
\end{theorem}

\begin{corollary}
  In the uniform wheel topology with cloud bandwidth $\bc$ and local
  link bandwidth $\bl\ge\bc$, \CCW with an operation of
  grain size $g\le\bc$ can be executed in
  $O\left(\dfrac{s}{\bl}+\min\left(\sqrt{\dfrac{s}{\bc}},\dfrac{\bl}{\bc}\right)+\log n\right)$
  rounds.
\end{corollary}
%\boaz{fill in differences from holistic}

In the high level, modular combining is the same as holistic
combining, as presented in \algref{alg:aw-hi} (\algref{alg:aw-node} is
slightly modified). % \yehuda{and 4?}.
All of the preprocessing steps (\ref{aw-1}--\ref{aw-3}) and their
analysis from \sectionref{sec:prep} remain unchanged.  The
difference is in the implementation of the low level (\ref{aw-4}) and
the high level (\ref{aw5}) steps.

For a low level step, we note that the computation tree is no longer
necessary; thanks to the {modularity} of operator $\otimes$, a simple
one-pass procedure suffices.  For interval $I=\interval{\ell}{r}$, the
algorithm forwards $S_\ell$ from node $\ell$ through the local links
all the way to node $r$, and every node along the way combines the
grains it receives with its local corresponding grain,
and forwards the result grain as soon as it is computed.
% relevant chunk \yehuda{you have not yet mentioned chunks or chunk size !} of its input before passing it on.

More formally, let $i\ne \ell$ be some node in $I$.  Let
$x=S_\ell^{i-1}$ be the operand that $i$ should receive from node
$i-1$, and let $y=S_i$. We consider the partition of $x$ and $y$
according to the grains of $\otimes$ as described in
\defref{def:modular-op} %\yehuda{by the current definition $s$ is the
% size?!}\boaz{??}.
For every grain $x_j$ that $i$ fully receives, it
calculates locally the product $x_j \otimes_j y_j$ and proceeds to
send it immediately to node $i+1$.
\begin{lemma}\label{OLD:lem:pipe-lo}
  Let $\otimes$ be a modular operator with grain size $g$ as in
  \defref{def:modular-op}.% \yehuda{?}. 
  Using pipelining, line \ref{aw-4} of
  \algref{alg:aw-hi} can be computed in an interval $I$ in
  $O({s/\phi(I)}+\ceil{g/\phi(I)}\cdot|I|)$% \yehuda{why multiplying by I?}
  rounds.
\end{lemma}
\Proof
% The time to compute the first grain of the result, using pipelining,
% is $O(\ceil{g/\phi(I)}\cdot|I|)$. 
The number of messages required
to send all $s$ bits from a node $j$ to node $j+1$ is at most
$\ceil{s/\phi(I)}$. An intermediate node can compute the
result of a grain and start forwarding it to the next node after
$\ceil{g/\phi(I)}$ steps, since a complete grain is needed.
The lemma follows.
% Thus the
% overall time to compute all grains 
% is $O(|I|\cdot\ceil{g\over\phi(I)}+{s/\phi})$.
\QED

The pipelining strategy applies also to the tree nodes computed
in line \ref{aw5} of \algref{alg:aw-hi}. Specifically, we need to
change \algref{alg:aw-node} to work grain-by-grain as follows.
Suppose that interval $I$ is
in charge of filling in the value to a tree node $y$ with children
$y_\ell$ and $y_r$.
We assume that the order of reading and writing a string $S$ in \CR
and \CW is sequential, i.e., the first bits of $S$ are retrieved (or
written, resp.) first. We run, in parallel, \CR on $y_\ell$ and $y_r$,
and we also run \CW of $y$ in
parallel to them. We can implement this parallelization using multiplexing of the nodes of $I$, at the cost of a
constant factor slowdown: each node is taking part of only a constant number of
\CR and \CW actions concurrently.
%\yehuda{not clear. I did not understand}. 
As soon as a grain of $y_\ell$ and the corresponding grain of
$y_r$ are available, the leader of $I$
computes the corresponding grain of the result and writes it using
$\CW$. This way, computing a grain at a tree-node requires
$O(\ceil{g/\bc(I)|})$ rounds. Hence the first grain is computed at the
root after $O(\ceil{g/\bc(I)}\log n)$ rounds. In every round we can
send $\min(\bc(I),\phi(I))$ bits,
% fit at least $\bc(I)/g$ grains,
and hence the last grain is written
$O(Z_{\max})$ rounds later. %\yehuda{not clear enough.  how do we know
                            %the pipelining stages do not interfere
                            %with each other on different links?}
Thus we obtain the following result.
\begin{lemma}\label{OLD:lem:pipe-hi}
  Let $\otimes$ be a modular operator with grain size $g$ as in
  \defref{def:modular-op}. Using pipelining, line \ref{aw5} of
  \algref{alg:aw-hi} can be computed in 
  $O(Z_{\max}+\ceil{g\over\bc(I_{j_c})}\log n)$ rounds.
\end{lemma}


\theoremref{thm-aw-modular} follows from \lemmaref{lem:pipe-lo} and
\lemmaref{lem:pipe-hi}. 


\subsection{\CCR}
\label{OLD:sec:AR}
%%%%%%%%%%%%%%%%
In the \CCR operation, an $s$-bits string $S$, initially stored in the cloud node $v_c$, is
disseminated to all processing nodes. Recall that \CR allows a single
processing node to read a string from the cloud; to let all nodes obtain that
string, we use a cover of the intervals, as computed in lines
\ref{aw-1}--\ref{aw-3} of \algref{alg:aw-hi}. Let $C$ be that cover. The algorithm
implementing \CCR consists of an invocation of \CR in each interval of
$C$ by the interval leader, followed by disseminating the string
within each interval to all members. Clearly, the number of rounds
required to disseminate within a single interval $I$ is $O(Z_I)$ for the \CR operation,
and $O(|I|+s/\phi(I))$ rounds to disseminate $S$ throughout $I$. Using
the limited overlap of intervals in $C$ and \defref{def:intervals2},
similarly to the proof of \lemmaref{lem-lo}, we obtain the following
result.
\begin{theorem}\label{OLD:thm-AR}
	\CCR can be performed in
	$O(Z_{\max})$ rounds.
\end{theorem}

In addition, since any algorithm that solves the \CCR problem would also solve the \CR problem for every node $i$, we get from \theoremref{theorem:CR_LB} the following result.

\begin{theorem}\label{OLD:thm-AR-LB}
	Any algorithm solving \CCR requires
	$\Omega(Z_{\max})$ rounds.
\end{theorem}





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cwc"
%%% End:


==> old/conc.tex <==

\section{Conclusion and Open Problems}
\label{sec:conc}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this paper we have introduced  a new model that incorporates cloud
storage with a bandwidth-constrained communication network. We have developed
a few building blocks in this model, and
used these primitives to obtain effective  solutions to some
real-life distributed applications.
There are many possible directions for future work; below, we mention a few.
%
% demonstrates the power
% that can be achieved by using cloud storage that is common among different
% processing nodes. We considered a basic form of this model,
% the \emph{wheel} model, and proved lower and upper bounds for some basic problems,
% and demonstrated how to use these as primitives for different applications
% on said model. As is the case with new models, we believe that there are still
% many problems and variations to explore, of what can be achieved in the \CWC model,
% some of which are presented here as open problems.

One interesting direction is to validate the model with
\emph{simulations and/or implementations} of the algorithms, e.g., implementing the
federated learning algorithm suggested here.

A few algorithmic question are left open by this paper.
For example, can we get good approximation ratio for the problem of combining in a general (directed, capacitated) network? Our approximations dealt only with the cases of fat links and the wheel.
%extend our wheel-topology algorithms to \emph{more
%general families of graphs}. We think that some of the basic ideas in
%our algorithms apply in general as well
% \yehuda{a bit empty sentence.  why do you believe so? we should be
%more concrete}.\boaz{it's kinda standard :(}

Another interesting issue %to consider 
is the case of \emph{multiple cloud
nodes}: How can nodes use them effectively, e.g., in combining?
Possibly in this case one
should also be concerned with privacy considerations.

% Another direction is a potentially harder generalization to \emph{directed graphs}:
% Either considering links that can carry information only in one direction, or links whose bandwidth is not symmetric,
% i.e. either the upload and download speeds to and from the cloud are not the same, or the local links are asymmetric.

Finally, an important direction to explore is \emph{fault
  tolerance}: Practically, clouds are considered highly reliable.
%\yehuda{what does "extremely reliable" mean. }\boaz{seven nines? it's
%not important}.
How should we exploit this fact to build more robust systems? and on the other
hand, how can we build systems that can cope with varying cloud
latency?

% Another native expansion, is to consider these and similar tasks on different topologies,
% as opposed to this paper
% in which we have only discussed the wheel topology.
% An interesting observation for the \emph{uniform clique} topology ($n$ nodes,
% all connected to each other with link with a $\bl$ bandwidth, and all are
% connected to a cloud node $v_c$ with links with a $\bc$ bandwidth),
% is that either all network links, or all cloud links, can be discarded completely
% while slowing down the system only by a constant factor, depending on $\bc$ and $\bl$.
% If $\bc \ge n\bl$, then all local links can be simulated by writing all local messages
% to the cloud, and then having them read by their destination node.
% If $\bc \le n\bl$, then the cloud can be simulated by sending each messages
% to different nodes in chunks of size $\bl$, and then receiving the
% desired information from the nodes that got them through the local links.






%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cwc"
%%% End:


==> old/dynamic.tex <==
\section{Implementation of Basic Communication Primitives in \CWC}
\label{app:multiple}
\subsection{Dynamic Flows}
\label{ssec:dynamic}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 The concept of \emph{quickest flow}~\cite{quickest}, a variant
of \emph{dynamic flow}~\cite{Skutella-flows}, is defined as follows.%
\footnote{
	We adapt the original definition to our context by setting all transmission
	times to $1$.
}
A \emph{flow network} consists of a directed weighted graph
$G=(V,E,c)$ where 
$c:E\to\mathbb{N}$, with a distinguished source and sink nodes,
denoted $s,t\in V$, respectively. 
A \emph{dynamic flow} with \emph{time horizon} $T\in\mathbb{N}$
and \emph{flow value} $F$
is a mapping
$f:E\times[1,T]\to \mathbb{N}$ that specifies for each edge $e$ and
time step $j$, how much flow $e$ carries between steps $j-1$
and $j$,  subject to the natural constraints:
\begin{compactitem}
\item Edge capacities. For all $e\in E, j\in[1,T]$:
  \begin{equation}
    f(e,j)\le~c(e)\label{const-edge}
  \end{equation}
\item Only arriving flow can leave. For all $ v\in V\setminus\Set{s},
  j\in[1,T-1]$: 
  \begin{equation}
    \sum_{i=1}^{j}\sum_{(u,v)\in E}\!\!f((u,v),i)
  \,\ge  \sum_{i=1}^{j+1}\sum_{(v,w)\in E}\!\!f((v,w),i)
    \label{const-node}\\
  \end{equation}
\item No leftover flow. For all $v\in V\setminus\Set{s,t} $:
  \begin{equation}
    \sum_{j=1}^{T}\sum_{(u,v)\in E}\!\!f((u,v),j)
    \,=  %\!\!
   \sum_{j=1}^{T}\sum_{(v,w)\in E}\!\!f((v,w),j) \label{const-node-end}
  \end{equation}
\item Flow value---source.
  \begin{equation}
  \sum_{j=1}^T\left(\sum_{(s,v)\in E}\!\!f((s,v),j)
         \!\!\,\right.\left.-\!\!
   \sum_{(u,s)\in E}\!\!f((u,s),j)\right)
   =F\label{const-source}
  \end{equation}
\item Flow value---sink.
  \begin{equation}
    \sum_{j=1}^T\left(\sum_{(t,v)\in E}\!\!f((t,v),j)
      \!\!\,\right.\left.-\!\!\sum_{(u,t)\in E}\!\!f((u,t),j)\right)
  =-F   \label{const-sink}
  \end{equation}
\end{compactitem}
%Constraint \ref{const-edge} imposes edge capacities.
% Constraint \ref{const-node} says that 
% Constraint \ref{const-node-end} guarantees that no flow is left in any
% of the non-sink, non-source nodes after $T$ steps.
% Constraints \ref{const-source}-\ref{const-sink} complete the
% picture, saying that in total, $F$ units of flow are shipped from $s$
% to $t$ in the time interval $[1,T]$.

In the usual flavor of dynamic
flows, $T$ is given and the goal is to maximize $F$. In the quickest
flow variant, the roles are reversed.

\begin{definition}
	Given a flow  network,
	the \textbf{quickest flow} for a given value $F$ is a dynamic flow
	$f$ satisfying (\ref{const-edge}-\ref{const-sink}) above with flow value $F$, such that the
	time horizon $T$ is minimal.
\end{definition}

\begin{theorem}[\cite{quickest}]
	\label{thm-quickest}
	The quickest flow problem can be found in strongly polynomial time.
\end{theorem}


Another related problem that we make use of, is the \emph{evacuation problem}
\cite{evacuation-problems}, specifically the case of a single sink node
\cite{Skutella-multiple-sources}.
In this problem,
each node $v$ has an initial amount of $F(v)$ flow units, and the goal is to transmit
all the flow units to the sink in the minimum amount of time.
Each node $v$ with a non-zero $F(v)$ is considered a source.
Similarly to the single source case, a \emph{dynamic flow} of \emph{multiple sources}
with \emph{time horizon} $T\in\mathbb{N}$ is a mapping
$f:E\times[1,T]\to \mathbb{N}$, subject to the edge capacity
constraints (\Eqr{const-edge}), and the following modified constraints:
\begin{compactitem}
\item Only initial and arriving flow can leave.  For all $ v\in V, j\in[1,T-1]$:
  \begin{equation}
    F(v)+\sum_{i=1}^{j}\sum_{(u,v)\in E}\!\!f((u,v),i)
    \,\ge
    \sum_{i=1}^{j+1}\sum_{(v,w)\in E}\!\!f((v,w),i)
	\label{const-mul-node}
  \end{equation}
\item Flow value---all sources. For all $v\in V$:
  \begin{equation}
	\sum_{j=1}^T\left(\sum_{(v,w)\in E}\!\!f((v,w),j)
	-\!\!
	\sum_{(u,v)\in E}\!\!f((u,v),j)\right)
	=F(v)
	\label{const-mul-source}
  \end{equation}
\item Flow value---sinks.
  \begin{equation}
	\sum_{j=1}^T\left(\sum_{(u,t)\in E}\!\!f((u,t),j)
	-\!\!
	\sum_{(t,w)\in E}\!\!f((t,w),j)
	\right)=
	\sum_{v\in V}{F(v)}
	\label{const-mul-sink}
  \end{equation}
\end{compactitem}
% Similarly to the single source case,
% %Constraint \ref{const-mul-edge} imposes edge capacities.
% Constraint \ref{const-mul-node} says that all flow that leaves 
% a node $v$ up to step $j+1$ does not exceed the initial amount of flow of $v$
% and the flow that arrived at $v$ up to step $j$, combined.
% %Constraint \ref{const-node-end} guarantees that no flow is left in any
% %of the non-sink, non-source nodes after $T$ steps.
% Constraint \ref{const-mul-source}
% says that in total, $F(v)$ units of flow are shipped from node $v$
% in the time interval $[1,T]$.
% Constraint \ref{const-mul-sink} completes the
% picture, saying that in total,
% the amount of flow units that arrive at the sink $t$ in the time interval $[1,T]$
% is exactly the total amount of flow units that are initially stored in all the nodes
% altogether.


\begin{definition} \label{def-evacuation}
	Given a flow  network in which each node $v$ has value $F(v)$,
	%	and a sink node $t$,
	a solution to the evacuation problem is a dynamic flow of multiple sources $f$
	satisfying (\ref{const-edge}) and (\ref{const-mul-node}-\ref{const-mul-sink}), such that the
	time horizon $T$ is minimal.
	%	of time horizon $T$ such that each node $v$ initially has $F(v)$ flow units,
	%	and after $T$ time steps node $t$ has all $\sum_{v\in V}{F(v)}$ flow units,
	%	such that $T$ is minimized.
	%	$f$ needs to satisfy the dynamic flow constraints (\ref{const-edge}-\ref{const-sink}),
	%	under some trivial modifications to allow for multiple sources.
\end{definition}


\begin{theorem}[\cite{Skutella-multiple-sources}]
	\label{thm-evacuation}
	The evacuation problem can be found in strongly polynomial time.
\end{theorem}

\subsection{Using Dynamic Flows in \CWC}

In this \dsection we give optimal implementations of  basic cloud access
primitives that serve as building blocks in more complex tasks. These are
the tasks of reading and writing to or from the cloud, invoked by a
single node (\CW and \CR), or by all nodes (\CAW
and \CAR). Our goal is to find the best \emph{schedules}
(cf.~\defref{def-sched}) by pooling the cloud bandwidth of the nodes.
We  present optimal solutions to these problems in general directed
graphs, using the quickest flow algorithm.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%	
\para{Serving a Single Node:}
%\label{ssec:dynamic-flow}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ignore{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	The dynamic flow problem~\cite{Skutella-flows, Ahuja-Flows} is a
	generalization  of the maximum flow
	problem that dates back to Ford and
	Fulkerson \cite{Ford-Fulkerson}.  
	\QstF \cite{Minieka-flow, Wilkinson-flow} is a variant of dynamic
	flow. In this problem 
	there is a graph $G=(V,E)$ with source node $s\in V$ and a target node
	$t\in V$ with each edge $e$ having bandwidth $w(e)$ and traversal time
	$t(e)$.  The goal is to send a given amount of flow units from $s$ to
	$t$ through the network of $G$ in a minimal amount of rounds, without
	exceeding the bandwidth limitations of each edge and with the
	traversal of each edge $e$ requiring $t(e)$ rounds.
	
	The \QstF Problem can be solved using an algorithm for
	the Maximum Flow problem: for a given time estimate $T$, construct a layered graph
	$\FG{G}{T}$ of $T+1$ layers with each layer $i \in \interval{0}{T}$
	containing a copy of all nodes in $V$,
	$\left\{ (v, i) \mid v\in V \right\}$.
	For each node $v$ and layer $i\in \interval{0}{T-1}$, connect $(v,i)$ and $(v,i+1)$
	with a link of infinite bandwidth.
	For each link $e=(u,v)\in E$ and for each $i \in \interval{0}{T-t(e)}$, connect node
	$(u, i)$ to $(v, i+t(e))$ with a link of bandwidth $w(e)$.
	\todo{add a figure?}
}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let us consider \CW first.
We start with a lemma stating the close relation between schedules (\defref{def-sched})
implementing \CW
in our model and dynamic flows.

\begin{lemma}\label{lem:schedule-iff-dynamic}
	Let $G=(V,E,w)$ be a graph in the \CWC model.
	Then there is a schedule implementing $\CW_i$ from processing node $i$
	to cloud node $v_c$ with message $S$ of size $s$
	in $T$ rounds
	if and only if there is a dynamic flow of value $s$ and time horizon $T$ from source node $i$
	to sink node $v_c$.
\end{lemma}
\Proof
Converting a schedule to a dynamic flow is trivial,
as send and receive operations between processing nodes and \FW and \FR operations
directly translate to a dynamic flow that transports the same amount of flow
while maintaining bandwidth capacities and resulting with a desired dynamic flow.
For the other direction (converting a dynamic flow to a schedule),
let $f$ be a dynamic flow of time horizon $T$ and value $s$ from node $i$ to the cloud $v_c$.
We describe a schedule $A$ implementing $\CW_i$
%(i.e., sends a message $S$ of size $s$ from $i$ to $v_c$)
as follows.

First, we construct another dynamic flow $f'$ which is the same as $f$,
except that no flow leaves the sink node $v_c$.
%\todo{explain why we can do that}
Formally, let $\val_g(v,t)$
%$\sum_{i=1}^{t}
%\sum_{(u,v)\in E}f((u,v),i) -
%\sum_{i=1}^{t}
%\sum_{(v,w)\in E}f((v,w),i)$
be the total number of flow units that are stored in node $v$ at time step $t\in\Set{0,T}$
according to some dynamic flow $g$.
Flow $f'$ is constructed by induction;
In time step $1$, $f'$ is the same as $f$, except for setting
$f'(e,1) = 0$ for every edge $e$ that leaves $v_c$.
Let $t\in \Set{1,T-1}$. In step $t+1$, $f'$ is defined the same as $f$,
while truncating the sum of all flow that leaves node $v$ to be at most $\val_{f'}(v,t)$
for every node $v$, and setting $f'(e,1) = 0$ for every edge $e$ that leaves the sink.

Let $G_p = G-\{v_c\}$, and let $\val_g(G_p, t)$  denote $\sum_{v\in V_p}\!\val_g(v,t)$
for some dynamic flow $g$.
 Initially, $\val_f(G_p, 0) = \val_{f'}(G_p, 0) = s$,
and that by the induction, in every step $t\in \Set{1,T}$,
%$f'(e,t) \le f(e,t)$ and thus
$\val_f(G_p, t) \ge \val_{f'}(G_p, t)$ due to flow units not being able to
get to $G_p$ from $v_c$.
Finally, in time step $T$, $\val_f(G_p, T) = 0$ since all flow was sent to the sink,
and thus $\val_{f'}(G_p, T) = 0$ as well
and $\val_{f'}(v_c,T) = s$ due to flow conservation.
Therefore, $f'$ is a dynamic flow of time horizon (at most) $T$ and value $s$.

Now, we use $f'$ to describe the volume of data that is sent along each link
in every round of the schedule $A$, by translating flow between processing
nodes to send/receive operations, and between processing and cloud nodes to \FW operations
(no \FR operations are required according to $f'$, because no flow leaves $v_c$).
To specify which data is sent in every operation of the schedule,
refer to all \FW operations of the schedule.
Let $K$ be the number of \FW operations in $A$, let $i_k$ be the node
initiating the $k$-th call to \FW and let $l_k$ be
the size of the message in that call.
We assign the data transferred on each link during $A$ so that
when node $i_k$ runs the $k$-th \FW, it would write the part of $S$
starting at index
$s\cdot{ \sum_{j=1}^{k-1}{l_j}} $
and extending for $l_k$ bits.
Note that processing nodes do not need to exchange indices of the data they transfer,
as all nodes can calculate in preprocess time the schedule and thus
``know in advance''
the designated indices of the transferred data.

Correctness of the schedule $A$ follows from the validity of $f$, as well as its 
time complexity.
\QED




\begin{theorem}
	[\theoremref{thm-cw}]
	Given any instance $G=(V,E,w)$ of the \CWC model, an optimal
	schedule realizing $\CW_i$ can be computed in polynomial time.
\end{theorem}
\Proof
Consider a $\CW$ issued by a
processing node $i$, wishing to write $s$ bits to cloud node $v_c$. We
construct an instance of quickest flow as follows.
The flow network is $G$ where $w$ is the link capacity function, node $i$
is the source and $v_c$ is the sink. The requested flow
value is $s$. The solution, computed by \theoremref{thm-quickest},  is directly translatable to a schedule,
after assigning index ranges to flow parts according to \lemmaref{lem:schedule-iff-dynamic}.
Optimality of the resulting schedule follows from the optimality of
the quickest flow algorithm.
\QED
\para{Remarks.}
\begin{compactitem}
	\item Interestingly, in the presence of multiple cloud
	nodes, it may be the case that while writing to one cloud
	node, another cloud node is used as a relay station.
	\item Schedule computation can be carried out
	off-line: we can compute a schedule for each node $i$ and for each
	required file size $s$ (maybe it suffices to consider only powers of $2$),
	so that in run-time,
	the initiating node would only need to tell all other nodes which schedule to use.
	\footnote{
		We note that sending the initiating messages can be problematic if it uses
		cloud nodes as relays, and may require some sort of synchronization across all
		processing nodes.
		%	such as a busy-loop wait on some file in the cloud.
	}
	%the schedule is sent along from the invoking
	%node.
	%\footnote{
	%  We note that sending the schedule may be problematic if it uses
	%  cloud nodes as relays.
	%  }
\end{compactitem}

\medskip\noindent
Finally, we observe that the reduction sketched in the proof of
\theoremref{thm-cw}  works for reading just as well: the only
difference is reversing the roles of source and sink, i.e.,
pushing $s$ flow units from the cloud node $v_c$ to the requesting
node $i$. We therefore have also:
\begin{theorem}
	[\theoremref{thm-cr}]
	Given any instance of the \CWC model, an optimal schedule realizing
	$\CR_i$ can be computed in polynomial time.
\end{theorem}



\para{Serving Multiple Nodes:}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Consider now operations with multiple invocations. Let us start with
$\CAW$ (\CAR is analogous, as mentioned above). Recall that in this
task, each node has a (possibly empty) file to write to a cloud
node. If all nodes write to 
the same cloud node, then using
the evacuation problem
%a (slightly modified)
variant of the
quickest flow algorithm solves the problem (see \defref{def-evacuation}),
%\footnote{
%In the quickest flow algorithm, a standard max-flow algorithm is used on a layered
%graph of $T$ layers. To allow for $n$ source nodes, an additional layer is added
%with a new source node connected to all of the desired source nodes in the first layer.
%}
However, if we need to
write to multiple cloud nodes, we resort to the quickest \emph{multicommodity}
flow, defined as follows~\cite{Skutella-flows}.

We are given a flow network as described in \subsectionref{ssec:dynamic},
but with $k$ source-sink pairs $\Set{(s_i,t_i)}_{i=1}^k$, and $k$
\emph{demands} $d_1,\ldots,d_k$. We seek $k$ flow functions $f_i$,
where $f_i$ describes the flow of $d_i$ units of commodity $i$ from
its source $s_i$ to its sink $t_i$, subject to the usual constraints:
the edge capacity constraints (\ref{const-edge}) applies to the sum of
all $k$ flows, and the node capacity constraints (\ref{const-node}-\ref{const-node-end}),
as well as the source and sink constraints
(\ref{const-source}-\ref{const-sink}) are written for each commodity
separately.

For the case that all nodes write to the same cloud node,
we can get the following theorem.
\begin{theorem}
	[\theoremref{thm-caw-car}]
	Given any instance $G=(V,E,w)$ of the \CWC model, an optimal
	schedule realizing \CAW (\CAR) in which every node $i$ needs to write (read) a message
	of size $s_i$ to (from) cloud node $v_c$ can be computed in strongly polynomial time.
\end{theorem}
\Proof
Similarly to \lemmaref{lem:schedule-iff-dynamic}, one can see that there is such an algorithm
for \CAW if and only if there is a dynamic flow solving the evacuation problem 
(\defref{def-evacuation}).
Thus in order to solve \CAW, we simply need to construct a flow network as is done
in \theoremref{thm-cw}, and apply \theoremref{thm-evacuation} in order to get the solution,
that can be then translated to a schedule.

A schedule for \CAR can be obtained by reversing the schedule for \CAW,
similarly to \theoremref{thm-cr}.
\QED


\bigskip
For the case of multiple targeted cloud nodes,
it is known that 
determining whether there exists a feasible quickest multicommodity 
flow with a given time horizon $T$
is NP-hard, but on the positive side, there exists an FPTAS to
it~\cite{quickest-multi}, i.e., we can approximate the optimal $T$ to
within $1+\epsilon$, for any constant $\epsilon > 0$.
Extending the reduction for
single commodity in the natural way, we obtain the following result.

\begin{theorem}
	[\theoremref{thm-caw-car-multi}]
	Given any instance of the \CWC model and $\epsilon>0$, a
	schedule realizing 
	$\CAW$ or $\CAR$ can be computed in  time polynomial in the instance
	size and $\epsilon^{-1}$. The length of the schedule is at most
	$(1+\epsilon)$ times larger than the optimal length.
	%  If all nodes
	%  write to (or read from) the same cloud node, optimal schedules for
	%  $\CAW$ and
	%  $\CAR$ can be computed in strongly polynomial time.
\end{theorem}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cwc"
%%% End:




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cwc.tex"
%%% End:


==> old/federated.tex <==
\def\XX{\mathbf{x}}
\def\YY{\mathbf{y}}
\def\ZZ{\mathbf{z}}

\section{Federated Learning With the Cloud}
\label{sec:federated}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section we explain how can the \cwc framework be used in the
context of federated learning, abbreviated FL henceforth.

First, let us briefly review the concept of FL (see
\cite{federated-17,federated-cacm} for a more detailed description; we
concentrate on the \emph{horizontal} flavor of FL here). The
premise is that while labeled data data is abundant, much of it is
private and the owners are not happy to share it (e.g.,
medical or financial information, or personal photographs). On the other hand,
effective learning by neural networks 
requires massive samples of labeled data. To bridge over this gap,
FL is a framework wherein each user applies the learning process to
its private data, and the parameters of their
learned networks are combined and shared with all, so that the only
information that leaks is the resulting combined network: no
individually generated information is shared with others.

In \cite{federated-secure}, a cryptographic protocol for FL
is presented, under the assumption that any two users can
communicate directly. The protocol of \cite{federated-secure} is
engineered to be
robust against malicious users, and uses cryptographic machinery such as
Diffie-Hellman key agreement and threshold secret sharing.  Here, we
propose
a simple scheme that is
tailored to the wheel topology of \figref{fig-ring}, assuming that
users are ``honest but curious.''

In a nutshell, the idea is as follows.
Each of the users has a vector of $m$ weights.  Weights are represented
by non-negative integers from $\Set{0,1,\ldots,M-1}$, so that user
input is simply a vector in$(\mathbb{Z}_M)^m$. We denote the
vector of user $i$ by $\XX_i$. The goal of the computation is to find
$\sum_{i=1}^n\XX_i$, which is also a vector in
$(\mathbb{Z}_M)^m$. To compute this sum securely, each user $i$
chooses a random vector $\ZZ_i\in(\mathbb{Z}_M)^m$, and
sends $\ZZ_i$ to user $i+1$. Then each user $i$ computes
$\YY_i=\XX_i-\ZZ_i+\ZZ_{i-1}$, where addition is modulo $M$. From
that point on, computation proceeds as usual using the $\YY_i$ values
instead of the $\XX_i$ values. It is easy to see that
$\sum_{i=1}^n\YY_i=\sum_{i=1}^n\XX_i$ because the $\ZZ_i$ vectors cancel
out. It is also clear that any partial sum of the $\ZZ_i$s is a random vector in
$(\mathbb{Z}_M)^m$. 

% While homomorphic encryption can be used in principle,
% The observation that makes FL work is that the weights vectors are
% additive: if the data is split over $n$ agents, with agent $i$ owning
% data $D_i$, and applying an iteration of the network $N$ results in
% improvement vector $v_i=N(D_i)$, then the global improvement vector
% $v=N(\bigcup_{i=1}^nv_i)$ satisfies $v=\sum_{i=1}^nv_i$.
% This additivity allows each user to apply the current network to her
% private data, send the resulting vector to a \emph{trusted central
%   server}, which combines the results, updates the network, and sneds
% the updated description to the users for another iteration, without
% any user compromising the privacy of her data. Another advantage of
% FL is that the computation load is shared among the users, relieving
% the demand on the server by some amount.

% Our \cwc paradigm can be used by FL in case where user-cloud bandwidth
% is an issue, while local communication enjoys high bandwidth. The idea
% is that users can locally--and privately--add 
% weight vectors using local links, and upload the resulting vector
% collectively. This way iteration time can be cut down considerably.






%%% Local variables:
%%% TeX-master: "cwc"
%%% End:

==> old/intro2.tex <==
\section{Introduction}
\label{sec:intro}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
While being very critical for the Internet operation, the DNS system is unforgiving, it has no \ariel{CTRL-Z}, i.e., no undo command.
For example, several Microsoft services like Azure and others were not available for a few hours in 2019 due to an erroneous DNS update that could not be easily corrected or undone \cite{azure}. 
Furthermore, the system is very sensitive to authoritative server failures or crashes due to DDoS or other attacks. \ariel{XXX - explain why}
In this paper, we examine \DNSUD{}, a method to add an undo command to the DNS system for a reasonable price in resources.
\DNSUD{} also increases the fault tolerant of the DNS system to name server crashes.

Internet domain name owners and managers have to set the TTL value associated with their domain records in the DNS system \cite{rfc1034} to dictate the maximum time a record may be stored in resolvers, stub resolvers, and client caches before they should obtain a fresh copy from the authoritative server \cite{rfc1035}.
Associating short TTL values with domain names is the current remediation for DNS \ariel{unforgiveness} however it comes with a high price tag in excess DNS traffic (\ariel{refreshing a popular domain record in different resolvers every TTL time}).
On the other hand, two major risks are associated with high TTL values for domain names \cite{choose-ttl-values}; first, if inadvertently a domain name is announced with the wrong IP, then the corresponding service is inaccessible for the duration of this high TTL time; secondly, if a service has to change its IP address (e.g., for maintenance, load balancing or any other reason) then again the clients have to wait for the expiration of the TTL before the change takes effect. 
\DNSUD{} suggested here provides the benefits of both: an undo command for quick recovery from erroneous updates and robustness against crashes, and at the same time, large TTL values to reduce the load on DNS authoritative servers.

\ignore{%%%%%%%%%%%%%%%%%
As a result, the TTL value of many domains is very short ($1-5$ minutes), even though most domains change their IP address infrequently (less than once a month). Content distribution networks (CDNs) \cite{kazunori2012cdn, centralized-dns} use even shorter TTLs ($\sim$ tens of seconds) to achieve high availability, load balancing, and frequent updates but only some of them indeed change their IP quite often.

The main consequence of choosing short TTL values is that most DNS requests receive the same response over and over, resulting in extra traffic to learn that there is nothing new.
}%%%%%%%%%%%%%%%%%%

There are two major observations on which \DNSUD{} is based; First, the method is backward compatible and adaptive. That is, any portion of the system may use \DNSUD{} while other parts continue operating in the traditional DNS method. 
Secondly, about $80\%$ of the domains on the Internet have a very high ratio of inter-IP address update time and TTL length.
These $80\%$ of domains would greatly benefit from using \DNSUD{}, while the others may keep using the traditional DNS mechanisms with low TTL values.
As a typical example, consider the popular Microsoft domain office.com whose TTL is $5$ minutes, but its IP address has not been updated for $3$ years.
Thus, at least every $5$ minutes, office.com is evicted from the resolvers' cache, and upon receiving a DNS request, the resolvers issue a new query to the authoritative server holding office.com.  That is, short TTL values are a significant cause of excess traffic between clients and resolvers as well as between resolvers and authoritative servers.

As stated above, our motivation came from incidents in which the wrong IP address was inadvertently associated with a domain, resulting in service disruption for the duration of the corresponding TTL value, which sometimes was several hours, as in the Microsoft incident from 2019 \cite{azure}. Where 
    Microsoft services like Azure, Microsoft 365 umbrella, Dynamics, and DevOps were down for more than 2 hours due to an incorrect DNS update.
    Microsoft published: "During the migration of a legacy DNS system to Azure DNS, some domains for Microsoft services were incorrectly updated." In another incident, in 2021 SiteGround services \cite{siteground} were not accessible to Google crawlers for several hours due to an incorrect DNS update.
    The company explained: "We have implemented a fix for the Google bot crawling issue experienced by some sites... Please allow a few hours for the DNS changes to take effect".
Other similar incidents have occurred, such as Zoho\cite{zoho}, Slack \cite{slack}, Microsoft \cite{win-update}, and Akami \cite{akami}.

\ignore{%%%%%%%%%%%%%%%%%%%%%%%%% 
We estimate this excess traffic by calculating the ratio between the average time between IP address updates for a domain and its corresponding TTL value. In addition, our analysis indicates that more than $80\%$ of the $500,050$ most popular domains change their IP address less than once a month and more than $60\%$ less than once a year. \footnote{We combined an up to date top $500$ domains list of moz.com with the top $500,050$ list of Alexa from $2021$. Due to the constrains of SecurityTrails \cite{securitytrails} we sampled $200$ domains from this list.  See Section \ref{sec:freq-updates}.} For these domains we found that at most $0.2\%$ of DNS responses contain a DNS record that has been changed since the previous response, \ariel{e.g., the IP address of the domain "Office.com" has not changed for more than $3$ years, but its TTL value is $300$ seconds.
Thus, every $300$ seconds at most, the domain is evicted from the resolver's cache, and upon receiving a DNS request, the resolvers issue it to the authoritative server.} As a result, short TTL values are a significant cause of excess traffic between clients and resolvers as well as between resolvers and authoritative servers.
This excessive traffic also causes client latency and server performance impairment \cite{moura2019cache}. In addition, website owners expose themselves to another availability problem - if there is no access to their authoritative servers, when their short TTL expires, the access to their website is disabled \cite{facebook}.

As stated above, our motivation came from incidents in which the wrong IP address was inadvertently associated with a domain, resulting in service disruption for the duration of the corresponding TTL value, which sometimes was several hours, as in the Microsoft incident from 2019:
\begin{itemize}[leftmargin=0.12in]\setlength\itemsep{0em}
    \item Microsoft \cite{azure} - In 2019, Microsoft services like Azure, Microsoft 365 umbrella, Dynamics, and DevOps were down for more than 2 hours due to an incorrect DNS update. Microsoft published: "During the migration of a legacy DNS system to Azure DNS, some domains for Microsoft services were incorrectly updated."
    \item SiteGround \cite{siteground} - In 2021, SiteGround services were not accessible to Google crawlers for several hours due to an incorrect DNS update. The company explained: "We have implemented a fix for the Google bot crawling issue experienced by some sites... Please allow a few hours for the DNS changes to take effect".
\end{itemize}
Similar incidents have occurred, such as Zoho\cite{zoho}, Slack \cite{slack}, Microsoft \cite{win-update}, and Akami \cite{akami}.

}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nsdionly{%%%%%%%%%%%%%%%%%%%%
Many people rightfully describe the DNS as the phone book of the Internet.
In both, when clients need the IP address of a domain or the phone number of another person or business, they query either the DNS system or use a search engine to query for the desired phone number. However, there is a difference; IP addresses sometimes change frequently, while the phone number of people change quit infrequently. Thus using a contact-list (cache) on mobile devices is helpful for phone books but requires much more care and sophistication in the DNS system due to the dynamic nature of IP addresses associated with endpoints. Still, the DNS system relies on caches with a TTL value attached to each record. However, suppose, for some reason, the cache contains the wrong IP address for a domain. In that case, there is no automatic mechanism to query the authoritative server again to get a fresh record. As a result, clients query the DNS system regularly, regardless of whether record updates have occurred, unlike updates of a phone contact list when the mentioned person updates her phone number.

Internet service owners compromise on any choice of TTL: large TTL values cause slow recovery from an IP address change, while short TTLs generate excess traffic and load.
}%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this paper, we propose \DNSUD{}, a mechanism to update a record in resolver caches before the associated TTL has expired.
In a nutshell, \DNSUD{} updates the resolvers about domains whose records were recently updated.
After that, the resolvers remove the corresponding records from their cache.
Upon receiving a subsequent request for a removed domain, the resolver performs a new resolution in the standard DNS system to get a fresh update.
\DNSUD{} is secure, efficient, robust to DDoS attacks, and fully compatible with the current DNS system. 

\ariel{Furthermore, \DNSUD{} enables Internet services to significantly increase the TTL values associated with their domain names in resolvers' cache (client caches are discussed in the sequel). Thus, we add an additional second TTL value, called DNS\em{RU}-TTL while maintaining the traditional TTL that is used to communicate with clients and resolvers that do not use the method. 
To achieve backward compatibility,
DNS\em{RU}-TTL is sent in DNS responses in an optional field (in the ADDITIONAL section) for resolvers that have implemented \DNSUD{}.
\ignore{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Domain names with short TTL values (less than $10$ minutes) benefit from \DNSUD{} since larger TTL values reduce their DNS traffic and the average latencies experienced by clients. Furthermore, for domain names with large TTL values, \DNSUD{} provides quick recovery from IP address changes.
To achieve the backward compatibility of the \DNSUD, we added an additional TTL value, an optional field, used by clients and resolvers that are not yet using the \DNSUD, besides the traditional TTL value (used by the clients).
} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this way, an authoritative server that uses \DNSUD{} can communicate with resolvers that implemented or did not the method, and a resolver that uses \DNSUD{} can communicate with both authoritative servers that implemented or did not the method.
In Section \ref{sec:beyond}, we discuss methods to expand \DNSUD{} to enable clients to use the additional larger TTLs and reduce the excessive DNS traffic also between clients and resolvers.}
\ignore{While the method could be applicable also for clients and stub resolvers, in their case efficiency and complexity of the method, as well as their small cache size, needs to be considered, see Section \ref{sec:beyond}.}
\nsdionly{%%%%%%%%%%%%%%%%%%
Unlike the phone book, the trigger in \DNSUD{} is initiated by the authoritative server rather than the client, i.e., some kind of a pull method initiated by a push.
}%%%%%%%%%%%%%%%%%%

Related work and alternative methods are presented in Section \ref{sec:background}. Detailed description of the \DNSUD{} service is provided in Section \ref{sec:solution}.
In Section \ref{sec:increase-ttl} we describe the primary implication of increasing TTL values and how we preserve the backward compatibility of \DNSUD{}. \ariel{In section \ref{sec:analysis}, we analyze the relevancy and feasibility of the method, and discuss about its possible implications in Section \ref{sec:implications}.}
In Section \ref{sec:extension} an extension is presented to provide fast recovery when an authoritative server is unavailable.
In Section \ref{sec:beyond} we expand our method to apply also to the clients -- resolvers communication, that is, updating stale records in browsers and other client applications before the corresponding TTL has expired. Finally, conclusions are given in Section \ref{sec:conclusion}.

\ignore{Our analysis indicates that more than $80\%$ of the $50$ most popular domains and the $450-500$ most popular, change their IP address less than once a month, and more than $50\%$ less than once a year. Domain names with short TTL values (less than $10$ minutes) benefit from \DNSUD, by using much larger TTL values and reducing their DNS traffic and the average latencies experienced by clients. Also, \DNSUD{} could ensure a constant and quick recovery from IP address changing for domain names with large TTL values.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cwc"
%%% End:


==> old/locallywide.tex <==
\subsection{The Case of Fat links and Commutative Operators}
\label{sec-fat-combining}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Recall that given a parameter $s$, we say that a \CWC system
$G=(V,E,w)$ has
\emph{fat links} if the bandwidth of all its local links is at least
$s$, and if all links are symmetric (i.e., have the same bandwidth on both directions).
In this \dsubsection we focus on combining with a commutative operator in
systems with fat links. In this case (unlike the results of \subsectionref{sec-ccw-flow}) we
can construct a near-optimal algorithm for \CCW.
The idea is to use multiple $\CW$ and \CR operations
instead of \CAW and \CAR. The challenge is to
minimize the number of operations that any single node needs to participate in simultaneously:
%have small overlap between the operations:
to this end we use 
Awerbuch and Peleg's sparse covers.

We note that the results shown in this \dsubsection are
stated for $s$-fat-links graphs and
operators with operands of size $s$.
However, the presented algorithms can be easily modified for the case
of $s$-fat-links graphs and operands of size $s'$,
increasing the running-time by a factor $\ceil{s'/s}$,
either by repeating the algorithm $\ceil{s'/s}$ times,
or by multiplexing.
The lower bounds presented in this \dsubsection however, may change
greatly depending on the values of $s$ and $s'$, not necessarily by an $\ceil{s'/s}$ factor.
In case that $s'/s = O(1)$, i.e., $s' = O(s)$, the lower and upper bounds
achieved in this \dsubsection remain the same.




We start with a tight analysis of \CW and \CR in this setting and then
generalize to \CCW and \CCR.



\subsubsection{\CW and \CR}
Consider $\CW_i$, where $i$ wishes to write $s$ bits to a given cloud node. 
The basic tension in finding an optimal schedule for $\CW_i$ is that in order to use more cloud bandwidth, nodes further from $i$ need to be enlisted. But while more bandwidth reduces the total
time, reaching these extra nodes (that provide the extra BW) increases the total time.
Therefore, our algorithm looks for the
sweet spot where the effects are more-or-less balanced.

For example, consider a simple path of $n$ nodes with infinite local bandwidth
and a single cloud node $v_c$
\ignore{(see \figref{fig-tradeoff-example})}.
Let $l$ be the left endpoint,
let $w(u,v_c) = x$ for every node $u$, and assume that
node $l$ attempts to write a message $S$ of size $s$ bits to the cloud.
To write the message by itself, node $l$ would require $s/x$ rounds.
Using the bandwidth of all $n$ nodes for that matter would take
$O(s/nx)$ rounds, but would also require $n-1$ rounds to send the file
along the path.
The optimal solution however would be to use only $\sqrt{s/x}$ nodes,
in which case the time to send the file to all nodes would be $\sqrt{s/x}$,
and the time to send the file to the cloud using their combined bandwidth would be
${\frac{s}{x\cdot \sqrt{s/x}}} = \sqrt{s/x}$ as well.


\ignore{%%%%  no space for this figure in ICDCN 
\begin{figure}[t]
	\centering
	\scalebox{.7}{
		\begin{tikzpicture}
			\node[draw, circle, inner color=white, minimum size=1cm] at (0,0) (mid) {$$};
			\node[draw, circle, fill=yellow!90!black, minimum size=1cm] at (-2,0) (l) {$l$};
			\node[draw, circle, inner color=white, minimum size=1cm] at (3,0) (r) {};
			\node[draw, circle, inner color=white, minimum size=1cm] at (5,0) (rfar) {$$};
			\node at ($(mid)!.5!(r)$) (dots) {\ldots};
			
			\node [cloud, draw,cloud puffs=23,cloud puff arc=120, aspect=7, inner ysep=1em]
			at 	(1.6, 2.5)
			{\emph{$v_c$}};
			
			\draw [-] (mid) -- (l)
			node [above,text width=3cm,text centered,midway] {$\infty$};
			\draw [-] (mid) -- (dots)
			node [above,text width=3cm,text centered,midway] {$\infty$};
			\draw [-] (r) -- (dots)
			node [above,text width=3cm,text centered,midway] {$\infty$};
			\draw [-] (r) -- (rfar)
			node [above,text width=3cm,text centered,midway] {$\infty$};
			\draw [->] (mid) -- (0, 1.45)
			node [right,text width=0cm,text centered,midway] {$x$};
			\draw [->] (r) -- (3, 1.45)
			node [right,text width=0cm,text centered,midway] {$x$};
			\draw [->] (l) -- (-2, 1.45)
			node [right,text width=0cm,text centered,midway] {$x$};
			\draw [->] (rfar) -- (5, 1.45)
			node [right,text width=0cm,text centered,midway] {$x$};
		\end{tikzpicture}
	}
	\caption{ \em
		A simple path example. The optimal distance to travel in order to
		write an $s$-bits file to the cloud would be $\sqrt{s/x}$.
	}
	\label{fig-tradeoff-example}
\end{figure}
}%%%%


Formally, in the general case, we define clusters of processing nodes in a graph,
and define the ``cloud clusters'' of nodes and their parameters,
which are clusters that optimize the ratio between their diameter
and their total bandwidth to the cloud.
We then continue to
present algorithms for \CW and \CR that uses only nodes of
a given cloud cluster,
%following the lines of \cite{Peleg:book},
% We then continue to define the ``cloud clusters'' of nodes and their parameters,
and prove that the running-timeof the \CW and \CR algorithms on these clusters
are optimal.

%We start with a few definitions.

\begin{definition}\label{def-clusters}
	Let $G=(V,E,w)$ be a \CWC system with processor nodes $V_p$ and cloud nodes $V_c$.
	The \textbf{cloud bandwidth} of a processing node $i \in V_p$ w.r.t.\ a
	given cloud node $v_c\in V_c$ is $\bc(i)\DEF w(i,v_c)$.
	A \textbf{cluster} $B \subseteq V_p$ in $G$ is a connected set
	of processing nodes. The \textbf{cloud (up or down) bandwidth} of cluster $B$ w.r.t\ a given
	cloud node,
	denoted $\bc(B)$, is the sum of the cloud bandwidth to $v_c$ over all nodes in
	$B$: $\bc(B)\DEF\sum_{i\in B}\bc(i)$.  The (strong) \textbf{diameter}
	of cluster $B$, denoted $\Diam(B)$, is the maximum distance between
	any two nodes of $B$ in the induced graph $G[B]$:
	$\Diam(B) = \max_{u,v \in B} {dist_{G[B]}(u, v)}$.
	%  The \textbf{timespan} of cluster $B$, denoted $Z(B)$, is given by
	%  $Z(B) = \Diam(B) + {s}/{\bc(B)}$.
\end{definition}

We also use the following standard definition, applied to the network without the cloud.

\begin{definition}\label{def-Ball}
	Let $G=(V,E,w)$ be a \CWC system with processing nodes $V_p$ and
	cloud nodes $V_c$.  The \textbf{ball of radius $r$
		around node $i\in V_p$}, denoted $\Br r i$ is the set of nodes at most $r$ hops away
	from $i$ in $G_p$.
\end{definition}
\noindent
Note that the metric here is hop-based
(while the weight  $w$
indicates link bandwidths). %, not latency. 
% Also, balls are defined with
% respect to local links only.

Finally, we define the concept of cloud cluster of a node.



\begin{definition}\label{def-Bi}
	Let $G=(V,E,w)$ be a \CWC system with processing nodes $V_p$ and
	cloud node $v_c$, and let $i\in V_p$.
	% \item A \textbf{ball} of radius $r$ from node $i$, $\Br{r}{i}$,
	%   is the set of all nodes within distance $r$ from $i$
	%   ($\Br{r}{i} = \{ v \mid d(i,v) \le r \}$).
	Given $s\in\mathbb{N}$,  the \textbf{$s$-cloud radius} of
	node $i$, denoted $\kkR{i}s$, is defined to be
	%  $\Diam(G_p)$ if
	%  $\bc(V)<s$, and otherwise
	$$
        \kkR{i}s\DEF\min
	\left(\Set{\Diam(G_p)}\,\cup\, \Set{k\mid 
		%k \le \Diam(G_p) \wedge
		\left(k\tp 1\right) \cdot \bc(\Br{k}{i}) \ge s}\right)~.
	$$
	%   , but we cap \kkR{i}s$ 
	%   If not such $k$ exists, we define $\kkR{i}s$ to be $\Diam(G_p)$.
	The ball $\BR{i}\DEF \Br{\kkR{i}s}{i}$ is the $s$-\textbf{cloud
		cluster} of node $i$.
	The \textbf{timespan} of the $s$-cloud cluster of $i$
	is denoted $\ZR{i}\DEF \kkR{i}{s} + \frac{s}{\bc(\BR{i})}$.
	%  is denoted $\ZR{i}\DEF \Diam(\BR{i}) + {s}/{\bc(\BR{i})}$.  
	We sometimes omit the %subscript
	$s$ qualifier when it is clear from the context.
\end{definition}
In words, $\BR{i}$ is a cluster of  radius $\kR i $ around node $i$,
where $\kR i$ is the smallest radius that allows writing $s$ bits to $v_c$ by
using all cloud bandwidth emanating from
$\BR i$ for $\kR i+1$ rounds.
$\ZR{i}$ is the sum of the time required to send a message from node $i$ to all nodes of
$\BR{i}$ with the time required to send a message of size $s$ to $v_c$
when all the nodes of the cluster send it together.
% such that the time required to transfer $s$ bits to all nodes in the cluster
% through the local links, is as close as possible to the time required to write
% $s$ bits using all the cloud bandwidth emanating from $\BR i$. 
%$\kR{i}$ is easily computable, and that
Notice, it is easy to compute the cloud cluster of a node.   The upper bound is then:
\begin{theorem}\label{theorem:CW_UB}
	Given a fat-links \CWC system, \algref{alg:cw-hi} solves the
	$s$-bits $\CW_i$ problem in $O(\ZR{i})$ rounds on $\BR{i}$.
\end{theorem}


\begin{algorithm}[t]%\small
	\caption{$\CW_i$ }
	\label{alg:cw-hi}
	\begin{algorithmic}[1]
		\STATE \label{cw-alg-BFS-tree}
		Construct a BFS spanning tree of $\BR{i}$ rooted at node $i$
		and assign for each index $1 \le x \le |\BR{i}|$ a unique node
		$v(x)\in \BR{i}$ according to their BFS order ($v(1)=i$)
		\STATE \label{cw-alg-send-local}
		Broadcast $S$ from node $i$ to all nodes in $\BR{i}$ using the tree
		\FOR{all $x:=1$ \textbf{to} $|\BR{i}|$, in parallel}
		\STATE\label{cw-alg-node-write}{
			Node $v(x)$ writes to the cloud the part of $S$ starting at
			%      $s\cdot\left({ \sum_{y=1}^{x-1}{\bC{v(y)}} }\right)/{\bC{\BR i}} $
			$s\cdot\frac{ \sum_{y=1}^{x-1}{\bC{v(y)}} }{\bC{\BR i}} $
			and extending for $s\cdot\frac{\bC{v(x)}}{\bC{\BR i}}$ bits,
			writing $\bC{v(x)}$ bits in every round.}
		\STATE\label{cw-alg-ack}{Node $v(x)\ne i$ sends an acknowledgment to $i$
			when done, and halts}
		\ENDFOR    
		\STATE\label{cw-alg-end} Node $i$ halts when all acknowledgments
		are received.
		\hfill{\em // useful when reversing for \CR}
	\end{algorithmic}
\end{algorithm}



\smallskip
Next, we show that our solution for $\CW_i$ is optimal, up to a
constant factor.  We consider the case of an incompressible input
string: such a string exists for any size $s\in\mathbb{N}$ (see, e.g.,
\cite{LiV:Kolmogorov}).  As a consequence, {in any execution of a
	correct algorithm, $s$ bits must cross any cut that separates $i$
	and the cloud node}, giving rise to our 
	%\yehuda{ $\frac{s}{\bc(\BR{i})}$} 
	lower bounds:

\begin{theorem}
	\label{theorem:CW_LB}
	$\CW_i$ in a fat-links \CWC    requires
	$\Omega(\ZR{i})$ rounds.
\end{theorem}


%\bigskip
By reversing time (and hence information flow) in a schedule of \CW, one gets a schedule for \CR. %\gal{is that clear enough?}.
Hence we have the following immediate corollaries.

\begin{theorem}\label{theorem:CR_UB}
	%  In a \CWC system with fat-links, 
	$\CR_i$ can be executed in
	$O(\ZR{i})$ rounds in a fat-links \CWC.
\end{theorem}

% Using arguments as for $\CW_i$, we also have the following lower bound.

\begin{theorem} \label{theorem:CR_LB} 
	$\CR_i$ in a fat-links \CWC    requires $\Omega(\ZR{i})$ rounds.
\end{theorem}

\para{Remark:}
Note that the lower bound
and the definition of \emph{cloud clusters} (\defref{def-Bi})
reveals an interesting relationship between the
message size $s$ and the cloud clusters in a graph;
If $s$ is too large, then the cloud cluster of a node may include all processing nodes,
making the distance traveled on the local network irrelevant.
On the other hand, if $s$ is too small, the cloud cluster may include only
a single node, making the local network redundant.
%\gal{Boaz, is that what you wanted? it doesn't feel really interesting..}




%\subsection{Algorithms for Combining}
\subsection{\CCW}
\label{ssec:combining}

% We are now ready to prove an upper bound on \CCW in a \CWC system with
% fat-links when 
% the combining operator is commutative.
%Similarly to our strategy in solving \CW and \CR,
Having defined clusters for a single write or read,
we extend the notion to covers which consist of multiple
clusters. Below, we first show how 
to implement \CCW using any given cover,
and then use the result with \emph{sparse covers} \cite{AP90},
which has parameters that allow us to to get near-optimal performance.

Intuitively, every node $i$ has a cloud cluster $\BR{i}$ which allows it
to perform $\CW_i$, and calculating the combined value within every cloud cluster $\BR{i}$
is pretty straight-forward, as we later demonstrate in
\algref{alg:ccw-low} and \lemmaref{lemma:ccw-low-runtime}.
Therefore, given a cover of the graph that consists of pairwise disjoint
cloud clusters, \CCW can be solved by
combining the inputs within every cloud cluster, followed by
combination of the partial results in a computation-tree fashion using
\CW and \CR.
However, such a cover may not always exist.
Given a cover $\CC$ in which every node is a member of at most $\load(\CC)$ clusters,
we can use the same technique, while increasing the running-time by a factor of $\load(\CC)$
by multiplexing.
Using Awerbuch and Peleg's sparse covers theorem (see \theoremref{thm-AP}),
we can use the initial cover $\CC$ that consists of all cloud clusters in the graph
to construct another cover, $\CC'$, in which $\load(\CC')$ is at most $\log n$,
by paying a $\log n$ factor in the maximum diameter size of the clusters,
and use $\CC'$ to get near-optimal results.




% , we use the concept of covers.

% After defining some parameters of clusters and
% defining the standard notion of covers, we present an algorithm
% for \CCW that operates on a given cover of clusters, and then
% use it to obtain a near-optimal algorithm.
%

\begin{definition}\label{def-clusters-params}
	Let $G$ be a \CWC system, and let $B$ be a cluster in $G$ (see
	\defref{def-clusters}).  The \textbf{timespan of node $i$ in $B$},
	denoted $Z_B(i)$, is the minimum number of rounds required to
	perform $\CW_i$ (or $\CR_i$), using only nodes in $B$.
	The \textbf{timespan of cluster} $B$, denoted $Z(B)$, is given by
	$Z(B) = \min_{i\in B}Z_B(i)$.  The \textbf{leader} of cluster $B$,
	denoted $r(B)$, is a node with minimal timespan in $B$,
	i.e., $r(B) = \argmin_{i\in B} Z_B(i)$.
	%  (we break ties arbitrarily).
\end{definition}
In words, the timespan of cluster $B$ is the minimum time required
for any node in $B$
to write an $s$-bit
string to the cloud using only nodes of $B$.


\begin{definition}%[Covers]
	\label{def-covers}
	Let $G$ be a \CWC system with processing node set $V_p$.
	A \textbf{cover} of $G$ is a set of clusters
	$\CC = \{ B_1, \ldots, B_m \}$ such that 
	%every processing node
	%$v\in V_p$ is a member of at least one cluster in $C$, i.e.,
	$\cup_{B \in \cC} B = V_p$.
	The \textbf{load of node $i$} in a cover $\CC$ is the number of
	clusters in $\CC$ that contain $i$, i.e.,
	$\load_{\CC}(i) = |\{B \in \CC \mid i \in B\}|$.
	The \textbf{load of cover $\CC$} is the maximum load of any node
	in the cover, i.e.. $\load(\CC) = \max_{i\in V_p}
	{\load_{\CC}(i)} $.  % \todo{call
	% it overlap, or $over(C)$, instead of load?}
	The \textbf{timespan} of cover $\CC$, denoted
	$\ZC(\CC)$, is the maximum timespan of any cluster in $\CC$,
	$\ZC(\CC) = \max_{B\in \CC} {Z(B)}$.
	The \textbf{diameter} of cover $\CC$, denoted $\Diam_{\max}(\CC)$,
	is the maximum diameter of any cluster in $\CC$,
	$\Diam_{\max}(\CC) = \max_{B\in \CC} {\Diam(B)}$.
\end{definition}



\begin{algorithm}[t]%\small
	\caption{High-level algorithm for \CCW given a cover $\CC$}
	\label{alg:ccw-hi}
	\begin{algorithmic}[1]
		\STATE\label{cluster-graph}
		For a node $i\in V_p$, let $C_i[1],C_i[2],\ldots$ be the clusters containing $i$.
		% $B \ni i$ for whom $i \in B$
		% from $1$ to $\load_{\CC}(i)$.
		% Let $\ClusJ{i}{j}$ be the $j$-th cluster of node $i$. \boaz{bad notation $\ClusJ i j$}
		%    Construct a cluster graph $G_{\mathcal C}$ whose nodes are
		%    the clusters of $\CC$, and two nodes are connected by edge
		%    iff the corresponding clusters overlap.
		
		\STATE\label{ccw-1}
		For the rest of the algorithm, multiplex each round as $\load(\CC)$ rounds,
		such that each node $i$ operates in the context of cluster $C_i[j]$ %$\ClusJ{i}{j}$
		in the $j$-th round .
		% for $j=1,\ldots,\load_{\CC}(i)$.
		%    Color the nodes of $G_{\CC}$  using
		%    $\load(\CC) \tp 1$ colors. Let $\CC_j$ denote the
		%    set of clusters colored $j$, for $j=1,\ldots,\load(\CC) \tp 1$.
		%    \FOR{$l:=1$ \textbf{to} $\load(\CC)\tp 1$ (sequentially)
		%    }
		%    \label{ccw-colors}
		\FORALL{$B\in \CC$, in parallel}
		\label{ccw-startloop}
		\STATE\label{ccw-local}{
			Compute $P_B=\bigotimes_{j\in B}S_j$ using \algref{alg:ccw-low}
			\hfill{\em // convergecast using local links only}
			% \hfill$\rhd$~\textit{
			% the input of each node is combined exactly once in all iterations
			% }
		}
		\ENDFOR
		%    \ENDFOR
		\label{ccw-endloop}
		\STATE\label{ccw-high} % Compute $\bigotimes_{B\in C}P_B$ using
		Apply %\algref{alg:ccw-high:overlap} and then
		\algref{alg:ccw-high:node}
		\hfill{\em // the result is stored in the cloud}
	\end{algorithmic}
\end{algorithm}  


We now give an upper bound in terms of any given cover.
\begin{theorem}\label{thm-ccw-covers-ub}
	Given a cover $\CC$, \algref{alg:ccw-hi} solves \CCW in a
	fat-links \CWC in	$O\left(\Diam_{\max}(\CC) \cdot \load(\CC) + \ZC(\CC) \cdot \load(\CC) \cdot \log |\CC|\right)$
	rounds.
\end{theorem}

The basic strategy is to first compute the multiplication of the inputs
in each cluster 
using only the local links,
and then compute the multiplications among clusters using a
computation tree. However, unlike \algref{alg:caw-flow}, we use
\CW and \CR in possibly overlapping clusters instead of \CAW and \CAR.
% \todo{we can actually implement line \ref{ccw-high} using \algref{alg:caw-flow},
% which can only improve the runtime}




A high-level description is given in \algref{alg:ccw-hi}.  The
algorithm consists of a preprocessing part (lines
\ref{cluster-graph}-\ref{ccw-1}), and the execution part, which consists
of the ``low-level'' computation using only local links (lines
\ref{ccw-startloop}-\ref{ccw-endloop}), and the ``high-level''
computation among clusters (line \ref{ccw-high}).



\para{Preprocessing.}
%%%%%%%%%%%%%%%%%%%%%%
A major component of the preprocessing stage is computing the cover $\cC$, which we specify later (see \theoremref{thm-ccw-ub}). In \algref{alg:ccw-hi}
we describe the algorithm as if it operates in each cluster independently of
other clusters, but clusters may overlap. To facilitate this mode of operation, we use time multiplexing: nodes execute work on behalf of the clusters they are member of in a round-robin fashion, as specified 
in lines \ref{cluster-graph}-\ref{ccw-1} of \algref{alg:ccw-hi}.
% , the algorithm
% assigns a unique index between $1$ and $\load_{\CC}(i)$ to each cluster $B \in \CC$
% containing $i$, for every node $i$.
% %partitions
% %the cover to $\load(\CC)\tp 1$ colors. 
% In line \ref{ccw-1}, we explain how to execute cluster operations in parallel,
% by treating each round as $\load(\CC)$ rounds:
% In each round $1 \le j \le \load(\CC)$,
% every node $i$ would operate in the context of its $j$-th cluster.
This allows us to
invoke operations limited to clusters in all clusters
``simultaneously'' 
%of a given color
%class in parallel independently, as they are disjoint. Therefore we
%can apply such operations in all clusters
while paying a
$\load(\CC)$-factor in the running-time over a single invocation.

% \begin{lemma}
% 	\label{lem-coloring}
% 	$C$ can be partitioned into $\load(C)\tp 1$ color classes such that all
% 	clusters of the same color are pairwise disjoint.
% \end{lemma}
% \Proof Consider a graph $G_C$
% whose nodes are the clusters in $C$, and
% there is an edge connecting any two nodes whose corresponding
% clusters intersect.
% By definition,
% each cluster in $C$ 
% intersects at most $\load(C)$ other clusters in $C$,
% the maximum degree in $G_C$ is $\load(C)$,
% and therefore the nodes of $G_C$ can be colored by $\load(C)+1$
% colors by a greedy coloring algorithm.
% Since there is no edge connecting two nodes of the same color,
% we obtain the desired partition by defining $C_l$, for $l=1, \ldots \load(C)+1$, to be the
% set of all clusters whose corresponding nodes in $G_C$ are colored $l$.
% \QED


\para{Low levels: Combining within a single cluster.}
%\label{ssec-cluster-combining:low}
To implement line \ref{ccw-local} of \algref{alg:ccw-hi}, we build a
spanning tree within each cluster $B\in \CC$, and apply
Convergecast~\cite{Peleg:book} using $\otimes$.  To do that, we use a
rooted tree. In our case, the identity of the root affects the running
time by at most a factor $2$, so given a cluster $B$, we set its leader
$r(B)$ to be the root.  We state the following
immediate lemma (the running time ignores the multiplexing of \algref{alg:ccw-hi}).
\begin{lemma} \label{lemma:ccw-low-runtime} \algref{alg:ccw-low}
	computes $P_B = \bigotimes_{i\in B} S_i$ at node $r(B)$  in   $O(\Diam(B))$ rounds.
\end{lemma}
We note that to get the right overall result, each input $S_i$
is associated with a single cluster in $\CC$.  To this end, we
require each node to select a single cluster in which it is a member
as its \emph{home cluster}.  When applying \algref{alg:ccw-low}, we
use the rule that the input of node $i$ in a cluster $B\ni i$ is $S_i$
if $B$ is $i$'s home cluster, and $\Unit$ otherwise.

% For a cluster $B$, let $r$ denote with the minimal index in $B$, be the
% \emph{leader} of the cluster.
% The computation of the combined value of each cluster $B$ in $r(B)$ is achieved using
% Converge-Cast (\cite{Peleg:book}) and is demonstrated in
% \algref{alg:ccw-low}, as can be seen by the following trivial lemma.

% \Proof
% Correctness is obvious.
% For the time analysis, we note that the height $h$ of any BFS spanning tree of $B$
% can be at most $\Diam(B)$, and therefore the loop of Step \ref{alg:ccw-low:for-loop}
% requires at most $\Diam(B)$ rounds.
% Furthermore, finding a BFS spanning tree of cluster $B$ can be done in $O(\Diam(B))$
% rounds (\todo{add reference}).
% \QED




% We immediately get the following lemma, by noting that for every color
% $1\le l \le \load(C)+1$,
% all clusters of $C_l$ are pairwise disjoint and can therefore run \algref{alg:ccw-low}
% in parallel.
% %and that for every cluster $B \in C$, $\Diam(B) \le Z(B) \le \ZC(C)$.

%We state the following lemma for later reference.
Considering the scheduling obtained by Step \ref{ccw-1},
we get the following lemma.
\begin{lemma} \label{ccw-lem-lo} Steps
	\ref{ccw-startloop}--\ref{ccw-endloop} % \ref{aw-4}
	of \algref{alg:ccw-hi} terminate in
	$O(\Diam_{\max}(\CC) \cdot \load(\CC))$ rounds, with $P_B$ stored
	at the leader node of $B$ for each cluster $B\in C$.
\end{lemma}

\begin{algorithm}[t]%\small
	\caption{Computing the combined result of cluster $B$ at leader $r(B)$}
	\label{alg:ccw-low}
	\begin{algorithmic}[1]
		\STATE %\label{}
		Construct a BFS tree of $B$ rooted at node $r(B)$.
		Let $h$ be the height of the tree.
		\FOR{$d:=h$ \textbf{to} $2$} \label{alg:ccw-low:for-loop}
		\FORALL{$i \in B$ at layer $d$ of the tree, in parallel}
		\IF {$i$ is not a leaf}
		\STATE {$i$ computes $S'_i:=S_i \otimes \bigotimes_{j\in child(i)}S'_j$}
		\ELSE
		\STATE {$S'_i:=S_i$}
		\ENDIF
		\STATE {$i$ sends $S'_i$ to its parent node in the tree}
		\ENDFOR
		\ENDFOR    
		\STATE\label{alg:ccw-low:end} Node $r(B)$ computes
		$P_B:=  S_{r(B)} \otimes \bigotimes_{j\in child(r(B))}S'_j$
	\end{algorithmic}
\end{algorithm}



\para{High levels:  Combining using the cloud.}
%\label{ssec-cluster-combining:high}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
When \algref{alg:ccw-hi} reaches Step \ref{ccw-high}, the combined
result of every cluster is stored in the leader of the cluster.
The idea is now to fill in a computation tree whose 
leaves are these values.
%(cf.~\figref{fig-tree})
% \gal{I'm not sure that this figure relates here, other than being a tree}
% whose leaves are the cluster results. To get good running time, we
% schedule the computation carefully.

%First, to avoid paying the $(\load(\CC+1))$-factor over and
%over again, \algref{alg:ccw-high:overlap} copies all partial
%results to clusters to the largest color class $\CC$
%%subset of the
%%$\load(C)\tp 1$ subsets of $C$ that were acquired in Step \ref{ccw-1},
%using \CW and \CR. Then
%\algref{alg:ccw-high:node} fills the values in
%the computation tree using only clusters of that color class without
%any interference among them. We now explain these steps in more detail.


%Let $m$ be the number of clusters in the largest color class, i.e.,
%$m = \max\Set{|\CC_l|}$, let $B_i^l$ denote the $i$-th cluster
%in $C_l$ under some fixed order, and let
%$P_i := \bigotimes_{l=1}^{\load(C)\tp 1}{P_{B_i^l}}$.  Assume \WLOG
%that $\CC_1$ is the largest color class,
%i.e., $|\CC_{1}| = m$.  Since we use the largest color class,
%we have the following result. %(Note that \CR and \CW require at most $\ZC(C)$)
%\begin{lemma} \label{lemma:alg:ccw-high:overlap}
%  \algref{alg:ccw-high:overlap} computes $P_i$ in the leader of
%  cluster $B_i^1$, for every $1 \le i \le m$ in
%  $O(\ZC(\CC) \cdot \load(\CC))$ rounds.
%\end{lemma}
%\Proof By \theoremref{theorem:CW_UB},
%\theoremref{theorem:CR_UB}, and the definition of
%$\ZC(\CC)$ (\defref{def-covers}). \QED

%\begin{algorithm}[t]%[H]\small
%  \caption{Computing partial results in color class $\CC_1$ of maximal size $m$}
%  \label{alg:ccw-high:overlap}
%  \begin{algorithmic}[1]
%    \FOR[Write loop]{$l:=2$ \textbf{to} $\load(\CC)\tp 1$} \label{}
%    % \hfill$\rhd$~~\emph{Write loop}
%    \FOR{$i:=1$ \textbf{to} $m$, in parallel}
%    \STATE {Cluster $B_i^l$ writes $P_{B_i^l}$ to the cloud by initiating
%      \CW at node $r(B_i^l)$}
%    \ENDFOR
%    \ENDFOR
%    \FOR[Read loop]{$i:=1$ \textbf{to} $m$, in parallel}
%    % \hfill$\rhd$~~\emph{Read loop}
%    \FOR{$l:=2$ \textbf{to} $\load(\CC)\tp 1$} \label{}
%    \STATE {Cluster $B_i^1$ reads $P_{B_i^l}$ from the cloud by initiating
%      \CR at node $r(B_i^1)$}
%    \ENDFOR
%    \STATE Node $r(B_i^1)$ computes
%    $P_i := \bigotimes_{l=1}^{\load(\CC)\tp 1}{P_{B_i^l}}$
%    \label{alg:ccw-high:overlap:combine}
%    \ENDFOR
%  \end{algorithmic}
%\end{algorithm}


We combine the partial results by filling in the values of a
computation tree defined over the clusters.  The leaves of the tree
are the combined values of the clusters of $\CC$, as
computed by %in line \ref{alg:ccw-low:end} of
\algref{alg:ccw-low}.  To fill in the values of other nodes
in the computation tree, we use the clusters of $\CC$: Each node in
the tree is assigned a cluster which computes its value using the \CR
and \CW primitives.
%Let $h(I)$, the rightmost node of an interval $I$, be the
%\emph{leader} of the interval.

\begin{algorithm}[t]%\small
	\caption{Computing the high level tree-nodes values}
	\label{alg:ccw-high:node}
	\begin{algorithmic}[1]
		\FOR{$l:=\ceil{\log |C_1|}$ \textbf{to} $1$} %\label{}
		\FORALL{tree-nodes $y$ in layer $l$ of the computation tree, in parallel}
		\STATE Let $B := \Clus(y)$
		\IF {$y$ is not a leaf}
		\STATE Let $y_\ell$ and $y_r$ be the left and the right children
		of $y$, respectively.
		\STATE \label{alg:ccw-high:node:read1}
		$r(B)$ invokes \CR for $\Val(y_\ell)$
		\STATE \label{alg:ccw-high:node:read2}
		$r(B)$ invokes \CR for $\Val(y_r)$
		\STATE $r(B)$ computes $\Val(y):=\Val(y_\ell)\otimes \Val(y_r)$
		\ELSE
		\STATE $\Val(y):=P_B$
		\hfill{\em // if $y$ is a leaf its value is already stored at $r(B)$}
		\ENDIF
		\hfill
		\STATE \label{alg:ccw-high:node:write}
		$r(B)$ invokes $\CW$ for $\Val(y)$
		\ENDFOR
		\ENDFOR
	\end{algorithmic}
\end{algorithm}    

Specifically, in \algref{alg:ccw-high:node} we consider a binary tree
with $|\CC|$ leaves, height $\ceil{\log|\CC|}$, where each non-leaf node
has exactly two children.  This is easily done by constructing a
complete binary tree with $2^{\ceil{\log|\CC|}}$ leaves,
and deleting the rightmost leaf repeatedly until there are exactly $|\CC|$ leaves.
If by the end the rightmost leaf is the only child of its parent, we delete
the rightmost leaf repeatedly until this is not the case.

%deleting the
%rightmost $2^{\ceil{\log|C_1|}}-|C_1|$ leaves, and if $|C_1|$ is odd, then
%we ``fold'' the rightmost leaf into its parent (that leaf is the only
%child of that parent). \todo{explain better. not clear, how do you build a tree with $9$ leaves that way?}

We associate each node $y$ in the computation tree with
a cluster $\Clus(y)\in\cC$ and a value $\Val(y)$ as follows: the
processors in $\Clus(y)$ are responsible to compute $\Val(y)$.
Clusters are  assigned to leaves by index:
The $i$-th leaf from the left is associated with the $i$-th cluster of $\CC$.
For internal nodes, we assign the clusters arbitrarily except that we
ensure that no
cluster is assigned to more than one internal node. (This is possible
because in a tree where every node has two or no children, the number
of internal nodes is smaller than the number of leaves.)

The clusters assigned to tree nodes compute the values as
follows (see \algref{alg:ccw-high:node}).
The value associated with a leaf $y_{B}$ corresponding to cluster $B$ is
$\Val(y_{B})=P_B$.
%i.e., the
%combined value of all clusters with index $i$,
%as computed in line \ref{alg:ccw-high:overlap:combine} of \algref{alg:ccw-high:overlap}.
This way, every
leaf $x$ has $\Val(x)$, stored in the leader of $\Clus(x)$,
which can write it to the cloud using \CW.
For an internal node $y$ 
with children $y'$ and $y''$,  the leader of
$\Clus(y)$ obtains $\Val(y')$ and $\Val(y'')$ using \CR, computes
their product $\Val(y)=\Val(y')\otimes\Val(y'')$ and invokes $\CW$ to
write it to the cloud. %\yehuda{should it be written to $h(Iy)$}
Note that the invocations of \CW and \CR in a cluster $B$ are carried using
only the processing nodes of $B$.

Computation tree values are %thus 
filled layer by layer, bottom up.

\para{Remark: Using Flow-Based \CCW.}
We note that in \algref{alg:ccw-high:node},
Lines \ref{alg:ccw-high:node:read1}, \ref{alg:ccw-high:node:read2} 
and \ref{alg:ccw-high:node:write} essentially compute \CAR and \CAW
in which only
the relevant cluster leaders have inputs.
% and the other nodes
% have an input of size $0$. 
Therefore, these calls
can be replaced with a collective
call for appropriate \CAR and \CAW,
making the multiplexing of Line \ref{ccw-1} of \algref{alg:ccw-hi} unnecessary
(similarly to \algref{alg:caw-flow}).
By using  optimal schedules for \CAW and \CAR,
the running-time
can only improve. However, the upper bound of \theoremref{thm-ccw-covers-ub}
still stands.
%is the best possible for some graphs.
%
% as the time complexity of \CAR and \CAW is problematic to compute,
% since it depends on optimal flow solutions.
% We thereby prefer to use \algref{alg:ccw-high:node} as it is,
% for a more explicit and constructive schedule.





%\boaz{rewrite}
%We note that in Step \ref{ccw-high} of \algref{alg:ccw-hi},
%the use of \algref{alg:ccw-high:node} could have been replaced with \algref{alg:caw-flow}
%from \sectionref{sec:va},
%by assigning the input of every cluster leader $r(B)$ to be $P_B$
%(or to be the product of all $P_{B'}$ of clusters $B'$ whose leader is also $r(B)$),
%and assigning $\Unit$ as the input of all nodes that do not lead any cluster.
%Since \algref{alg:caw-flow} operates on all nodes simultaneously using flow-based primitives,
%it could be ran without the need for the multiplexing of Step \ref{ccw-1}
%of \algref{alg:ccw-hi}.
%
%Both algorithms operate in a computation tree fashion (see \figref{fig-tree}),
%and essentially commit a constant number of \CAW and \CAR procedures with $O(|\CC|)$ inputs
%of size $s$ at each layer.
%From \theoremref{????} \todo{add ref}, we know that the complexity of the operations
%in each layer in \algref{alg:caw-flow} is optimal, and thus the complexity
%of each layer in \algref{alg:ccw-high:node}, remains an upper bound.
%Therefore, the time required to perform \algref{alg:caw-flow} is bounded by
%the time analysis of Step \ref{ccw-high}, as stated by \lemmaref{ccw-lem-hi}.
%
%This means that by using \algref{alg:caw-flow} in Step \ref{ccw-high},
%the round complexity of \algref{alg:ccw-hi} can only be improved.



%\subsection{Combining Using Sparse Covers}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%We now arrive at our main theorem.
%which yields an explicit upper bound for any graph $G$,
%which is optimal as is proven in \theoremref{theorem:CCW-LB}, up to a poly-log factor.
%The upper bound is expressed in terms of the cloud clusters of nodes (see \defref{def-Bi}).

\bigskip
\para{Sparse Covers.}
We now arrive at our main result, derived from
\theoremref{thm-ccw-covers-ub}
using a particular flavor of covers.
the result is stated in terms of the maximal timespan of a graph, according to the following
definition:

\begin{definition} \label{graph-Zmax}
	Let $G=(V,E,w)$ be a $CWC$ system with fat links.
	$\Zmax = \max_{i\in V_p} \ZR{i}$ is the \textbf{maximal timespan} in $G$.
\end{definition}
In words, $\Zmax$ is the maximal amount of rounds that is required for any
node in $G$ to write an $s$-bit message to the cloud,
up to a constant factor
(according to \theoremref{theorem:CW_LB}).

\begin{theorem}\label{thm-ccw-ub}
	Let $G=(V,E,w)$ be a \CWC system with fat links, and let $\otimes$
	be a commutative combining operator.
	%   Let $\Zmax = \max_{i\in V_p} \ZR{i}$ be the {maximal timespan} of cloud
	%   clusters in $G$.
	Then \CCW can be solved in $O(\Zmax \log^2 n)$
	rounds.
\end{theorem}
% \todo{we repeat the definition of $\Zmax$ in every theorem. should we add a definition?}


To prove \theoremref{thm-ccw-ub} we use sparse covers, as constructed by Awerbuch
and Peleg.
% Idealy, in order to prove \theoremref{thm-ccw-ub},
% we would have wanted to take the cover $C=\{ \BR{i} \mid i \in V_p \}$ and use
% \theoremref{thm-ccw-covers-ub} on it,
% but unfortunately, $\load(C)$ is not known and may even be
% $\Omega(n)$, and so applying \theoremref{thm-ccw-covers-ub} on $C$ is not enough.

% Instead, our proof will use a theorem presented in \cite{Peleg:book} \todo{change to AP}
% that given a cover of a graph allows to create another cover with some more convenient
% traits, as is shown in the following theorem:

\begin{theorem}[\cite{AP90}]
	\label{thm-AP}
	Given any cover $\CC$ and an integer $\kappa\ge 1$, a cover
	$\CC'$ that satisfies the following properties can be
	constructed in polynomial time.
	\begin{compactenum}[(i)]
		\item \label{sparse:1} For every cluster $B\in \CC$ there exists a
		cluster $B'\in \CC'$ such that $B \subseteq B'$.
		\item \label{sparse:2}
		$\max_{B'\in \CC'} \Diam(B') \le 4\kappa \max_{B \in \CC}
		\Diam(B)$
		\item \label{sparse:3}
		$\load(\CC') \le 2\kappa |\CC|^{1/\kappa}$.
		% 		\todo{make sure that I translated the theorem correctly. it is crucial to the proof and I'm afraid that I missed something...}
	\end{compactenum}
\end{theorem}


% In \theoremref{theorem:CCW-LB} we show that the result is optimal up
% to a polylog factor. 

%The proof of \theoremref{thm-ccw-ub} follows from a more refined
%upper bound in the following lemma.
%% use the following definition.
%
%% \begin{definition}
%%   Let $B_\Diam$ be the cloud cluster with the largest diameter
%%   $\Diam(B_\Diam)$, and let $B_c$ be the cloud cluster with the least
%%   cloud bandwidth $\bc(B_c)$.
%% \end{definition}
%
%\begin{lemma}\label{lemma-ccw-ub-partial}
%  Let $D_{\max}$ be the maximal cloud cluster diameter, and let
%  $B_{\min}$ be the smallest cloud bandwidth of a cloud cluster.
%  Then \CCW can be solved in
%  $O(D_{\max}\log^2 n + {{s}\over{B_{\min}}} \log n)$
%  rounds.
%\end{lemma}
\par\noindent\textbf{Proof of \theoremref{thm-ccw-ub}:~}
Let $\CC$ be the cover defined as the set of all cloud
clusters in the system.
By applying \theoremref{thm-AP} to $\CC$ with
$\kappa = \ceil{\log n}$,
%and noting that $|\CC|=n$.
we obtain a cover $\CC'$
with $\load(\CC') \le 4\ceil{\log n}$ because $|\CC|\le n$.
By \ref{sparse:2}, $\Diam_{\max}(\CC') \le 4\ceil{\log n} \cdot \Diam_{\max}(\CC)$.
% \gal{we should explain why every $B'\in \CC'$ contains some $B\in \CC$}.
%
% We assume that for each $B' \in C'$, there is a $B \in C$ such that $B \subseteq B'$.
% This is true by the construction in \cite{Peleg:book},
% and also because if it were not the case, then by \ref{sparse:1}
% we could have taken a set $C''$
% such that rule \ref{sparse:1} would apply
% by taking one cluster in $C'$ for each cluster in the original $C$ that contains it.
% This also means that $|C'| \le |C|$,
% and therefore, $\log |C'| \le \log |C| = \log n$.
Now, 
let $B' \in \CC'$.
We can assume \WLOG that there is a cluster $B\in \CC$ such that $B\subseteq B'$
(otherwise $B'$ can be removed from $\CC'$).
% Let $B\in \CC$ be a cluster such that $B\subseteq B'$.
$B$ is a cloud cluster of some node $i\in B'$,
and therefore by \lemmaref{lemma:cloud-cluster-timespan} and by
\defref{def-clusters-params}, we get that $Z(B') \le Z(B) = O(\ZR{i}) = O(\Zmax)$.
%Then $\bc(B') \ge \bc(B) \ge B_{\min}$ and therefore
%\begin{equation}
%  \label{eq:sparse}
%  Z(B')
%  ~=~ \Diam(B') + \frac{s}{\bc(B')}
%  ~\le~ D_{\max}4\log n +
%  \log n\frac{s}{B_{\min}}~.
%\end{equation}
Since this bound holds for all clusters of $\CC'$,
$\ZC(\CC') = O(\Zmax)$.

Applying \theoremref{thm-ccw-covers-ub}
to cover $\CC'$ we obtain
% get an upper bound of
% $O(\Zmax(\CC') \cdot (\load(\CC') +\log |\CC'|))$ rounds to complete \CCW,
% and by applying all of the aforementioned statements, this translates
% to 
a time  upper bound for \CCW of
$%O(\Zmax(\CC') \cdot (2\log n +\log n)) = O(\Zmax(C') \log n) =
O\left(\Diam_{\max}(\CC) \cdot \log^2 n + \Zmax \cdot \log^2 n\right)$
rounds .
Finally, let $B_{j} \in \CC$ be a cloud cluster of diameter $\Diam_{\max}(\CC)$.
Recall that by \defref{def-Bi},
$\Diam(B_{j}) \le 2\kR{j} \le  2\ZR{j} \le 2\Zmax$.
We therefore obtain an upper bound of $O(\Zmax \log^2 n)$ rounds.
\QED

% \theoremref{thm-ccw-ub} follows immediately by noting that
% $\Diam(B_\Diam) \le Z(B_\Diam) \le \Zmax$ and
% ${{s}\over{\bc(B_c)}} \le Z(B_c) \le \Zmax$.
% \QED

\smallskip
We close with a lower bound.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{theorem}\label{theorem:CCW-LB}
	Let $G=(V,E,w)$ be a \CWC system with fat links.
	%   , and let $\otimes$
	%   by a commutative combining operator.
	%   Let $\Zmax = \max_{i\in V_p} \ZR{i}$ be the {maximal timespan} of cloud
	%   clusters in $G$.
	Then \CCW requires $\Omega(Z_{\max})$ rounds.
\end{theorem}


% \todo{add corollaries for more topologies, namely: Clique, Tree, d-dimensional torus}





\subsubsection{\CCR}
\label{sec:CCR}
%%%%%%%%%%%%%%%%
To implement \CCR, one can reverse the schedule %and directions of 
\CCW. However, a
slightly better implementation is possible, because there is no need
to ever write to the cloud node.  More specifically, let $\mathcal{C}$
be a cover of $V_p$.  In the algorithm for \CCR, each cluster leader
invokes \CR, and then the leader disseminates the result to all
cluster members.  The time complexity for a single cluster $B$ is
$O(Z(B))$ for the \CR operation, and $O(\Diam(B))$ rounds
for the dissemination of $S$ throughout $B$
(similarly to \lemmaref{lemma:ccw-low-runtime}).
Using the
multiplexing to $\load(\CC)$ as in in Step
\ref{ccw-1} of \algref{alg:ccw-hi}, we obtain the
following result.
% \begin{theorem}\label{thm-CCR-covers}
%   Let $G=(V,E,w)$ be a \CWC system with fat links, and let
%   $\Zmax = \max_{i\in V_p} \ZR{i}$ be the {maximal timespan} of cloud
%   clusters in $G$.   Given  any cover $\mathcal{C}$, \CCR can be performed in
%   $O(\Zmax(\CC) \cdot \load(\CC) + \Diam_{\max}(\CC) \cdot \load(\CC))$ rounds.
% \end{theorem}
% Similarly to the proof of \theoremref{thm-ccw-ub}, using
% \theoremref{thm-AP}, we get the following result.

\begin{theorem}\label{thm-CCR-covers}
  Let $G=(V,E,w)$ be a \CWC system with fat links.
%   , and let $\Zmax = \max_{i\in V_p} \ZR{i}$ be the {maximal timespan} of cloud
%   clusters in $G$.
  Then \CCR can be performed in
  $O(\Zmax \cdot \log^2 n)$ rounds.
%   \todo{we can actually get more refined upper bound of
%   $\\ZC(\CC) \log n + \Diam_{\max}(\CC) \log^2 n $. should we mention it?}
\end{theorem}

% \todo{In the wheel setting, $\load(C) = 2$ and we don't need \cite{Peleg:book},
% and thus the runtime is just $O(\Zmax)$.}

Finally, we note that since any algorithm for \CCR 
 also solves $\CR_i$ problem for every node $i$, we get from
\theoremref{theorem:CR_LB} the following result.

\begin{theorem}\label{thm-AR-LB}
  Let $G=(V,E,w)$ be a \CWC system with fat links.
%   and let $\Zmax = \max_{i\in V_p} \ZR{i}$ be the {maximal timespan} of cloud
%   clusters in $G$.
  Any algorithm solving \CCR requires
  $\Omega(Z_{\max})$ rounds.
\end{theorem}



% \gal{I didn't add here the algorithm for \CCR. In fact, I kept the \CCR subsection
% exactly as it were in the previous submission}

% \gal{I didn't add here the case studies subsection from my thesis.
% do we want it? some of it? maybe in the appendix?}







%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cwc"
%%% End:


==> old/model.tex <==
\section{Model and Preliminaries}
\label{sec:model}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{model-body}

==> old/multiple.tex <==
\section{Communication Primitives in \CWC}
\label{sec:rw}

% \yehuda{
%  Considering copying a file from a node to the cloud, or in the other direction, as a dynamic flow with time horizon the following results are derived. See
%  details in \appref{app:multiple}.
% }
% \boaz
{In this section we state the complexity results for the basic operations of reading and writing to the cloud by one or all processors.
The results are derived using standard dynamic flow techniques. Details are deferred to }\appref{app:multiple}.

\begin{theorem}
  \label{thm-cw}
  Given any instance $G=(V,E,w)$ of the \CWC model, an optimal
  schedule realizing $\CW_i$ can be computed in polynomial time.
\end{theorem}

\begin{theorem}
	\label{thm-cr}
	Given any instance of the \CWC model, an optimal schedule realizing
	$\CR_i$ can be computed in polynomial time.
\end{theorem}

\begin{theorem}
	\label{thm-caw-car}
	Given any instance $G=(V,E,w)$ of the \CWC model, an optimal
	schedule realizing \CAW (\CAR) in which every node $i$ needs to write (read) a message
	of size $s_i$ to (from) cloud node $v_c$ can be computed in strongly polynomial time.
\end{theorem}

\begin{theorem}
	\label{thm-caw-car-multi}
	Given any instance of the \CWC model and $\epsilon>0$, a
	schedule realizing 
	$\CAW$ or $\CAR$ can be computed in  time polynomial in the instance
	size and $\epsilon^{-1}$. The length of the schedule is at most
	$(1+\epsilon)$ times larger than the optimal length.
	%  If all nodes
	%  write to (or read from) the same cloud node, optimal schedules for
	%  $\CAW$ and
	%  $\CAR$ can be computed in strongly polynomial time.
\end{theorem}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cwc"
%%% End:




==> old/old-intro.tex <==
\section{Introduction}
\label{sec:intro}

\ignore{%%%
\paragraph{Background and the new model.}
}%%%



XXX

%%%%%%%   %%%%%%%
\begin{figure*}[t]
  \small
  \centering
  \def \n {7}
  \def \np {(\n+1)}
  \def \radius {1.5cm}
  \def \margin {11}
  \begin{tikzpicture}%[scale=0.6, every node/.style={scale=0.6}]
    % \node[draw, circle, inner color=white,outer color=orange] (mid){$v_c$};
    \node (mid) {};
    \foreach \s in {0,...,\n} {
      \node[draw, circle] (v\s) at ({90-360/\np * (\s )}:\radius) {$v_\s$};
      \draw[line width=2pt] ({360/(\np) * (\s )+\margin}:\radius) 
      arc ({360/\np * (\s)+\margin}:{360/\np * (\s+1)-\margin}:\radius);
      % \draw[-] (mid) -- (v\s);
    }%
    \node at (-90:1.5*\radius) (bot) {Local edges only};
  \end{tikzpicture}
  \hspace*{12mm}
  \begin{tikzpicture}
    \node[draw, circle, inner color=white,outer color=orange] (mid) {$v_c$};
    % \node (mid) {};
    \foreach \s in {0,...,\n} {
      \node[draw, circle] (v\s) at ({90-360/\np * (\s )}:\radius) {$v_\s$};
      % \draw[line width=2pt] ({360/(\np) * (\s )+\margin}:\radius) 
      % arc ({360/\np * (\s)+\margin}:{360/\np * (\s+1)-\margin}:\radius);
      \draw[-] (mid) -- (v\s);
    }%
    \node at (-90:1.5*\radius) (bot) {Cloud edges only};
  \end{tikzpicture}
  \hspace*{12mm}
  \begin{tikzpicture}
    \node[draw, circle, inner color=white,outer color=orange] (mid) {$v_c$};
    % \node (mid) {};
    \foreach \s in {0,...,\n} {
      \node[draw, circle] (v\s) at ({90-360/\np * (\s )}:\radius) {$v_\s$};
      \draw[line width=2pt] ({360/(\np) * (\s )+\margin}:\radius) 
      arc ({360/\np * (\s)+\margin}:{360/\np * (\s+1)-\margin}:\radius);
      \draw[-] (mid) -- (v\s);
    }%
    \node at (-90:1.5*\radius) (bot) {Computing with the cloud};
  \end{tikzpicture}
  \caption{\it Wheel topology with $n=8$.  The $v_i$ nodes are processing
    nodes connected by a ring of high-bandwidth links. The cloud node
    $v_c$ is connected to the processing nodes by lower-bandwidth
    links. All links are bidirectional and symmetric.
  }
  \label{fig-ring}
\end{figure*}


\subsection{The \CWC Model}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In our abstraction, the cloud is a common
storage space, 
% (such as Dropbox, Google Drive, Microsoft's One Drive etc.),
connected to all the nodes in the network
%  Unlike the HYBRID model, we do
% not assume that the limiting factor in accessing the cloud is the
% capacity of the nodes. Rather, we take the view that 
with links of prescribed bandwidth. 
The model,  called ``Computing with the Cloud'' 
(\CWC) is formulated along the following
lines. 
\input{model-body}
\ignore{ %%%%%%%%%%%%
\begin{compactitem}
	\item There are two types of nodes: \emph{Processing nodes} (sometimes
	referred to as \emph{network nodes} or \emph{processors}), that can execute arbitrary
	computations, and \emph{cloud nodes}. Cloud nodes (possibly more
	than one) are passive nodes that function as shared storage: they
	support only read and write requests, and they are connected to all
	(or many) of the processor nodes.  We reiterate: our concept of
	cloud represents storage clouds (such as Dropbox) and not
	computation clouds (such as EC2).
	\item There are two types of links: \emph{local network
		links}, that connect processor nodes to each other, and
	\emph{cloud links}, that connect processor nodes to cloud nodes (no
	link connects two cloud nodes). Links are directed, and each link
	has its prescribed
	bandwidth. 
	% In line with the tremendous progress
	% in communication bandwidth, we abandon the conservative estimate
	% of logarithmic number of nits per round. Typically, the bandwidth
	% available in local links is way larger, albeit not
	% infinite. However,
	% We typically assume that local links have significantly more
	% bandwidth than cloud links.
	% links to the cloud node have distinctly less
	% bandwidth, since they abstract long routes through the
	% Internet.
	\item We consider a synchronous network. In each
	round, the processor nodes may exchange
	messages with each other and with the cloud, where message sizes are
	limited by the  per-round link bandwidths.
\end{compactitem}
%%%%%%%%%%%%%%%%%%%%%%%%%%
We believe that our model is fairly widely applicable.
A processing node in our model may represent anything from
a computer cluster with a single gateway to the Internet, to
cellphones or even smaller devices with non-shared Internet
connection. The local links can range from high-speed fibers to
Bluetooth or infrared links. Typically in this setting the local links
have bandwidth much larger than the cloud links (and cloud downlinks
in many cases have larger bandwidth than cloud uplinks).
Another possible interpretation of the model
is a closed system (say, in a corporation), 
where a cloud node represents a storage or a file
server. In this case the cloud link bandwidth may be as large as the local
link bandwidth.

\ignore{%%%%
	The ultimate goal of this  study is to understand the effectiveness 
	of the \CWC model. We believe that it is applicable in a wide range
	of scenarios.
	Furthermore, we can show that this model helps in designing
	algorithms.}%%%%

}%%%%%%%%%%%%%

\subsection{Problems Considered and Main Results}
\label{sec:problem-statements}
% \boaz{rephrased}
Our main results in this \paper 
are efficient algorithms in
the \CWC model to combine values stored at nodes, 
for example vector addition and matrix multiplication.
To this end, we first show how to implement building blocks 
that allow transmission of large messages
(or files) from processing nodes to the cloud nodes and back, using dynamic flow %with time horizon
techniques.  
Finally,  we show how to use the combining algorithms
to derive new
algorithms for federated learning and file de-duplication (dedup) in the \CWC model.

More specifically, we provide implementations of the following tasks.

%with the architecture described in \figref{fig-api}:
\ignore{%%%
these are high-level tasks invoked by the applications and realized
using the lower-level \FW, \FR to interact with a cloud neighbor, and
message send/receive to communicate with a processor neighbor. 
The tasks we consider are the following.
}%%%


%\begin{wrapfigure}{r}{6cm}
%\centering
%\begin{tikzpicture}[thick,scale=0.7, every node/.style={scale=0.7}]
%\node[draw,text width=2.3cm,minimum height=1cm,align=center] (cloud) at (1.5,1) {cloud node};
%\node[draw,text width=2.33cm,minimum height=1cm,align=center] (neighbor) at (4.5,1) {processor node};
%\node[draw,fill=yellow!80!black,text width=3cm,minimum height=1cm,align=center] (cwc) at (3,3) {\CWC layer};
%\node[draw,text width=3cm,minimum height=1cm,align=center] (app) at (3,5) {application layer};
%\draw [<->] (cloud.north) -- (cwc.south);
%\node[align=left] at (1,2) {\texttt{file}* ops};
%% \node[align=left] at (3,2){read(file, location) \\ write(file, location)};
%\draw [<->] (neighbor.north) -- (cwc.south);
%\node[align=right] at (5.1,2) {send/receive};
%\draw [<->] (cwc.north) -- (app.south);
%\node[align=left] at (2,4) {\textbf{cloud}* ops}; 
%% $\CW_i$(file) \\ \CAW \\ \CAR};
%% \node[align=left] at (3,4.5) {$\CR_i$(file) \\ $\CW_i$(file) \\ \CAW \\ \CAR};
%\end{tikzpicture}
%\caption{\em Task interfaces at a processor.}
%\label{fig-api}
%\end{wrapfigure}

\subsubsection{ Basic cloud operations:}
Let $i$ denote a processing node and let $v_c$ denote a cloud node.
\newline
\emph{$\CW_i$:} write an $s$-bits file $f$ stored at  node $i$ to  node $v_c$.
% Sometimes part of a file is written in which case the index of the bit in which the writing should start is specified.
% A processor writes, i.e., uploads, an $s$-bits string $S$
% to cloud node $v_c$. 

\noindent
\emph{$\CR_i$:} fetch an $s$-bits file $f$
from node $v_c$ to node $i$. 

\noindent
\emph{$\CAW$:} For each node $i\in V_p$, write an $s$-bits file $f_i$ stored at node $i$ to  node $v_c$. 

\noindent
\emph{$\CAR$:} Each node $i\in V_p$ simultaneously fetches a copy of $s$-bits file $f_i$
from cloud node $v_c$ for $i=1, \ldots, n$.
\ignore{%%%%%
for each
processing node $i\in V_p$, fetch from cloud node $v_c$ file $f_i$ to node $i$.
}%%%%%


\ignore{%%%
	The task is invoked by all processors
	together, with two global arguments: a cloud node
	identifier $v_c$ and a name $f$. The goal is to return to all nodes
	the contents of $f$  in $v_c$.
}%%%

\subsubsection{ Combining and dissemination operations:}
\ \ 
\newline
\noindent
\emph{\CCW:} Each processing node $v_i$ has an $s$-bits input string $S_i$, and
there is a binary associative operator
$\otimes:\Set{0,1}^s\times\Set{0,1}^s\to\Set{0,1}^s$
(note that the result is as long as each of the operands). The requirement
is to write to a cloud node $v_c$ the $s$-bits string %$\bigotimes S_i$.
$S_1\otimes S_2\otimes\cdots\otimes S_n$.
% In this problem the processing nodes compute $f(S_0, S_1, \ldots S_{n-1})$ and write the result at a cloud node. 
 Borrowing from Group Theory, we call the operation
$\otimes$ \emph{multiplication}, and $S_1\otimes S_2$ is
the \emph{product} of $S_1$ by $S_2$. In general, $\otimes$ is not
necessarily commutative. % unless explicitly stated otherwise.
We assume the existence of a
unit element for $\otimes$, denoted $\Unit$, such that
$\Unit\otimes S=S\otimes\Unit=S$ for all $s$-bits strings $S$. The
unit element is represented by a string of $O(1)$ bits.
For example, $S_i$ could be vectors and $\otimes$ vector addition (or the
$S_i$'s could be square matrices and $\otimes$ could be matrix multiplication).
%We distinguish between the case in which $f$ is associative or not.
Examples for commutative operators include
vector (or matrix) addition over a finite field,
bitwise operations such as \texttt{and}, \texttt{or} and \texttt{xor},
leader election, % (with operand size $s = \log n$),
and the top-$k$ problem. % (with operand size $s= k\log n$).
Examples for non-commutative operators may be
matrix multiplication (over a finite field) and
function composition. % such as permutation combining
% (with $s$ being the size of the domains and codomains of all functions).

\noindent
\emph{\CCR:} All the nodes $i\in V_p$ simultaneously fetch a copy of an $s$-bits file $f$
from  node $v_c$. (Similar to network broadcast.)


\subsubsection{Applications:}
First, notice that \CCW and \CCR can be used directly to provide matrix multiplication,
matrix addition, and vector addition. We also outline the implementation of the following.

\noindent
\emph{\bf{Federated learning (FL)} \cite{federated-17}:} In FL, a collection of distributed devices collaborate in training a
neural network to construct a model of some concept, but do not wish to send
their data as is to other nodes (providing some sense of privacy). 
Unlike \cite{federated-17}, in our model the central server is 
a passive storage device that does not carry out computations.
We show how  elementary secure computation techniques, along with our
combining algorithm, can efficiently help  training an ML model in the federated scheme
implemented in \CWC, while maintaining privacy.

\noindent
\emph{\bf{File de-duplication:}} 
Finally, we show how to use \CCW with \CCR to efficiently solve the
de-duplication problem (see, e.g., \cite{dedup-performance}). Deduplication
(or dedup) is a basic tool in file stores, where
redundant identical copies of a file (or part of file) are identified (and possibly deleted, keeping one copy).
We implement file de-dup in the \CWC model on collections of files stored at the different processing nodes. The algorithm keeps one copy of each replica and a pointer to where the copies were stored.

% \yehuda{no definition for non-associative function?,  What about other problems, Federated Learning?}
\ignore{%%%
	The task is invoked by all processors
	together. Each processor $i$ has a bitstring $S_i$, all of the same
	length $s$. There are also two global arguments: a cloud node
	identifier $v_c$ and a name $f$. The goal is to write in $v_c$, under
	the name $f$, the value of
	$\bigotimes_{i=0}^n S_i$, under the assumption that $\otimes$ is an
	associative operation.
}%%%

%First, we note that once we require that an invocation of a task
%requires a ``completed'' response at the invoking processor, read and
%write are essentially the same task, reversed: Suppose we are given an
%execution of \CW invoked by $i$ with string $S$ and name $f$. Then
%viewing  the response as
%an invocation, and letting messages flow in the reversed direction,
%ends with $S$ (the contents of $f$) delivered at $i$, i.e., a response
%for a \CR. We therefore concentrate henceforth on writing, without
%loss of generality.
%
% \ \ \ 
 
% \noindent
% \emph{\bf{Schedules:}}
Our goal in all the tasks and algorithms %, for all these tasks, 
is to find a schedule that implements the task in the minimum amount of time.
\begin{definition}\label{def-sched}
  Given a \CWC model, a \textbf{schedule} for time interval
  $I$ is a mapping that assigns, for each time step in $I$ and each link $(u,v)$: a send
  (or null) operation
  if $(u,v)$ is a local link, and a \FW or \FR (or null) operation if $(u,v)$ is a
  cloud link.
\end{definition}


\ignore{%%%%%%
Within this model, we formalize and analyze a few primitive tasks
that can be useful for general computations.  % We focus on a
% particularly simple topology (see \figref{fig-ring}), in which the
% processing nodes are arranged in a ring. In this
% model,
Specifically, we provide efficient implementations for the following  building
blocks and applications:
%
% \todo{no longer true. Elaborate that we support general topologies now,
% with the assumption of wide local links...}
% \ignore{%%%%%%%
% \paragraph{Our results.}
% In this work, we focus on a particularly simple topology (see
% \figref{fig-ring}), in which the processing nodes are connected
% by local edges as a ring, and they are all connected to a single cloud
% node. This wheel-shaped topology allows us to study the effect of
% the direct cloud links on a distance-constrained local network. This
% topology also abstracts the scenario in which local processing nodes
% communicate only to their nearest neighbors, say by short-range,
% high-bandwidth wireless links. We consider both the \emph{general wheel
% model}, where links may have different bandwidths, and the
% \emph{uniform wheel model}, in which all local links have the same
% bandwidth and all cloud links have the same bandwidth. We provide the
% following results.
% }%%%%%%%

\para{Basic file operations: \CW, \CR, \CAW, \CAR}. 
%
In \CW, a file held by a processor node
needs to be written to
a cloud node. In \CR, a file stored in a cloud node needs to be fetched to
a requesting node. In \CAW each processing node has a file to write,
and similarly in \CAR each node requests a file to read from a
cloud node.
% \CCR is similar to broadcast in networks: The requirement is to
% disseminate a file stored in the cloud to all processing nodes.
Using flow techniques, we provide time-optimal algorithms for these
tasks in general directed weighted graphs.
}%%%%%%

\noindent\textbf{Special topologies.}
The precise complexity of each of these tasks depends on the
given network topology, and we therefore study a few cases of interest.  %  (see \theoremref{theorem:two_sided_UB} and
% \defref{def-Ii})
%\smallskip
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

First, we consider \textbf{$s$-fat-links} network, defined to be, for
a given parameter $s\in\mathbb{N}$, as the \CWC model with the following additional assumptions:
\begin{compactitem}
\item All links are bidirectional and symmetric, i.e., $w(u,v)=w(v,u)$ for every link $(u,v) \in E$.
\item Local links have bandwidth at least $s$.
\item There is only one cloud node $v_c$.
\end{compactitem}
% where we assume that
% all links are bidirectional, and that the bandwidth
% of every local link is at least $s$, the number of bits in the
% operands. No other assumptions are made in this case.
% \boaz{new} 
The fat links model seems suitable in many real-life cases where
local links are much wider than cloud links (ulinks to the Internet), as is the intuition
behind the HYBRID model \cite{AHKSS20}.

Another topology we consider is the \textbf{wheel network}, depicted
schematically in \figref{fig-ring} (right).
In a wheel topology there are $n$
processing nodes denoted $0,\ldots,n-1$ arranged in a ring, and exactly one cloud
node $v_c$ connected to  all processing nodes.
% We refer to link $(i,i+1)$ as the
% \emph{clockwise} %\gal{(or right)} 
% link of $i$, and to link $(i-1,i)$ as the
% \emph{counterclockwise} %\gal{(or left)} 
% link of $i$ (throughout, node indices are to be taken modulo $n$).
%
\emph{The uniform wheel} is a wheel network
where all cloud links have the same bandwidth $b_c$ and all local links have
the same bandwidth $b_l$. In the uniform wheel
model,  we typically assume that
$\bc\ll\bl$.

% \boaz{new} 
The wheel network is motivated by non-commutative combining 
operations, where the order of combining inputs induces a
linear order on the processing nodes, i.e., a line of
nodes, where node 0 holds the first input, node 1 the second input etc. Connect the first and the last node for symmetry,
and  connect a cloud node to all---and viol\'a, the wheel.
\ignore{%%%
\begin{definition}\label{def-wheel}
  The \textbf{$n$-wheel model} is a graph $G=(V,E,w)$. The node set is
  partitioned $V=V_p\cup V_c$, where the \textbf{processor nodes} are
  $V_p=\{0,\ldots,n-1\}$, and the \textbf{cloud nodes} are $V_c=\Set{v_c}$.
  The \textbf{local links} are $E_L = \{(i, (i+1)\bmod n) \mid 0 \le i <
  n \}$, and the \textbf{cloud links} are
  $E_C = \{ (i, v_c) \mid 0 \le i < n \}$.%
  \footnote{Throughout this paper, when referring to node $i+1$ where
    $i\in V$, addition is to be taken modulo $n$. The bandwidth of each
    link $e$ is given by $w(e)\in\mathbb{N}$.
  }
\end{definition}
}%%%
% For brevity, we denote $w(i,v_c)$ by $\bc(i)$ and refer to it as the
% \emph{cloud bandwidth} of $i$.
%
%

% Note that otherwise, i.e., if $\bc=\Omega(\bl)$, then
% for the tasks
% considered here,   completely ignoring the local links incurs  only a
% constant-factor blowup in the time complexity.

%\smallskip
%\noindent\textbf{Dynamic flows.}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cwc.tex"
%%% End:

% \boaz{this repeats the paragraph from p.1}
% For a particularly simple case, consider \CW of an
% $s$-bits file in the uniform $n$-node {wheel},
% which is described as follows.
% In a wheel
% (see \figref{fig-ring}),
% processing nodes are connected as a ring, and they are all connected to
% a single cloud node. All links are bidirectional,
% cloud links have the same bandwidth $b_c$ and local links have the same bandwidth $b_l$.
% %and cloud link and local link bandwidths are $\bc$ and $\bl$, respectively. 
% Without using the cloud 
% (\figref{fig-ring}, left), one may replace \CW by a broadcast. However,
% disseminating any message to all nodes takes $\Omega(n)$ 
% rounds due to the 
% distance that must be covered; on the other hand, without using the
% local links (\figref{fig-ring}, middle), \CW and \CR require
% $\Omega(s/\bc)$ rounds due to the limited bandwidth. But in the 
% \CWC model, $\Theta (\sqrt{s/\bc} )$ rounds suffice to do \CW
% (or \CR), assuming that the local link bandwidth is large enough.% 
% \footnote{ The time complexity is $O(\sqrt{s/\bc})$ if
% 	% $\bl\ge\sqrt{s\cdot\bc}$
% 	$s\le\bc\bl^2$ or $O(s/\bl)$ otherwise.  See \corollaryref{cor-ub}.
% }
%
% This is a significant improvement when compared to
% approaches that do not use both local and cloud links: Disseminating
% the file to all nodes without the cloud (\figref{fig-ring}, left)
% takes $\Omega(n)$ rounds due to distance that must be covered, and
% that writing the file to the cloud without being helped by the local
% links (\figref{fig-ring}, middle) requires $\Omega(s/\bc)$ rounds due
% to the limited bandwidth.
For example, if $s=n$ and the cloud link bandwidth is $\bc=\sqrt n$, then
dissemination is completed in $O(n^{1/4})$ rounds (assuming that the local link
bandwidth $\bl$ is at least $\Omega(n^{3/4})$). %\boaz{omit last sentence?}


\ignore{%%%%%%% 

\para{Combining and dissemination: \CCW, \CCR.}
% These tasks are
% similar to broadcast and convergecast in networks \cite{Peleg:book}.

%The \CCW task is the \CWC analog to
% convergecast~\cite{Peleg:book}. Specifically,
In \CCW, we are given an associative operator denoted $\otimes$
that maps a pair of $s$-bit operands to an $s$-bit result. 
Each node $i$ has a %n $s$-bits
string $S_i$ and the task is to write $\bigotimes_{i}S_i$ to a cloud node,
%for some associative binary operator $\otimes$, 
assuming that the
result is also an $s$-bit string.
% $f(v_1, v_2, \ldots v_n)$ must be written to the cloud.
% % (and from there to all nodes).
% Typical examples may be writing to the cloud the sum of
% $n$ vectors, or the product of $n$ matrices.
% The
% algorithm in this case may split and combine each input to pieces and
% compute $f$ on the fly as the pieces traverse the network. 
Our first major technical result, described in \sectionref{sec:va}, is a
near-optimal algorithm for commutative operators (such as
vector addition) in the case of \emph{fat links networks}, where the bandwidth of
all local links is at least $s$ bits per round
(\theoremref{thm-ccw-ub}).

%In \subsectionref{sec:CCW-asymmetric} we extend our results to the case of asymmetric
%cloud links, in which the download speed and the upload speed of a processing node
%may differ. This case represents more accurately many real life scenarios,
%as upload rates are often slower than download rates over the Internet.

In the case of a non-commutative operator
(e.g., matrix multiplication), there is a given linear order of the
operands, and thus results depend greatly on the assumption of how are
operands distributed over nodes.  In \subsectionref{sec:wheel}
we study a simple case, where the nodes are linearly ordered as in
the wheel topology (\figref{fig-ring}), and present direct
construction that facilitate an improved algorithm for
\CCW for any given link bandwidths.
% , whose complexity is within a logarithmic factor from
% optimal \boaz{fill from sec.5} (\theoremref{??}).
% In fact, the
% algorithm can be used to compute all prefix sums \cite{LadnerF-80}
% (\theoremref{thm-prefix}).
% to constant . We
% distinguish between two cases. In the \emph{holistic} case, one needs
% the whole operands to compute the result (this is the case, for
% example, with matrix multiplication); and in the \emph{modular} case (e.g., in vector addition), given aligned parts of two
% operands, one can compute the corresponding part of the result. The
% modular case allows for pipelining, which speeds up the computation by
% a logarithmic factor (\theoremref{thm-aw-modular}).
% We note that in \CCW, nodes apply the operator to
% messages as they flow through the network (see, e.g.,
% \cite{leighton-book}), 
% % \gal{why assumed? this is our implementation, we have them do that, it is not an assumption. I think this sentence is redundant}
% as is the case when nodes hold matrices and the
% goal is to write a product (or the sum) of these matrices.

The task of \CCR is analogous to standard network
broadcast~\cite{Peleg:book}: the goal is to disseminate an $s$-bit
file stored in the cloud to all processor nodes. Timewise, \CCR can be
viewed as the reverse of \CCW, but since we assume that concurrent
reads are allowed, we are able to provide improved complexity results
(\theoremref{thm-ccr-gen} and \theoremref{thm-CCR-covers}).

}%%%%%%%


\subsubsection{Overview of techniques.}
For the basic file operations, \CW, \CR, \CAW and \CAR,
an optimal schedule is provided based on \emph{dynamic flow} techniques,
or more specifically, \emph{quickest flow}, which have been studied in
numerous papers in the past (cf. \cite{quickest, Skutella-flows}). See
\subsectionref{ssec:dynamic} and \sectionref{sec:rw} for more details.
However, a closed-form expression
for the time complexity of these schedules
for general graphs is not known.
%as well as an optimal schedule for the tasks of
%\CAW and \CAR.
We consider the tasks of \CW and \CR on some more restricted topologies.

In \subsectionref{sec-fat-combining},
we present tight lower and upper bounds for \CW and \CR in the \textbf{$s$-fat-links} network, where $s$ is the input size at each node.
\ignore{We skip the exact expressions here, since they are quiet involved,
depending on the topology and link capacities of the graph.}%%
Let $\ZR{i}$ denote the upper (and lower) bound on the time complexity of \CW
(and \CR), that is initiated by node $i$, as proven in \theoremref{theorem:CW_UB}
(see \defref{def-Bi}).
We then continue to consider the tasks \CCW with \emph{commutative operators}
and \CCR, and
%present tight bounds up to a polylog factor
prove a near optimal
upper bound for their time complexity in the \textbf{$s$-fat-links} network, of
$O(\max_i \ZR{i} \cdot \log^2 n)$ (\theoremref{thm-ccw-ub})
% ,
% \theoremref{thm-CCR-up})
as well as a lower bound of $\Omega(\max_i\ZR{i})$ (\theoremref{theorem:CCW-LB},
\theoremref{thm-AR-LB}).

The main strategy of our algorithms is to first find, for every processing node $i$,
a cluster of processing nodes that allows it to perform \CW in $\ZR{i}$ rounds.
We then perform \CCW by combining the values
within every cluster using convergecast \cite{Peleg:book},
and then combining the resulted products in a computation-tree fashion.
Using the sparse covers construction of Awerbuch and Peleg \cite{AP90},
we obtain a cover that allows to perform the described procedure
in near-optimal time (see \theoremref{thm-ccw-ub}).

For the case of \emph{non-commutative operators}, a natural order of the nodes is
derived from the requested order of the operands, and hence we consider these operators
on a graph of the wheel topology, as depicted in \figref{fig-ring}.
This time around, due to the restricted topological assumptions,
we present algorithms for wheel graphs with \emph{arbitrary} bandwidth, both for cloud
links and for local links.
Once again, we denote by $\ZR{i}$ the tight upper and lower bound of \CW and \CR
from node $i$ (\defref{def-Ii}).
We prove an upper bound for \CCW
in this scenario of $O(\max_i \ZR{i} \cdot \log n)$ in \theoremref{thm-ccw-intervals-ub}
and a lower bound of $\Omega(\max_i\ZR{i})$ in \theoremref{thm-aw-lb}.

Finally, in \sectionref{sec:applications}, we demonstrate how the considered tasks
can be applied for the purposes of Federated Learning and File Deduplication.




\subsection{Related Work}
\label{app-related}
%%%%%%%%%%%%%%%%%%%%%%%%%
Our model is based on, and inspired by, a long history of theoretical
models in distributed computing. To gain some perspective, we offer
here a brief review.
% More details are provided in
% \sectionref{sec-related}.


Historically, distributed computing is split along the dichotomy of
message passing vs shared memory~\cite{Pierre10}. While message
passing is deemed the ``right'' model for network algorithms, the
shared memory model is the abstraction of choice for programming
multi-core machines. 

The prominent message-passing models are LOCAL~\cite{L92},
and its derived CONGEST~\cite{Peleg:book}. In these models, a system
is represented by a connected (typically undirected) graph, in which
nodes represent processors and edges represent communication links.
\ignore{
The basic actions are message send (initiated by processors) and
message receive (initiated by links). Local computation is assumed to
be unbounded and instantaneous, so that the running time of a network
algorithm is just the number of communication rounds it requires.
%
In the LOCAL model, message size is unbounded, and therefore the only
restriction for a node to retrieve any piece of information  is
the number of hops separating the node from the location of that
information.
% As a consequence,  a statement
% of the form ``node $v$ can output after $t$ rounds'' means that the output at
% node $v$ is independent of any input (value or action) located more
% than $t$ hops away from $v$ \cite{L92}. This property makes LOCAL
% a clean model to analyze locality in graph problems.
%
The CONGEST model is a refined version of LOCAL, with the additional
restriction that messages may be only $O(\log n)$-bits long, where $n$ is the number of
nodes.%
\footnote{%
	More precisely, the number of bits in a message is a parameter of
	the CONGEST model, and the default value of that parameter is
	$O(\log n)$.  This value is chosen for reasons similar to the choice
	of word size in the sequential RAM model~\cite{AhoHU74}: this way, a
	message can contain a constant number of references to nodes and
	edges, and possibly other
	variables whose magnitude is bounded by a polynomial in $n$.
	%
}
} In LOCAL, message  size is unbounded, while in CONGEST, message
size is restricted, typically to $O(\log n)$ bits.
Thus, CONGEST % is traditionally
% thought of as more realistic than LOCAL, as it
accounts not only for the
distance information has to traverse, but also for information volume  
and  the
bandwidth available for its transportation.

% It is important to note that in the absence of faults, both network
% algorithms models can be assumed synchronous: If processors and links
% are reliable but run in different speeds, one can use a
% synchronizer~\cite{A-85} to hide these differing speeds, allowing
% algorithms to be developed in the synchronous model (in which
% processors advance in lockstep rounds, where each round consists of
% receive-compute-send substeps).
While most algorithms in the LOCAL and CONGEST models assume
fault-free (and hence synchronous) executions, in the distributed
shared memory model, asynchrony and faults are the primary source of
difficulty. Usually, in the shared memory model one assumes that there
is a collection	 of ``registers,'' accessible by multiple threads of
computation that run at different speeds and may suffer crash or even
Byzantine faults (see, e.g., \cite{AttiyaW}). The main issues in this
model are coordination and fault-tolerance. Typically, the only
quantitative hint to communication cost is the number and size of the
shared registers.

%%%%%%%%
%\ignore{
Quite a few papers consider the combination of message
passing and shared memory, e.g., 
\cite{MNV,FKK,logp-new,qsm,BSP,AdlerGMR-99}.
The uniqueness of the \CWC model with respect to past work is that it  combines passive storage nodes with a  message passing network with restrictions on the links bandwidth.
%}
\ignore{
%%%%%%%%%%%%%%%%%%%%%%%
An early attempt to somehow
restrict bandwidth in parallel computation, albeit indirectly, is due
to Mansour et al.~\cite{MNV}, who considered PRAM with $m$ words of
shared memory, $p$ processors and input length $n$, in the regime
where $m\ll p\ll n$. The LogP model~\cite{logp-new} by Culler et al.\
aimed at adjusting the PRAM model to network-based realizations.
Another proposal that models shared memory
explicitly is the QSM model of Gibbons et al.~\cite{qsm}, in which
there is an explicit (typically uniform)  limit on the bandwidth
connecting processors to shared memory. QSM is 
similar to our \CWC model, except that there is no network connecting
processors directly. A thorough comparison of bandwidth limitations in
variants of the BSP model~\cite{BSP} and of QSM is presented by Adler et
al.~\cite{AdlerGMR-99}.  We note that LogP and BSP do not
provide  shared memory as a primitive object: the idea is to describe
systems in a way that allows implementations of abstract shared memory.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Another proposal that combines message passing with shared memory
is
the ``m\&m'' model, recently proposed by Aguilera et
al.~\cite{ABCGPT18}. The m\&m
model assumes that processes can exchange messages via
a fully connected network, and there are shared registers as well,
where each shared register is accessible only by a subset of the 
processes.
The focus in~\cite{ABCGPT18} is on solvability of distributed tasks in 
the 
presence of
failures, rather than performance.
}

% Recently, with the advent of massive data centers and high-bandwidth
% communication, new variants were proposed to facilitate  a formal study
% of algorithms in these environments. 
%We mention here two.  
The CONGESTED CLIQUE (CC) model~\cite{LotkerPPP-05}
is a special case of CONGEST,
where the underlying communication graph is assumed to be fully
connected. % (i.e., a clique over the processors). % In this model, all
% information is reachable within 1 hop---but it can be retrieved only
% in quanta of $O(\log)$ bits. Theoretically, one can view  CC as an
% orthogonal model to LOCAL: whereas in LOCAL the only constraint is
% length (distance), in CC the only constraint is width (congestion).
% Practically, i
The CC model is appropriate for computing \emph{in} the cloud, as it
% Even though the model was originally conceived for theoretical study, 
% it 
has been shown that under some relatively mild
conditions, algorithms designed for the CC 
model can be implemented in the MapReduce model, i.e., run in 
datacenters~\cite{HegemanP-15}. Another model for computing in the
cloud is the MPC model~\cite{KSV10}. 
%
% Thus it appears that the long-accepted model of communication modeled
% by graph is losing prominence in the message passing world, even
% though the actual underlying hardware works by message passing.
Very recently, the HYBRID model~\cite{AHKSS20} was proposed as a 
combination of CC
with classical graph-based communication. % The HYBRID
% marries the LOCAL and the CC models as follows. T
More specifically, the HYBRID model assumes the existence of  two
communication networks: one for local communication between neighbors,
where links are typically of infinite bandwidth (exactly like LOCAL);
the other network is a \emph{node-congested} clique, i.e., a node can
communicate with every other node directly via ``global links,'' but
there is a small upper bound (typically $O(\log n)$) on 
the total number 
of messages a node can
send or receive via these global links in a round.
Even though the model was presented only recently, there is already 
a line of algorithmic work in it, in particular for computing
shortest paths~\cite{AHKSS20,KS-20,CLP20}.
% (we stress again that the
%capacity restriction does not apply
%to the local links).

%%%%  %%%%%
\textbf{Discussion.} Intuitively, our  \CWC model can be viewed as
the classical 
CONGEST model over the processors, augmented by
special cloud nodes  (object stores)
connected to some (typically, many) compute nodes.
To reflect modern demands and availability of resources, we relax the 
very stringent bandwidth 
allowance of
CONGEST, and usually envision networks with much larger link
bandwidth (e.g., $n^\epsilon$ for some $\epsilon>0$).

Considering previous network models, it appears that  HYBRID  is
the closest to  \CWC, even though HYBRID
was not expressly designed to model the cloud. In our view,
\CWC is indeed more 
appropriate for computation with  the cloud. First, % it appears that 
in most
cases, global communication (modeled by clique edges in HYBRID) is 
limited by link bandwidth, unlike 
HYBRID's
node capacity constraint, which seems somewhat artificial. Second, HYBRID is 
not readily amenable to  model multiple clouds, while this is a
natural property of \CWC . 
%Third,
%the focus in the HYBRID model papers \cite{AHKSS20,KS-20} is on graph
%topology problems, which appear less useful, in some sense, in the
%presence of global communication such as a clique of a cloud, since
%global links distort topology in a deep sense.

Regarding shared memory models, we are unaware of topology-based
bandwidth restriction on shared memory access in distributed
models. In some general-purpose parallel computation models (based on 
BSP~\cite{BSP}), communication capabilities are specified using a 
few
global parameters such as latency and throughput%  (see
% \sectionref{sec-related})
, but these models deliberately abstract topology away.
% (with the exception of \cite{MNV}, see
% \ref{sec-related}).
In distributed (asynchronous) shared memory, the number of bits 
that need to be
transferred to and from the shared memory is seldom explicitly
analyzed. 
%Our modeling of explicit communication with the shared
%storage may therefore be useful even without local
%communication links.



%Due to space consideration, we defer discussion of related work to \appref{app-related}.

\noindent \textbf{Paper organization.} 
In \sectionref{sec:rw} we study collaborative reads and writes in the
\CWC model. In \sectionref{sec:va} we consider \CCW and \CCR in
general networks and in fat links networks.  In \sectionref{sec:wheel}
we consider \CCW for non-commutative operators in the wheel topology.
In \sectionref{sec:applications} we consider application level usage
of the \CWC model, such as federated learning and
deduplication. Conclusions and open problems are presented in
\sectionref{sec:conc}.
Due to space limitations many details and proofs appear in an appendix.




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cwc"
%%% End:


==> old/singlewheel.tex <==
\def\tp{\!+\!}
\def\tm{\!-\!}

\section{\CR and \CW In Wheel Systems}
\label{OLD:sec:rw}

In this section we study the basic tasks of $\CW$ and $\CR$ in the
general wheel system.
We use the subscript $i$ to denote the originating processing node: in
$\CW_i$, an $s$-bits file stored in node $i$ needs to be written to $v_c$,
and in $\CR_i$, an $s$-bits file stored in the $v_c$ needs to be
copied to $i$.
We start with an algorithm for $\CW_i$ in
\sectionref{ssec:write_one_sided}, present a lower bound in
\sectionref{single-lb}, and in \sectionref{ssec:CR} argue
that the same analysis holds for \CR as well.


\subsection{\CW: Upper Bound}
\label{OLD:ssec:write_one_sided}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%	
For ease of presentation we consider the ``one sided'' case in which
node $i$ does not use one of its incident ring links.  As we shall
see, this limitation does not increase the time complexity by more
than a constant factor. Hence we consider the case in which node $i$
cannot send messages on its counterclockwise link.  \ignore{
\begin{lemma}\label{OLD:lem-oneway-ub}
  Let $T_\ell(s)$ and $T_r(s)$ denote the minimal number of rounds
  required to write an $s$-bits file to $v_c$ without sending any
  messages on link $({i},{i\tp1})$ ($({i\tm1},{i})$, resp.).  
Then there exists an algorithm that writes an $s$-bits
  file to $v_c$ while sending messages on 
  both $({i},{i\tp1})$ and $({i\tm1},{i})$ in at most $O(\min(T_\ell(s)),T_r(s)))$ rounds.
\end{lemma}
}
\ignore{%%%%%%%%%
%In light of the simplification presented in \lemmaref{lem-oneway-ub},
Henceforth, we consider the \emph{one-sided} $\CW_i$ task, in which 
% \begin{definition}
%   The $\uploadproblem(i, s)$: The system has the wheel topology, as
  %described in \defref{def-wheel}.  % A given node $i$ stores a
%   file (bit-string) of length $s$. The requirement is that the file
%   will be written to the cloud.
% \end{definition}
%In this task, only one of the local link of $i$ may be used to solve the \CW task.
node $i$ may not send messages on $(i, i\tm1)$: it may use only
$(i,i+1)$, and its cloud link. Obviously, our analysis applies also to
the symmetric case where $i$ may not use $(i,i\tp1)$.
}%%%%%%%%%

% \yehuda{Gal, can you please add a high level intuitive explanation of the algorithm here}
We present pseudocode in \algref{alg:cw-hi}.  The intuition behind the
algorithm is to find out how far clock-wise should node $i$ seek help
in uploading the file.  Consider a processing node $l$, $h$ hops
clock-wise from node $i$ with a large bandwidth link to the cloud node
$v_c$: should $i$ try to forward part of its file to $l$ for
transmission to $v_c$?  If $i$ and all the other $h$ nodes on the path to
$l$ have zero bandwidth links to $v_c$ then clearly yes, but if on the
other hand the total bandwidth to the cloud of these nodes is large
enough to send the file to $v_c$ then the answer is no. Since by the
time ($h$ rounds) the data arrives at $l$ it could have been sent
already to $v_c$.  Thus sending parts of the file farther in the
clock-wise direction becomes useless as both the distance from $i$
increases, and the bandwidth to the cloud along the path increases as
well.  In other words, as data is sent farther clock-wise, more
cloud bandwidth becomes available, but more time is required to reach
it. In addition, narrow bandwidth on the local links may limit the
reachability of cloud bandwidth of remote nodes.  Fortunately, in the
wheel topology, we can easily find the sweet spot that balances the
constraints optimally (up to a constant factor).
% interval of processors, which balances the tradeoff
% between the available bandwidth from the interval to the cloud, and
% the distance that needs to traversed to get to that bandwidth (the
% interval length). Due to \lemmaref{lem-oneway-ub}, it is sufficient to
% look at intervals with $i$ as an endpoint (``one-sided'' intervals).
% required to send $s$ bits to all nodes in the interval through the \emph{local} network,
% and the time required to send $s$ bits through the \emph{cloud} network
% when all nodes of the interval are working together.
% we first find for the initiating node $i$
% its \emph{one-sided} interval that 
Given the optimal interval of nodes, we further simplify the algorithm
(paying another constant factor in its time complexity)  
by first sending the entire file along the interval and then 
each node on the interval writes a chunk of the file to the cloud,
where the chunk size of node $j$ is proportional to $j$'s cloud bandwidth, $w(j,v_c)$.

Formally, let us first define intervals on the ring and their parameters.
\begin{definition}\label{OLD:def-intervals}
	%Let $G=(V,E,w)$ be an $n$-node wheel graph.
  An \textbf{interval}
  $\interval{i}{i\tp k}\DEF\Set{i,i\tp 1,\ldots,i\tp k}\subseteq V$ in a
  given wheel graph is a path
  of processing nodes on the ring. Given an interval $I=[i,i+k]$,  $|I|=k+1$ is its \textbf{size}, and $k$ is its
  \textbf{length}.  The \textbf{cloud bandwidth} of $I$,
  denoted $\bc(I)$, is the sum of the cloud bandwidth of all nodes in
  $I$: $\bc(I)=\sum_{i\in I}\bc(i)$.  The \textbf{bottleneck
    bandwidth} of $I$, denoted $\blmin(I)$, is the smallest bandwidth
  of a link in the interval:
  $\blmin(I)=\min\Set{w(i,i\tp1)\mid i,i\tp1\in I}$.  If  $|I|=1$, define $\blmin(I) = \infty$.
\end{definition}
%
% The \emph{cloud bandwidth} of an interval $I$, denoted $\bc(I)$, is
% the total bandwidth of cloud edges emanating from $I$. Formally,
% $\bc(I)=\sum_{i\in I}\bc(i)$.\\ 
%We now define, for any processor node $i$, a special interval. The
%definition is constructive and plays a key role in the algorithms
%ahead.
%We further define the following notions for each node $i\in V_L$.
%
\begin{definition}\label{OLD:def-Ii}
  Let $i$ be a processing node. We define the following quantities for
  clockwise intervals; counterclockwise intervals are defined
  analogously. 
\begin{compactitem}
\item \label{OLD:def:kc}
  $\kCR{i}$ is the length
  of the smallest interval starting at $i$, for which the product of
  its size by the total bandwidth to the cloud along the interval
  exceeds $s$,  i.e.,
  $\kCR{i}=\min\Set{k\mid \left(k\tp 1\right) \cdot \bc([i,i\tp k]) \ge
    s}$. $\kCR{i}=n$ if no such integer exists.
\item \label{OLD:def:kl}
  $\kLR{i}$ is the length
  of the smallest clockwise interval starting at node $i$, for which the bandwidth
  of the clockwise-boundary link bandwidth is smaller than the total
  cloud bandwidth of the interval, i.e.,
  $\kLR{i}=\min\Set{k\mid w(i\tp k,i\tp k\tp 1)<\bc(\interval{i}{i\tp k})}$,
  or $n$ if no such integer exists.
\item $\kR{i}= \min\Set{\kCR{i}, \kLR{i}}$.
\item $\IR{i} = \interval{i}{i\tp \kR{i}} $. The interval $\IR{i}$ is
  called the (clockwise) \textbf{cloud interval} of node $i$.
\item $\ZR{i} = |\IR{i}| + \dfrac{s}{\blmin(\IR{i})} +
  \dfrac{s}{\bc(\IR{i})}$. $\ZR{i}$ is the \textbf{timespan} of the
  (clockwise) cloud interval of $i$.
	% \item	
	% 	Define $\bLminR{i} = \min\limits_{i \le j \le i+\kR{i}
        % 	- 1}{\bL{j}{j+1} }$ if $\kR{i} \ne 0$, or
        % 	$\bLminR{i}=\infty$ otherwise.
   \end{compactitem}
\end{definition}
Note that $\kR{i}$ is easily computable. The algorithm for \CW
(\algref{alg:cw-hi}) is specified
using the cloud intervals.
Its complexity is given in the following theorem.
% We now state and prove the upper bound.
% A matching lower bound is shown in \theoremref{theorem:one_sided_LB}.

%Note that \defref{def-Ii} refers to a cloud interval ``to the right'' of
%node $i$; analogous definitions apply to an interval
%$\Set{i \tm k,i \tm k \tp 1,\ldots,i}$ to the left of $i$.
%\subsubsection{Upper Bound}

%We are now ready to state our upper bound.
\begin{theorem}\label{OLD:theorem:one_sided_UB}
  \algref{alg:cw-hi} solves the $s$-bits $\CW_i$ problem %from node $i$
  without using link $({i \tm 1}, i)$ in  $O(\ZR{i})$ rounds.
\end{theorem}

\begin{algorithm}[t]%[H]\small
  \caption{$\CW_i$}
  \label{OLD:alg:cw-hi-old}
  \begin{algorithmic}[1]
    \STATE \label{OLD:cw-alg-send-local}
    forward $S$ from node $i$ to all nodes in $\IR{i}$
    \FOR{ all $j\in\IR{i}$, in parallel}
    \STATE\label{OLD:cw-alg-node-write}{
      node $j$ writes to the cloud the part of $S$ starting at
      $s\cdot\frac{\bC{\interval{i}{j\tm 1}}}{\bC{I_{i}}} $
      and extending for $s\cdot\frac{\bC{j}}{\bC{I_{i}}}$ bits,
      writing $\bC{j}$ bits in every round.}
    \STATE\label{OLD:cw-alg-ack}{node $j\ne i$ sends an acknowledgement to $i$
      when done, and halts}
    \ENDFOR    
    \STATE\label{OLD:cw-alg-end} node $i$ halts when all acknowledgements are received.
  \end{algorithmic}
\end{algorithm}

% While the naive algorithm, in which node $i$ uses the full capacity of
% its links (the cloud link and the link to ${i+1}$) to send
% information, and so does every other node, until all $s$ bits are
% uploaded to the cloud, is trivially optimal, its complexity analysis
% may be tricky.\\ 
%\theoremref{theorem:one_sided_UB} is proved using \algref{alg:cw-hi}.
\Proof
Clearly, the algorithm writes $S$ to the cloud, i.e., it solves
$\CW_i$. 
For the time analysis, note that Step \ref{cw-alg-send-local} requires
$O\left(|\IR{i}| + {{s}\over{\bLminR{i}}} \right)$ rounds: there are
$s$ bits to send over $|I_i|-1$ hops with bottleneck bandwidth $\phi(I_i)$.
In Step \ref{cw-alg-node-write}, each node $j$ writes
% $s\cdot{\bC{j}\over\bC{I{i}}} $ 
% bits to the cloud while writing
$\bC{j}$ bits in each round (except perhaps the last round), and since
it needs to write 
$s\cdot{\bC{j}\over\bC{I{i}}} $ bits  overall, this step requires
$O\left({s}/{\bC{\IR{i}}} \right)$ rounds for all $j\in\IR{i}$.
Step \ref{cw-alg-ack} requires $|\IR{i}|$ rounds.
Thus, the algorithm terminates in
$O \left({|\IR{i}| + \dfrac{s}{\bLminR{i}} +
\dfrac{s}{\bC{\IR{i}}}}\right)
= O(\ZR{i})$ rounds. \QED

We have the following immediate consequence.
\begin{theorem}\label{OLD:theorem:two_sided_UB}
 Let $Z_i^\ell$ and $Z_i^r$ denote the timespans of the counterclockwise and the clockwise cloud intervals of $i$, respectively. Then $\CW_i$ can be solved in $O(\min(Z_i^\ell,Z_i^r))$ rounds.
%	There is an algorithm that writes an $s$-bits message originating
%	from node $i$ to the cloud, that requires at most $O(\ZR{i})$
%	rounds.
\end{theorem}


\begin{corollary}\label{OLD:cor-ub}
  In the uniform wheel topology with cloud bandwidth $\bc$ and local
  link bandwidth $\bl\ge\bc$, \CW terminates in
  $O\left({s\over\bl}+\min(\sqrt{s\over\bc},{\bl\over\bc})\right)$
  rounds. If $\bl<\bc$, the running time is $O(s/\bc)$ rounds.
\end{corollary}
\Proof
If $\bl<\bc$, $\kLR{i}=0$, $\phi(I_i)=\infty$ and the result follows.
Otherwise, by definition we have $\kCR{i}=\sqrt{s/\bc}-1$ and
$\kLR{i}=\bl/\bc-1$, hence $|\IR{i}|=O(\min(\sqrt{s/\bc},\bl/\bc))$. It
follows that $\bc(\IR{i})=O(\min(\sqrt{s/\bc},\bl))$. The result follows by
noting that
$\bLminR{i}=\bl$.
\QED
% \noindent
% For example, for $\bc=\sqrt{s}$ and $\bl\ge s^{3/4}$, the
% running time is $O(s^{1/4})$.

% \boaz{explain here how to extend the algorithm to 2 directions, maybe
%   to \CR}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\CW: Lower Bound}
\label{OLD:single-lb}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To prove a lower bound on the running time of an algorithm solving
$\CW_i$ in the wheel topology, we assume that
the $s$-bits string $S$ that node $i$ needs to write is incompressible.
Such a string
exists for any size $s\in\mathbb{N}$ (see, e.g., \cite{LiV:Kolmogorov}).
As a consequence,
\emph{in any execution of a correct algorithm, $s$ bits must cross any cut that
separates $i$ and the cloud}.
We use this observation in our lower bound arguments.

Similarly to our upper bound strategy, we first prove the lower bound
for ``one-sided'' intervals, and then extend it to the general case.
% Therefore, in the remainder of this section we focus on
% an upload protocol which does not use link $(i\tm 1,i)$.

% We now turn to show that $\Omega(\ZR{i}) = 
% O \left({|\IR{i}| + \dfrac{s}{\bLminR{i}} +
% 	\dfrac{s}{\bC{\IR{i}}}}\right)$ is a lower bound for the
% \CW problem.
% The idea is that the cloud interval
% $\IR{i}$ is an interval that optimizes, up to a constant
% factor, the tradeoff between the time
% required to send $s$ bits through the local network, and the time
% required to write such a message to the cloud.
% Here and in \figref{fig-Z-explanation},
% we give some intuition as for the significance of each term in
% the lower bound:
% \textit{
% \begin{compactitem}
% \item $|\IR{i}|$ is the length of the interval, and at least
%   $|\IR{i}|$ rounds are required to reach all nodes of the interval
%   from $i$.
% \item ${1}\over{\blmin(\IR{i})}$ is the rate of the bottleneck of the
%   interval.  If we were to send only $o(s)$ bits through that
%   bottleneck, then the interval could have been shortened not to
%   include that edge, and we could have still sent $s$ bits using the
%   shortened interval, in the same time up to a constant factor. Thus at
%   least $\Omega(s)$ bits should pass through there, thus requiring
%   $\Omega({{s}\over{\blmin(\IR{i})}})$ rounds.
% %In order to use nodes that are after this bottleneck, at least
% %$\Omega(s)$ bits should pass through there, thus requiring
% %$\Omega({{s}\over{\blmin(\IR{i})}})$ rounds. 
% %Otherwise, these nodes are not necessary and that edge should not be
% %in the interval. 
% \item $\bc(\IR{i})$ is the number of bits that can be sent to the
%   cloud in a single round by the nodes of $\IR{i}$. Thus, at least
%   ${s}\over{\bc(\IR{i})}$ rounds are required to upload an $s$-bits
%   message.
% \end{compactitem}
% }

\begin{theorem}
  \label{OLD:theorem:one_sided_LB}
  Any algorithm for $\CW_i$
  which does not use link $({i\tm 1}, i)$ requires $\Omega(\ZR{i})$ rounds.
\end{theorem}
\Proof
We show that each term
of $\ZR{i}$ is a lower bound on the running time of any algorithm
solving $\CW_i$. The theorem follows from \lemmaref{lemma:interval_length}, \lemmaref{lemma:interval_BN} and \lemmaref{lemma-phi}.
\QED
  
Similarly to \corollaryref{cor-ub}, we have the following corollary
for the uniform wheel.
\begin{corollary}\label{OLD:cor-lb}
  In the uniform wheel topology with cloud bandwidth $\bc$ and local
  link bandwidth $\bl$, any algorithm for \CW requires at least
  $\Omega\left({s\over\bl}+\min(\sqrt{s\over\bc},{\bl\over\bc})\right)$
  rounds if $\bl\ge\bc$, and $\Omega({s\over\bc})$ otherwise.
\end{corollary}
%
%
\ignore{
\begin{figure}[t]
  \centering
  \scalebox{.7}{
    \begin{tikzpicture}
      \node[draw, circle, fill=yellow!90!black, minimum size=1cm] at (0,0) (mid) {$i$};
      \node[draw, circle, inner color=white, minimum size=1cm] at (-2,0) (l) {$i-1$};
      \node[draw, circle, inner color=white, minimum size=1cm] at (2,0) (r) {$i+1$};
      \node [cloud, draw,cloud puffs=17,cloud puff arc=120, aspect=4.5, inner ysep=1em]
      at 	(0, 2.5)
      {\emph{$v_c$}};
      \draw [-] (mid) -- (l)
      node [above,text width=3cm,text centered,midway] {$0$};
      \draw [-] (mid) -- (r)
      node [above,text width=3cm,text centered,midway] {$0$};
      \draw [->] (mid) -- (0, 1.5)
      node [right,text width=0cm,text centered,midway] {$\bc(i)$};
      \draw [->] (r) -- (2, 1.5)
      node [right,text width=0cm,text centered,midway] {$0$};
      \draw [->] (l) -- (-2, 1.5)
      node [right,text width=0cm,text centered,midway] {$0$};
    \end{tikzpicture}
\hspace{8mm}
    \begin{tikzpicture}
      \node[draw, circle, fill=yellow!90!black, minimum size=1cm] at (0,0) (mid) {$i$};
      \node[draw, circle, inner color=white, minimum size=1cm] at (-2,0) (l) {$i-1$};
      \node[draw, circle, inner color=white, minimum size=1cm] at (2,0) (r) {$i+1$};
      \node [cloud, draw,cloud puffs=17,cloud puff arc=120, aspect=4.5, inner ysep=1em]
      at 	(0, 2.5)
      {\emph{$v_c$}};
      \draw [-] (mid) -- (l)
      node [above,text width=3cm,text centered,midway] {$0$};
      \draw [-] (mid) -- (r)
      node [above,text width=3cm,text centered,midway] {$w$};
      \draw [->] (mid) -- (0, 1.5)
      node [right,text width=0cm,text centered,midway] {$0$};
      \draw [->] (r) -- (2, 1.5)
      node [right,text width=0cm,text centered,midway] {$\infty$};
      \draw [->] (l) -- (-2, 1.5)
      node [right,text width=0cm,text centered,midway] {$0$};
    \end{tikzpicture}
\hspace{8mm}
    \begin{tikzpicture}
      \node[draw, circle, fill=yellow!90!black, minimum size=1cm] at (0,0) (mid) {$i$};
      \node[draw, circle, inner color=white, minimum size=1cm] at (-2,0) (l) {$i-1$};
      \node[draw, circle, inner color=white, minimum size=1cm] at (3,0) (r) {};
      \node[draw, circle, inner color=white, minimum size=1cm] at (5,0) (rfar) {$i+k$};
      \node at ($(mid)!.5!(r)$) (dots) {\ldots};
      
      \node [cloud, draw,cloud puffs=23,cloud puff arc=120, aspect=7, inner ysep=1em]
      at 	(1.6, 2.5)
      {\emph{$v_c$}};
      
      \draw [-] (mid) -- (l)
      node [above,text width=3cm,text centered,midway] {$0$};
      \draw [-] (mid) -- (dots)
      node [above,text width=3cm,text centered,midway] {$\infty$};
      \draw [-] (r) -- (dots)
      node [above,text width=3cm,text centered,midway] {$\infty$};
      \draw [-] (r) -- (rfar)
      node [above,text width=3cm,text centered,midway] {$\infty$};
      \draw [->] (mid) -- (0, 1.45)
      node [right,text width=0cm,text centered,midway] {$0$};
      \draw [->] (r) -- (3, 1.45)
      node [right,text width=0cm,text centered,midway] {$0$};
      \draw [->] (l) -- (-2, 1.45)
      node [right,text width=0cm,text centered,midway] {$0$};
      \draw [->] (rfar) -- (5, 1.45)
      node [right,text width=0cm,text centered,midway] {$\infty$};
    \end{tikzpicture}
  }
  \caption{ \em
    The lower bound at a glance. Labels near edges indicate
    their bandwidth.
    Left: $\IR{i}=\Set{i}$, and $Z_i\ge s/\bc(i)$.
    Middle: $\IR{i}=\Set{i,i\tp1}$, $\phi(\IR{i})=w$, so $Z_i\ge s/w$.
    Right: $\IR{i}=\Set{i,\ldots,i+k}$, so $Z_i\ge k$.
  }
  \label{OLD:fig-Z-explanation}
\end{figure}
}

\begin{lemma}
  \label{OLD:lemma:interval_length}
  Any algorithm for $\CW_i$
  that does not use edge $({i\tm 1}, i)$ requires 
  $\Omega \left( |\IR{i}|\right) = \Omega \left( \kR{i}\right)$
  rounds.
\end{lemma}
\Proof Let $A$ be an algorithm for $\CW_i$
  that does not use link $({i\tm 1}, i)$ and runs in $t_A$ rounds.
If $t_A \ge n$ then $t_A \ge \kR{i}$ and we are done. Otherwise,
we count the number of bits of $S$ that can get to the cloud in $t_A$
rounds. %\yehuda{by when?}.
% Once a bit
% gets to the cloud, we do not count it again if some other node reads
% it and writes it again. 
% We also assume that all bits of the message
% are written to the cloud as they are, without any manipulation. This
% assumption is justified, as we can assume that the input can't be
% compressed as there are $2^s$ inputs that are distributed uniformly.
%
Since $S$ is initially stored in $i$, and since link $({i\tm 1},
i)$ is not used, 
in round $t$  only the nodes in
$\interval{i}{i\tp t\tm1}$ can write to the cloud
 parts of $S$.
It follows that in a given round $t$,
at most $\bc([i,i\tp t\tm1])$ bits of
information are sent to the cloud and therefore, overall $A$
writes to the cloud at most
$\sum_{t=1}^{t_A}\bc([i,i\tp t\tm1]) \le t_A\cdot\bc([i,i\tp t_A\tm1])$
bits. Hence, by assumption that  $A$ solves $\CW_i$,
we must have $t_A\cdot\bc([i,i\tp t_A\tm1]) \ge s$. Since by definition,
$\kCR{i}$ is the minimal 
integer%
\footnote{
  $\kCR{i}$ may be $n$ if no such integer exists, but $t_A$ is an integer
  that satisfies the $\kCR{i}$ formula so this is not the case.
}
$\ell$ such that
$(\ell \tp 1)\sum_{j=i}^{i+\ell} \bC{j} \ge s$, we get that
$t_A \tm 1 \ge \kCR{i} \ge \kR{i}$ and the lemma follows. \QED


\begin{lemma}
  \label{OLD:lemma:interval_BN}
  Any algorithm for $\CW_i$
  which does not use edge $({i\tm 1}, i)$ requires 
  $\Omega({s}/{\blmin(\IR{i})})$ rounds.
\end{lemma}
\Proof
If $\kR{i}=0$, $\blmin(\IR{i})=\infty$ and the claim is trivial.
Otherwise, let $(j,j\tp 1)\in E$ be any link in
$\IR{i}$ with $\bL{j}{j\tp 1} = \bLminR{i}$.
Note that $j-i<\kR{i}$ because $j+1\in I_i$.
% $r = \argmin\Set{\bL{i\tp j}{i\tp j\tp 1}
%   \mid 0 \le j \le \kR{i}\!\! - \!\!1}$ (ties broken arbitrarily),
% % $r = \argmin\Set{\bL{i\!\!+\!\!j}{i\!\!+\!\!j\!\!+\!\!1}
% %   \mid 0 \le j \le \kR{i}\!\! - \!\!1}$.
% % the link $(i\tp r, i\tp r\tp 1)$ has the least bandwidth in $\IR{i}$,
% % meaning
% which implies that $\bL{i\tp r}{i\tp r\tp 1} = \bLminR{i}$.
%
Consider the total bandwidth of links emanating from the interval
$I' \DEF \interval{i}{j} $. Since we assume that
the link $(i\tm1,i)$ is not used, the number of bits that can leave
$I'$  in $t$ rounds is at most
$t\cdot\left(\bc(I')+ \bL{j}{j\tp 1}\right)$. 
Notice that % $s$ bits of the file originate at node $i$ and are written
% to the cloud, and thus
at least $s$ bits have to leave $I'$.

Observe that $\bc(I') \le \bL{j}{j\tp 1}$, because otherwise we would have
$\kLR{i}=j-i$, contradicting the fact that $k(i)>j-i$.
Therefore, any
algorithm $A$ that solves $\CW_i$ in $t_A$ rounds satisfies
$$
s~\le~t_A\cdot\left(\bc(I') + \bL{j}{j\tp 1} \right)
~\le~ 2t_A\cdot \bL{j}{j\tp 1}
~=~ 2t_A\cdot \bLminR{i} ~,
$$
and the lemma follows. \QED

\begin{lemma}\label{OLD:lemma-phi}
  Any algorithm for $\CW_i$
  which does not use edge $({i\tm 1}, i)$ requires 
    $\Omega \left({s}/{\bC{\IR{i}}} \right)$ rounds.
\end{lemma}

\Proof Let $A$ be any algorithm that solves $\CW_i$ in $t_A$ rounds.
Recall that $\kR{i} = \min(\kCR{i}, \kLR{i})$.  If $\kR{i}=n$ then
$\IR{i}$ contains all processor nodes $V_p$, and the claim is obvious, as no more
than $\bC{V_p}$ bits can be written to the cloud in a single round.
Otherwise, we consider the two cases: If $\kR{i} = \kCR{i}$, then
$\kR{i} \ge {s}/{\bC{\IR{i}}} - 1$ by definition, and we are done
since $t_A = \Omega(\kR{i})$ by \lemmaref{lemma:interval_length}.
Otherwise, $\kR{i} = \kLR{i}$. Let us denote $w_R=\bL{i\tp
  \kR{i}}{i\tp \kR{i}\tp1}$. In this case we have
$w_R < \bc(\IR{i})$.  We count how many
bits can leave $\IR{i}$.  Similarly to \lemmaref{lemma:interval_BN},
in a single round, at most $\bC{\IR{i}}$ bits can leave through the
cloud links, and at most $w_R$ bits can leave through
the local links. Since $A$ solves $\CW_i$, we must have
$
s
~\le~t_A\cdot\left(\bC{\IR{i}} +w_R\right)
~\le~ 2t_A \cdot \bC{\IR{i}} ~,$
and hence $t_A = \Omega\left({s}/{\bC{\IR{i}}} \right)$.
\QED




% \subsection{Using Links From Both Directions}
% \label{OLD:ssec:write_two_sided}
Given \theoremref{theorem:one_sided_LB} and its corresponding lower
bound for counterclockwise intervals, we can prove the lower bound for
two-sided intervals, under some reasonable assumptions.
%
%Recall that 
%Without loss of generality,
We consider algorithms that
do not manipulate bits, i.e., the only representation of a bit string
(and substrings) is by explicit listing of its content, where the
length is proportional to the number of bits.
We also assume that the algorithms are oblivious to contents: the algorithm execution is independent of the actual bit values in the file, its operation depends only on the network parameters and $s$, the number of bits to be transferred. 
% we only consider algorithms that operate in the same manner for every
% input size $s$, i.e., each node sends and receives the same amount
% of bits through its incident links in every round,
% regardless of the actual content of the input message.

\begin{lemma}\label{OLD:lem-oneway-lb}
  Let $Z_\ell$ denote the minimal number of rounds required by an
  algorithm for $\CW_i$ which does not use link
  $({i},{i\tp 1})$, and similarly let $Z_r$ the minimal number of
  rounds for an algorithm which does not use $({i\tm 1},{i})$.  Then
  any oblivious algorithm for $\CW_i$ (which uses all links) requires
  $\Omega(\min(Z_\ell,Z_r))$ rounds.
\end{lemma}

\Sketch Let $A$ be an algorithm by which node $i$ writes an $s$-bits file to the cloud 
in $t_A$ rounds. % $A$ may use nodes on both sides of $i$ to
% write its file.
We make a few assumptions on $A$ and show how to relax them without
affecting $A$'s running time.
%We start with a few simplifying assumptions on $A$,
%and prove that $A$ can be adjusted to allow these assumptions,
%while only improving on the its runtime.

%	\emph{$A$ is oblivious to the content of the message
%		(i.e the value of the bits).}
%	This assumption is legitimized by the aforementioned assumption that the algorithm
%	does not manipulate the message, and the existence of an incompressible input string.
%	
First, we assume that no message is sent from either node $i \tp 1$ or
	$i \tm 1$ to node $i$.
We assume that node $i$ is the only node that has information (the $s$-bits file)
prior to the execution of $A$,
and also that $A$ and all bandwidths in $G$ are known to all nodes.
Hence, node $i$ can locally simulate the execution of $A$,
and calculate in advance all messages that it receives through links
$(i, i\tm 1)$ and $(i \tp 1, i)$. Therefore $A$ can operate in the exact same manner,
without sending information through these links to node $i$.

Next, we assume that during the run of $A$, no node reads from $v_c$.
Since we assume that message contents is not manipulated, and that $A$
is oblivious to the content of the file, for any node $j$ that reads a bit string
from the cloud there are two options for the content it reads:
\begin{compactitem}
	\item Part of the file of node $i$. In this case, the destination of these bits
	is eventually the cloud, and thus the node(s) that wrote these bits to the cloud
	could have written them directly to their destination, and the read operation
	is redundant.
	\item Information that was sent from other node(s),
	which is not part of the file of node $i$.
	In that case, since $A$ is oblivious to the content of
	the file, node $j$ could have simulated locally the run of $A$ on some
	arbitrary input, and discover this message by itself without reading it
	from the cloud.
\end{compactitem}
	
In light of these simplifying assumptions on $A$,
let $s_r$ be the number of bits that were sent to
$v_c$ from nodes $\interval{i\tp 1}{i\tp t_A}$,
let $s_\ell$ be the number of bits that were sent to
$v_c$ from nodes $\interval{i\tm t_A}{i\tm 1}$,
and let $s'$ be the number of bits that were sent to
$v_c$ from node $i$.
Let $s'_r=s_r + s'$, $s'_\ell=s_\ell + s'$.

$A$ sends $s$ bits to the cloud, and thus we get that
$s \le s'+s_r+s_\ell \le s'_r + s'_\ell$,
from which we get that either $s'_r \ge s/2$ or $s'_\ell \ge s/2$.
Assume \WLOG the former.
By the assumptions on $A$, %one can see that 
the $s'_r$
bits sent by $\interval{i}{i+t_A}$ are independent of the operations
performed by nodes $\interval{i\tm t_A}{i\tm 1}$.

We can now construct an algorithm $A'$ that sends $s$ bits of
information originating in node $i$ to the cloud, without using the
link $(i\tm 1, i)$:
We run $A$, without sending any information through edge $({i\tm 1}, i)$,
and by that send $s'_r$ bits of the file to the cloud.
Once $A$ finishes, we run $A$ again in the same manner, now sending
the remaining $s-s'_r$ bits.
$A'$ requires $2t_A$ rounds, and by the definition of $Z_r$ we get
that $2t \in \Omega(Z_r)$. \QED



\ignore{
\begin{definition}\label{OLD:def-Ii-2-sided}
Let $\IR{i}^r$ and $\IR{i}^\ell$ be the intervals received in \defref{def-Ii}
for the cases that do not use
edge $(i \tm 1, i)$, and do not use edge $(i, i\tp 1)$, respectively. Let
$\ZR{i}^r$ and $\ZR{i}^\ell$ be the lower bounds that were
defined in \defref{def-Ii}
%received from \theoremref{theorem:one_sided_LB}
for these intervals, respectively.

We define the (\emph{not one-sided}) cloud interval $\IR{i}$ and timespan $\ZR{i}$
of node $i$
to be $\IR{i}^r$ and $\ZR{i}^r$
respectively, if $\ZR{i}^r < \ZR{i}^\ell$. Otherwise, we define
$\IR{i}$ and $\ZR{i}$ to be $\IR{i}^\ell$ and $\ZR{i}^\ell$
respectively.
\end{definition}
}

Combining %\lemmaref{lem-oneway-ub} with \theoremref{theorem:one_sided_UB}
%and 
\lemmaref{lem-oneway-lb} with \theoremref{theorem:one_sided_LB},
we obtain the following results.


\begin{theorem} \label{OLD:theorem:two_sided_LB} 
 Let $Z_i^\ell$ and $Z_i^r$ denote the timespans of the counterclockwise and the clockwise cloud intervals of $i$, respectively. Then any oblivious algorithm
 for $\CW_i$ requires $\Omega(\min(Z_i^\ell,Z_i^r))$ rounds.
% Any algorithm that
%  writes an $s$-bits message originating from node $i$ to the cloud,
%  requires at least $\Omega(\ZR{i})$ rounds.
\end{theorem}


\subsection{\CR:  Upper and Lower Bounds}
\label{OLD:ssec:CR}
%%%%%%%%%%%%%%%%%%%%%
We now consider $\CR_i$% , under the assumption that link bandwidth is symmetric, the same in both directions
. 
We claim that it is essentially the same as
$\CW_i$---reversed:
% Note that since we require that an invocation of $\CW_i$
% requires a ``done'' response at $i$, read and
% write are essentially the same task, reversed: 
 Given an
execution of $\CW_i$, consider running it  backwards. The
acknowledgements sent in $\CW_i$, run backwards, turn into ``start''
message sent by $i$,
and writes to the cloud by nodes of $\IR{i}$ in $\CW_i$ turn into reads from
the cloud in $\CR_i$. Finally, instead for $i$ sending $S$ to $\IR{i}$, in
$\CW_i$, in $\CR_i$ we have that the nodes of $\IR{i}$ send pieces of
$S$ to $i$, which assembles them to the complete $S$ and
halts. Pseudocode is presented in
\algref{alg:cr-hi}. We summarize as follows.


\begin{algorithm}[t]%[H]\small
  \caption{$\CR_i$}
  \label{OLD:alg:cr-hi}
  \begin{algorithmic}[1]
    \STATE{
      Node $i$ sends a ``start'' message to all nodes in $\IR{i}$,
      telling them when to start reading from the cloud.}
    \label{OLD:cr-alg-start}
    \FOR{ all $j\in\IR{i}$  in parallel}
    \STATE{
      Node $j$ reads from the cloud
      the part of the message starting at
      $s\cdot{\bc([i,j])\over\bC{I{i}}}$ and extending for
      $s\cdot{\bc(j)\over\bC{I{i}}}$ bits,
      by reading $\bC{j}$ bits in every round.
    }
    \label{OLD:cr-alg-node-read}
    \STATE {
      Node $j$ sends the part of $S$ it read through the local
      links to $i$.
    }
    \label{OLD:cr-alg-send-local}
    \ENDFOR    
    \STATE{ When all $s$ bits of the message are
      received at node $i$, \CR is done.
    }
    \label{OLD:cr-alg-end}
  \end{algorithmic}
\end{algorithm}

\begin{theorem}\label{OLD:theorem:CR_UB}
 Let $Z_i^\ell$ and $Z_i^r$ denote the timespans of the counterclockwise and the clockwise cloud intervals of $i$, respectively. Then 
 $\CR_i$ can be executed in  $O(\min(Z_i^\ell,Z_i^r))$ rounds.
\end{theorem}

% \Proof Taking the algorithm received in \theoremref{theorem:two_sided_UB},
% and reversing it as mentioned will result with an algorithm that reads $s$ bits from the cloud and sends them to node $i$, as required.

% To be more explicit, the reversed algorithm for \algref{alg:cw-hi}
% is described in high level in \algref{alg:cr-hi}.
% Note that this algorithm is described for the \emph{right} cloud interval of $i$,
% but the claim can be extended to both directions using a
% similar lemma to \lemmaref{lem-oneway-ub}.

% Similarly to the upper bound of \CW, one can see that
% step \ref{cr-alg-start} requires $O(|\IR{i}|)$ rounds,
% step \ref{cr-alg-node-read} requires $O\left({s}/{\bC{\IR{i}}} \right)$ rounds,
% and step \ref{cr-alg-send-local} requires
% $O\left(|\IR{i}| + {{s}\over{\bLminR{i}}} \right)$ rounds,
% which sums up to $O(\ZR{i})$ rounds in total.

Using arguments as for $\CW_i$, we also have the following lower bound.

\begin{theorem} \label{OLD:theorem:CR_LB}
 Let $Z_i^\ell$ and $Z_i^r$ denote the timespans of the counterclockwise and the clockwise cloud intervals of $i$, respectively. Then any oblivious algorithm
 for $\CR_i$ requires $\Omega(\min(Z_i^\ell,Z_i^r))$ rounds.
\end{theorem}

% \Proof Any such algorithm, can be ``reversed'' as described above,
% to get an algorithm that contradicts \theoremref{theorem:two_sided_LB}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cwc"
%%% End:




==> old/wheel.tex <==

\section{Non-Commutative Operators and the Wheel Settings}
\label{sec:wheel}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section we briefly consider \CCW for
non-commutative operators such as Matrix Multiplication.
Most details are given in \appendixref{sec:wheel-appendix}.

First note that \algref{alg:ccw-hi} and \theoremref{thm-ccw-covers-ub} %from \sectionref{ssec:combining}
still apply, as long as the ordering of the nodes matches
one of the possible ordering that is achieved by the algorithm.
% For example, if there is a cover $\cC$ of the system
% such that in each cluster all nodes are consecutive,
% and such that the combination of all nodes in the cluster is achievable
% in $O(\Zmax(C))$ rounds without using cloud links,
% the upper bound of \theoremref{thm-ccw-covers-ub}
% would still apply, as long as the order
% between the clusters is one that can be preserved by \algref{alg:ccw-high:overlap}
% (i.e., all clusters of a single color class are consecutive).
% Otherwise, an upper bound of $O(\Zmax(C) \cdot \load(C) \cdot \log |C|)$
% can be achieved by \algref{alg:ccw-hi} by discarding
% the use of \algref{alg:ccw-high:overlap}, and instead using \algref{alg:ccw-high:node}
% on all subsets $C_l$ in parallel, using multiplexing.
However, it is not always likely that the inputs are located according
to the ordering of some (unspecified) cover. Instead, we believe that
in the case of a non-commutative combining operator, it is reasonable
to assume that processing nodes are physically connected 
according to their combining order, i.e., in a line. Closing the cycle for symmetry and
adding a cloud link from each processor, we arrive at the wheel
topology, which we study in this section.
We assume that all links are bidirectional and bandwidth-symmetric.


We start with the concept of intervals that refines the concept of
clusters (\defref{def-clusters}) to the case of the wheel topology.

\begin{definition}\label{def-intervals}
	% Let $G=(V,E,w)$ be an $n$-node wheel graph.
	The \textbf{cloud bandwidth} of a processing node $i \in V_p$ in a
	given wheel graph is
    $\bc(i)\DEF w(i,v_c)$.
	An \textbf{interval}
	$\interval{i}{i\tp k}\DEF\Set{i,i\tp 1,\ldots,i\tp k}\subseteq V$ is a path
	of processing nodes in the ring. Given an interval $I=[i,i+k]$,  $|I|=k+1$ is its \textbf{size}, and $k$ is its
	\textbf{length}.  The \textbf{cloud bandwidth} of $I$,
	denoted $\bc(I)$, is the sum of the cloud bandwidth of all nodes in
	$I$: $\bc(I)=\sum_{i\in I}\bc(i)$.  The \textbf{bottleneck
		bandwidth} of $I$, denoted $\blmin(I)$, is the smallest bandwidth
	of a link in the interval:
	$\blmin(I)=\min\Set{w(i,i\tp1)\mid i,i\tp1\in I}$.  If  $|I|=1$, define $\blmin(I) = \infty$.
\end{definition}
(Note that bottleneck bandwidth was not defined for general clusters.)


Given these interval-related definitions, we adapt
the notion of ``cloud cluster'' (\defref{def-Bi}),
for problems with inputs $s$,
this time also accounting for the bottleneck of the interval.
We define $\IR{i}$ to be the \textbf{cloud interval} of node $i$,
and $\ZR{i} = |\IR{i}| + \dfrac{s}{\blmin(\IR{i})} +
\dfrac{s}{\bc(\IR{i})}$ to be the \textbf{timespan} of $\IR{i}$.
See \defref{def-Ii} for a more detailed explanation.

Similarly to the fat-links case, we get the following theorems
for the $\CW_i$ problem (and for $\CR_i$).

\begin{theorem}[See \theoremref{theorem:CW_UB_interval} and \theoremref{theorem:two_sided_UB}]
	In the wheel settings, $\CW_i$ can be solved in $O(\ZR{i})$ rounds for every node $i$.
\end{theorem}

\begin{theorem}[See \theoremref{theorem:one_sided_LB} and \theoremref{theorem:two_sided_LB}]
	In the wheel settings, Any algorithm for $\CW_i$
	requires at least $\Omega(\ZR{i})$ rounds for every node $i$.
\end{theorem}


Our main result in this section is an algorithm for \CCW for arbitrary
wheel topology that works in time which is a logarithmic factor larger
than optimal. In contrast to the result of \theoremref{thm-ccw-ub} that
applied only to graphs with fat links, here we analyze the wheel
topology with arbitrary bandwidths.
% $O(Z_{\max}\log n)$ rounds in the wheel settings, where $Z_{\max}$ is the maximal timespan
% of cloud intervals (cf.\ \defref{def:intervals2} and \theoremref{thm-aw-ub}).
We note that by using
standard methods \cite{LadnerF-80}, the presented algorithm can be extended to
compute, with the same asymptotic time complexity, all prefix sums,
i.e., compute  $\bigotimes_{i=0}^jS_i$ for each $0\le j<n$.

First, we refine the notion of $\Zmax$ (see \defref{def:intervals2}) for the wheel case.
Then, we adapt \algref{alg:ccw-hi} with the following theorem:

\begin{theorem}\label{thm-ccw-intervals-ub}
	In the wheel settings,
	\CCW can be solved in
	$O(\Zmax \log n)$ rounds
	by \algref{alg:ccw-hi}
\end{theorem}

This is a log factor improvement  over the fat-links case.
A complete proof is presented in the appendix in \theoremref{thm-ccw-intervals-ub:appendix}.
The main ideas that we use in the proof are as follows:
\begin{compactitem}
	\item In the wheel case, for any minimal cover $C'$ of the graph,
	$\load_{C'}(i) \le 2$ for every node $i$ (\lemmaref{lem-coverload}).
	This observation allows to operate on intervals ``simultaneously'',
	while paying only a constant factor to the runtime by multiplexing.
	
	\item Due to the limited local bandwidth, \algref{alg:ccw-low}
	can't be used with the same time analysis as in the fat-links case
	in Steps \ref{ccw-startloop}--\ref{ccw-endloop} of \algref{alg:ccw-hi}.
	Instead, we use pipelining to compute the inner product of every interval
	in the cover, as described in \lemmaref{lem-lo}.

	\item Since a minimal cover $C'$ is easily computed and has a constant 
	$\load(C')$, There is no need to use the result of Awerbuch
	and Peleg (\theoremref{thm-AP}) in the cycle case.
\end{compactitem}

\smallskip\noindent
Finally, we distinguish between \emph{holistic} and
\emph{modular} combining operators, defined as follows.
In modular combining, one can apply the combining
operator to aligned, equal-length parts of operands to get the output
corresponding to that part. For example, this is the case with vector
(or matrix) addition: to compute any entry in the sum, all that is
needed is the corresponding entries in the summands.
If the operand is not modular, it is called holistic
(e.g., matrix multiplication).
% no part of the product can be computed without both operands being
% % the product can be computed only when both operands are
% known in the entirety.
% This is the case, for example, with matrix
% multiplication.  
We call the aligned parts of the operands \emph{grains}, and their maximal size
$g$ is the \emph{grain size}.
See \defref{def:modular-op} for the full definition.
We show that in the modular case, %\gal{should we state here that it works only if all links have bandwidth that is at least the grain size?}
using pipelining, a logarithmic
factor can be shaved off the running time (more precisely, converted
into an additive term), as can be seen in the following theorem:


\begin{theorem}[See \theoremref{thm-aw-modular:appendix}]\label{thm-aw-modular}
  Let
  \begin{compactitem}
  \item $j_{\max} = \argmax_i\Set{|\IR{i}|}$
  \item $j_c = \argmin_i \Set{\bC{\IR{i}}}$
  \item $j_\ell = \argmin_i \Set{\bLminR{i}}$
  \item $Z_{\max} = {|\IR{j_{\max}}| + {s}/{\bLminR{j_\ell}} + s/{\bC{\IR{j_c}}} }$.
  \end{compactitem}
      Suppose  $\otimes$ is modular with
	grain size $g$,
	and that $w(e) \ge g$ for every link $e\in E$.
	Then \CCW can be solved in
	$O\left(Z_{\max}+\log n\right)$ rounds.
%	$O\left(Z_{\max}
%	+|I_{j_{\max}}|\ceil{\frac{g}{\phi(I_{j_{\ell}})}}
%	+\ceil{\frac{g}{\bC{\IR{j_c}}}}\log n\right)$.
\end{theorem}




%\gal{I didn't add the extension of asymmetric cloud links.}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cwc"
%%% End:


==> oldIntro.tex <==
\section{Introduction}
\label{sec:intro}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
While being very critical for the Internet operation, the DNS system is unforgiving, it has no \ariel{CTRL-Z}, i.e., no undo command.
For example, several Microsoft services like Azure and others were not available for a few hours in 2019 due to an erroneous DNS update which could not be easily corrected, undone \cite{azure}. 
Furthermore, the system is very sensitive to authoritative server failures or crashes due to DDoS or other attacks.
In this paper we examine \DNSUD{}, a method to add an undo command to the DNS system for a reasonable price in resources.
\DNSUD{} also increases the fault tolerant of the DNS system to name servers crashes.


Internet domain name owners and managers have to set the TTL value associated with their domain records in the DNS system \cite{rfc1034} to dictate the maximum time a record may be stored in resolvers, stub resolvers, and client caches before they should obtain a fresh copy from the authoritative server \cite{rfc1035}.
Associating short TTL values with domain names is the current remediation for the DNS unforgiveness however it comes with a high price tag in excess DNS traffic (refreshing a popular domain record in different resolvers every TTL time).
On the other hand, two major risks are associated with high TTL values for domain names \cite{choose-ttl-values}; first, if inadvertently a domain name is announced with the wrong IP, then the corresponding service is inaccessible for the duration of this high TTL time; secondly, if a service has to change its IP address (e.g., for maintenance, load balancing or any other reason) then again the clients have to wait for the expiration of the TTL before the change takes effect. 
\DNSUD{} suggested here provides the benefits of both: an undo command for quick recovery from erroneous updates and robustness against crashes, and at the same time, 
large TTL values to reduce the load on DNS authoritative servers.

\ignore{%%%%%%%%%%%%%%%%%
As a result, the TTL value of many domains is very short ($1-5$ minutes), even though most domains change their IP address infrequently (less than once a month). Content distribution networks (CDNs) \cite{kazunori2012cdn, centralized-dns} use even shorter TTLs ($\sim$ tens of seconds) to achieve high availability, load balancing, and frequent updates but only some of them indeed change their IP quite often.

The main consequence of choosing short TTL values is that most DNS requests receive the same response over and over, resulting in extra traffic to learn that there is nothing new.
}%%%%%%%%%%%%%%%%%%

There are two major observations on which \DNSUD{} is based; First, the method is backward compatible and adaptive.  That is, any portion of the system may use \DNSUD{} while other parts continue operating in the traditional DNS method. 
Secondly, about $80\%$ of the domains in the Internet have a very high ratio of inter IP address update time and TTL length.
These $80\%$ of domains would greatly benefit from using \DNSUD{}, while the others may keep using the traditional DNS mechanisms with low TTL values.
As a typical example, consider the popular Microsoft domain office.com whose TTL is $5$ minutes but its IP address has not been updated for $3$ years.
Thus, at least every $5$ minutes, office.com is evicted from the resolvers' cache, and upon receiving a DNS request, the resolvers issue a new query to the authoritative server holding office.com.  That is, short TTL values are a significant cause of excess traffic between clients and resolvers as well as between resolvers and authoritative servers.

As stated above, our motivation came from incidents in which the wrong IP address was inadvertently associated with a domain, resulting in service disruption for the duration of the corresponding TTL value, which sometimes was several hours, as in the Microsoft incident from 2019 \cite{azure}. Where 
    Microsoft services like Azure, Microsoft 365 umbrella, Dynamics, and DevOps were down for more than 2 hours due to an incorrect DNS update.
    Microsoft published: "During the migration of a legacy DNS system to Azure DNS, some domains for Microsoft services were incorrectly updated." In another incident, in 2021 SiteGround services \cite{siteground} were not accessible to Google crawlers for several hours due to an incorrect DNS update.
    The company explained: "We have implemented a fix for the Google bot crawling issue experienced by some sites... Please allow a few hours for the DNS changes to take effect".
Other similar incidents have occurred, such as Zoho\cite{zoho}, Slack \cite{slack}, Microsoft \cite{win-update}, and Akami \cite{akami}.

\ignore{%%%%%%%%%%%%%%%%%%%%%%%%% 
We estimate this excess traffic by calculating the ratio between the average time between IP address updates for a domain and its corresponding TTL value. In addition, our analysis indicates that more than $80\%$ of the $500,050$ most popular domains change their IP address less than once a month and more than $60\%$ less than once a year. \footnote{We combined an up to date top $500$ domains list of moz.com with the top $500,050$ list of Alexa from $2021$. Due to the constrains of SecurityTrails \cite{securitytrails} we sampled $200$ domains from this list.  See Section \ref{sec:freq-updates}.} For these domains we found that at most $0.2\%$ of DNS responses contain a DNS record that has been changed since the previous response, \ariel{e.g., the IP address of the domain "Office.com" has not changed for more than $3$ years, but its TTL value is $300$ seconds.
Thus, every $300$ seconds at most, the domain is evicted from the resolver's cache, and upon receiving a DNS request, the resolvers issue it to the authoritative server.} As a result, short TTL values are a significant cause of excess traffic between clients and resolvers as well as between resolvers and authoritative servers.
This excessive traffic also causes client latency and server performance impairment \cite{moura2019cache}. In addition, website owners expose themselves to another availability problem - if there is no access to their authoritative servers, when their short TTL expires, the access to their website is disabled \cite{facebook}.

As stated above, our motivation came from incidents in which the wrong IP address was inadvertently associated with a domain, resulting in service disruption for the duration of the corresponding TTL value, which sometimes was several hours, as in the Microsoft incident from 2019:
\begin{itemize}[leftmargin=0.12in]\setlength\itemsep{0em}
    \item Microsoft \cite{azure} - In 2019, Microsoft services like Azure, Microsoft 365 umbrella, Dynamics, and DevOps were down for more than 2 hours due to an incorrect DNS update. Microsoft published: "During the migration of a legacy DNS system to Azure DNS, some domains for Microsoft services were incorrectly updated."
    \item SiteGround \cite{siteground} - In 2021, SiteGround services were not accessible to Google crawlers for several hours due to an incorrect DNS update. The company explained: "We have implemented a fix for the Google bot crawling issue experienced by some sites... Please allow a few hours for the DNS changes to take effect".
\end{itemize}
Similar incidents have occurred, such as Zoho\cite{zoho}, Slack \cite{slack}, Microsoft \cite{win-update}, and Akami \cite{akami}.

}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nsdionly{%%%%%%%%%%%%%%%%%%%%
Many people rightfully describe the DNS as the phone book of the Internet.
In both, when clients need the IP address of a domain or the phone number of another person or business, they query either the DNS system or use a search engine to query for the desired phone number. However, there is a difference; IP addresses sometimes change frequently, while the phone number of people change quit infrequently. Thus using a contact-list (cache) on mobile devices is helpful for phone books but requires much more care and sophistication in the DNS system due to the dynamic nature of IP addresses associated with endpoints. Still, the DNS system relies on caches with a TTL value attached to each record. However, suppose, for some reason, the cache contains the wrong IP address for a domain. In that case, there is no automatic mechanism to query the authoritative server again to get a fresh record. As a result, clients query the DNS system regularly, regardless of whether record updates have occurred, unlike updates of a phone contact list when the mentioned person updates her phone number.

Internet service owners compromise on any choice of TTL: large TTL values cause slow recovery from an IP address change, while short TTLs generate excess traffic and load.
}%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this paper, we propose \DNSUD{}, a mechanism to update a record in resolver caches before the associated TTL has expired.
In a nutshell, \DNSUD{} updates the resolvers about domains whose records were recently updated.
After that, the resolvers remove the corresponding records from their cache.
Upon receiving a subsequent request for a removed domain, the resolver performs a new resolution in the standard DNS system to get a fresh update.
\DNSUD{} is secure, efficient, robust to DDoS attacks, and fully compatible with the current DNS system. 

\ariel{Furthermore, \DNSUD{} enables Internet services to significantly increase the TTL values associated with their domain names in resolvers' cache (client caches are discussed in the sequel). Thus, we add an additional second TTL value, called DNS\em{RU}-TTL while maintaining the traditional TTL that is used to communicate with clients and resolvers that do not use the method. 
To achieve backward compatibility,
DNS\em{RU}-TTL is sent in DNS responses in an optional field (in the ADDITIONAL section) for resolvers that have implemented \DNSUD{}.
\ignore{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Domain names with short TTL values (less than $10$ minutes) benefit from \DNSUD{} since larger TTL values reduce their DNS traffic and the average latencies experienced by clients. Furthermore, for domain names with large TTL values, \DNSUD{} provides quick recovery from IP address changes.
To achieve the backward compatibility of the \DNSUD, we added an additional TTL value, an optional field, used by clients and resolvers that are not yet using the \DNSUD, besides the traditional TTL value (used by the clients).
} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this way, an authoritative server that uses \DNSUD{} can communicate with resolvers that implemented or did not the method, and a resolver that uses \DNSUD{} can communicate with both authoritative servers that implemented or did not the method.
In Section \ref{sec:beyond}, we discuss methods to expand \DNSUD{} to enable clients to use the additional larger TTLs and reduce the excessive DNS traffic also between clients and resolvers.}
\ignore{While the method could be applicable also for clients and stub resolvers, in their case efficiency and complexity of the method, as well as their small cache size, needs to be considered, see Section \ref{sec:beyond}.}
\nsdionly{%%%%%%%%%%%%%%%%%%
Unlike the phone book, the trigger in \DNSUD{} is initiated by the authoritative server rather than the client, i.e., some kind of a pull method initiated by a push.
}%%%%%%%%%%%%%%%%%%

Related work and alternative methods are presented in Section \ref{sec:background}. Detailed description of the \DNSUD{} service is provided in Section \ref{sec:solution}.
In Section \ref{sec:increase-ttl} we describe the primary implication of increasing TTL values and how we preserve the backward compatibility of \DNSUD{}. \ariel{In section \ref{sec:analysis}, we analyze the relevancy and feasibility of the method, and discuss about its possible implications in Section \ref{sec:implications}.}
In Section \ref{sec:extension} an extension is presented to provide fast recovery when an authoritative server is unavailable.
In Section \ref{sec:beyond} we expand our method to apply also to the clients -- resolvers communication, that is, updating stale records in browsers and other client applications before the corresponding TTL has expired. Finally, conclusions are given in Section \ref{sec:conclusion}.

\ignore{Our analysis indicates that more than $80\%$ of the $50$ most popular domains and the $450-500$ most popular, change their IP address less than once a month, and more than $50\%$ less than once a year. Domain names with short TTL values (less than $10$ minutes) benefit from \DNSUD, by using much larger TTL values and reducing their DNS traffic and the average latencies experienced by clients. Also, \DNSUD{} could ensure a constant and quick recovery from IP address changing for domain names with large TTL values.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cwc"
%%% End:

==> single.tex <==
\def\tp{\!+\!}
\def\tm{\!-\!}

\section{\CR and \CW In Wheel Systems}
\label{sec:rw}

In this section we study the basic tasks of $\CW$ and $\CR$ in the
general wheel system.
We use the subscript $i$ to denote the originating processing node: in
$\CW_i$, an $s$-bits file stored in node $i$ needs to be written to $v_c$,
and in $\CR_i$, an $s$-bits file stored in the $v_c$ needs to be
copied to $i$.
We start with an algorithm for $\CW_i$ in
\sectionref{ssec:write_one_sided}, present a lower bound in
\sectionref{single-lb}, and in \sectionref{ssec:CR} argue
that the same analysis holds for \CR as well.


\subsection{\CW: Upper Bound}
\label{ssec:write_one_sided}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%	
For ease of presentation we consider the ``one sided'' case in which
node $i$ does not use one of its incident ring links.  As we shall
see, this limitation does not increase the time complexity by more
than a constant factor. Hence we consider the case in which node $i$
cannot send messages on its counterclockwise link.  \ignore{
	\begin{lemma}\label{lem-oneway-ub}
		Let $T_\ell(s)$ and $T_r(s)$ denote the minimal number of rounds
		required to write an $s$-bits file to $v_c$ without sending any
		messages on link $({i},{i\tp1})$ ($({i\tm1},{i})$, resp.).  
		Then there exists an algorithm that writes an $s$-bits
		file to $v_c$ while sending messages on 
		both $({i},{i\tp1})$ and $({i\tm1},{i})$ in at most $O(\min(T_\ell(s)),T_r(s)))$ rounds.
	\end{lemma}
}
\ignore{%%%%%%%%%
	%In light of the simplification presented in \lemmaref{lem-oneway-ub},
	Henceforth, we consider the \emph{one-sided} $\CW_i$ task, in which 
	% \begin{definition}
	%   The $\uploadproblem(i, s)$: The system has the wheel topology, as
	%described in \defref{def-wheel}.  % A given node $i$ stores a
	%   file (bit-string) of length $s$. The requirement is that the file
	%   will be written to the cloud.
	% \end{definition}
	%In this task, only one of the local link of $i$ may be used to solve the \CW task.
	node $i$ may not send messages on $(i, i\tm1)$: it may use only
	$(i,i+1)$, and its cloud link. Obviously, our analysis applies also to
	the symmetric case where $i$ may not use $(i,i\tp1)$.
}%%%%%%%%%

% \yehuda{Gal, can you please add a high level intuitive explanation of the algorithm here}
We present pseudocode in \algref{alg:cw-hi}.  The intuition behind the
algorithm is to find out how far clock-wise should node $i$ seek help
in uploading the file.  Consider a processing node $l$, $h$ hops
clock-wise from node $i$ with a large bandwidth link to the cloud node
$v_c$: should $i$ try to forward part of its file to $l$ for
transmission to $v_c$?  If $i$ and all the other $h$ nodes on the path to
$l$ have zero bandwidth links to $v_c$ then clearly yes, but if on the
other hand the total bandwidth to the cloud of these nodes is large
enough to send the file to $v_c$ then the answer is no. Since by the
time ($h$ rounds) the data arrives at $l$ it could have been sent
already to $v_c$.  Thus sending parts of the file farther in the
clock-wise direction becomes useless as both the distance from $i$
increases, and the bandwidth to the cloud along the path increases as
well.  In other words, as data is sent farther clock-wise, more
cloud bandwidth becomes available, but more time is required to reach
it. In addition, narrow bandwidth on the local links may limit the
reachability of cloud bandwidth of remote nodes.  Fortunately, in the
wheel topology, we can easily find the sweet spot that balances the
constraints optimally (up to a constant factor).
% interval of processors, which balances the tradeoff
% between the available bandwidth from the interval to the cloud, and
% the distance that needs to traversed to get to that bandwidth (the
% interval length). Due to \lemmaref{lem-oneway-ub}, it is sufficient to
% look at intervals with $i$ as an endpoint (``one-sided'' intervals).
% required to send $s$ bits to all nodes in the interval through the \emph{local} network,
% and the time required to send $s$ bits through the \emph{cloud} network
% when all nodes of the interval are working together.
% we first find for the initiating node $i$
% its \emph{one-sided} interval that 
Given the optimal interval of nodes, we further simplify the algorithm
(paying another constant factor in its time complexity)  
by first sending the entire file along the interval and then 
each node on the interval writes a chunk of the file to the cloud,
where the chunk size of node $j$ is proportional to $j$'s cloud bandwidth, $w(j,v_c)$.

Formally, let us first define intervals on the ring and their parameters.
\begin{definition}\label{def-intervals}
	%Let $G=(V,E,w)$ be an $n$-node wheel graph.
	An \textbf{interval}
	$\interval{i}{i\tp k}\DEF\Set{i,i\tp 1,\ldots,i\tp k}\subseteq V$ in a
	given wheel graph is a path
	of processing nodes on the ring. Given an interval $I=[i,i+k]$,  $|I|=k+1$ is its \textbf{size}, and $k$ is its
	\textbf{length}.  The \textbf{cloud bandwidth} of $I$,
	denoted $\bc(I)$, is the sum of the cloud bandwidth of all nodes in
	$I$: $\bc(I)=\sum_{i\in I}\bc(i)$.  The \textbf{bottleneck
		bandwidth} of $I$, denoted $\blmin(I)$, is the smallest bandwidth
	of a link in the interval:
	$\blmin(I)=\min\Set{w(i,i\tp1)\mid i,i\tp1\in I}$.  If  $|I|=1$, define $\blmin(I) = \infty$.
\end{definition}
%
% The \emph{cloud bandwidth} of an interval $I$, denoted $\bc(I)$, is
% the total bandwidth of cloud edges emanating from $I$. Formally,
% $\bc(I)=\sum_{i\in I}\bc(i)$.\\ 
%We now define, for any processor node $i$, a special interval. The
%definition is constructive and plays a key role in the algorithms
%ahead.
%We further define the following notions for each node $i\in V_L$.
%
\begin{definition}\label{def-Ii}
	Let $i$ be a processing node. We define the following quantities for
	clockwise intervals; counterclockwise intervals are defined
	analogously. 
	\begin{compactitem}
		\item \label{def:kc}
		$\kCR{i}$ is the length
		of the smallest interval starting at $i$, for which the product of
		its size by the total bandwidth to the cloud along the interval
		exceeds $s$,  i.e.,
		$\kCR{i}=\min\Set{k\mid \left(k\tp 1\right) \cdot \bc([i,i\tp k]) \ge
			s}$. $\kCR{i}=n$ if no such integer exists.
		\item \label{def:kl}
		$\kLR{i}$ is the length
		of the smallest clockwise interval starting at node $i$, for which the bandwidth
		of the clockwise-boundary link bandwidth is smaller than the total
		cloud bandwidth of the interval, i.e.,
		$\kLR{i}=\min\Set{k\mid w(i\tp k,i\tp k\tp 1)<\bc(\interval{i}{i\tp k})}$,
		or $n$ if no such integer exists.
		\item $\kR{i}= \min\Set{\kCR{i}, \kLR{i}}$.
		\item $\IR{i} = \interval{i}{i\tp \kR{i}} $. The interval $\IR{i}$ is
		called the (clockwise) \textbf{cloud interval} of node $i$.
		\item $\ZR{i} = |\IR{i}| + \dfrac{s}{\blmin(\IR{i})} +
		\dfrac{s}{\bc(\IR{i})}$. $\ZR{i}$ is the \textbf{timespan} of the
		(clockwise) cloud interval of $i$.
		% \item	
		% 	Define $\bLminR{i} = \min\limits_{i \le j \le i+\kR{i}
		% 	- 1}{\bL{j}{j+1} }$ if $\kR{i} \ne 0$, or
		% 	$\bLminR{i}=\infty$ otherwise.
	\end{compactitem}
\end{definition}
Note that $\kR{i}$ is easily computable. The algorithm for \CW
(\algref{alg:cw-hi}) is specified
using the cloud intervals.
Its complexity is given in the following theorem.
% We now state and prove the upper bound.
% A matching lower bound is shown in \theoremref{theorem:one_sided_LB}.

%Note that \defref{def-Ii} refers to a cloud interval ``to the right'' of
%node $i$; analogous definitions apply to an interval
%$\Set{i \tm k,i \tm k \tp 1,\ldots,i}$ to the left of $i$.
%\subsubsection{Upper Bound}

%We are now ready to state our upper bound.
\begin{theorem}\label{theorem:one_sided_UB}
	\algref{alg:cw-hi} solves the $s$-bits $\CW_i$ problem %from node $i$
	without using link $({i \tm 1}, i)$ in  $O(\ZR{i})$ rounds.
\end{theorem}

\begin{algorithm}[t]%[H]\small
	\caption{$\CW_i$}
	\label{alg:cw-hi}
	\begin{algorithmic}[1]
		\STATE \label{cw-alg-send-local}
		forward $S$ from node $i$ to all nodes in $\IR{i}$
		\FOR{ all $j\in\IR{i}$, in parallel}
		\STATE\label{cw-alg-node-write}{
			node $j$ writes to the cloud the part of $S$ starting at
			$s\cdot\frac{\bC{\interval{i}{j\tm 1}}}{\bC{I_{i}}} $
			and extending for $s\cdot\frac{\bC{j}}{\bC{I_{i}}}$ bits,
			writing $\bC{j}$ bits in every round.}
		\STATE\label{cw-alg-ack}{node $j\ne i$ sends an acknowledgement to $i$
			when done, and halts}
		\ENDFOR    
		\STATE\label{cw-alg-end} node $i$ halts when all acknowledgements are received.
	\end{algorithmic}
\end{algorithm}

% While the naive algorithm, in which node $i$ uses the full capacity of
% its links (the cloud link and the link to ${i+1}$) to send
% information, and so does every other node, until all $s$ bits are
% uploaded to the cloud, is trivially optimal, its complexity analysis
% may be tricky.\\ 
%\theoremref{theorem:one_sided_UB} is proved using \algref{alg:cw-hi}.
\Proof
Clearly, the algorithm writes $S$ to the cloud, i.e., it solves
$\CW_i$. 
For the time analysis, note that Step \ref{cw-alg-send-local} requires
$O\left(|\IR{i}| + {{s}\over{\bLminR{i}}} \right)$ rounds: there are
$s$ bits to send over $|I_i|-1$ hops with bottleneck bandwidth $\phi(I_i)$.
In Step \ref{cw-alg-node-write}, each node $j$ writes
% $s\cdot{\bC{j}\over\bC{I{i}}} $ 
% bits to the cloud while writing
$\bC{j}$ bits in each round (except perhaps the last round), and since
it needs to write 
$s\cdot{\bC{j}\over\bC{I{i}}} $ bits  overall, this step requires
$O\left({s}/{\bC{\IR{i}}} \right)$ rounds for all $j\in\IR{i}$.
Step \ref{cw-alg-ack} requires $|\IR{i}|$ rounds.
Thus, the algorithm terminates in
$O \left({|\IR{i}| + \dfrac{s}{\bLminR{i}} +
	\dfrac{s}{\bC{\IR{i}}}}\right)
= O(\ZR{i})$ rounds. \QED

We have the following immediate consequence.
\begin{theorem}\label{theorem:two_sided_UB}
	Let $Z_i^\ell$ and $Z_i^r$ denote the timespans of the counterclockwise and the clockwise cloud intervals of $i$, respectively. Then $\CW_i$ can be solved in $O(\min(Z_i^\ell,Z_i^r))$ rounds.
	%	There is an algorithm that writes an $s$-bits message originating
	%	from node $i$ to the cloud, that requires at most $O(\ZR{i})$
	%	rounds.
\end{theorem}


\begin{corollary}\label{cor-ub}
	In the uniform wheel topology with cloud bandwidth $\bc$ and local
	link bandwidth $\bl\ge\bc$, \CW terminates in
	$O\left({s\over\bl}+\min(\sqrt{s\over\bc},{\bl\over\bc})\right)$
	rounds. If $\bl<\bc$, the running time is $O(s/\bc)$ rounds.
\end{corollary}
\Proof
If $\bl<\bc$, $\kLR{i}=0$, $\phi(I_i)=\infty$ and the result follows.
Otherwise, by definition we have $\kCR{i}=\sqrt{s/\bc}-1$ and
$\kLR{i}=\bl/\bc-1$, hence $|\IR{i}|=O(\min(\sqrt{s/\bc},\bl/\bc))$. It
follows that $\bc(\IR{i})=O(\min(\sqrt{s/\bc},\bl))$. The result follows by
noting that
$\bLminR{i}=\bl$.
\QED
% \noindent
% For example, for $\bc=\sqrt{s}$ and $\bl\ge s^{3/4}$, the
% running time is $O(s^{1/4})$.

% \boaz{explain here how to extend the algorithm to 2 directions, maybe
%   to \CR}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\CW: Lower Bound}
\label{single-lb}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To prove a lower bound on the running time of an algorithm solving
$\CW_i$ in the wheel topology, we assume that
the $s$-bits string $S$ that node $i$ needs to write is incompressible.
Such a string
exists for any size $s\in\mathbb{N}$ (see, e.g., \cite{LiV:Kolmogorov}).
As a consequence,
\emph{in any execution of a correct algorithm, $s$ bits must cross any cut that
	separates $i$ and the cloud}.
We use this observation in our lower bound arguments.

Similarly to our upper bound strategy, we first prove the lower bound
for ``one-sided'' intervals, and then extend it to the general case.
% Therefore, in the remainder of this section we focus on
% an upload protocol which does not use link $(i\tm 1,i)$.

% We now turn to show that $\Omega(\ZR{i}) = 
% O \left({|\IR{i}| + \dfrac{s}{\bLminR{i}} +
% 	\dfrac{s}{\bC{\IR{i}}}}\right)$ is a lower bound for the
% \CW problem.
% The idea is that the cloud interval
% $\IR{i}$ is an interval that optimizes, up to a constant
% factor, the tradeoff between the time
% required to send $s$ bits through the local network, and the time
% required to write such a message to the cloud.
% Here and in \figref{fig-Z-explanation},
% we give some intuition as for the significance of each term in
% the lower bound:
% \textit{
% \begin{compactitem}
% \item $|\IR{i}|$ is the length of the interval, and at least
%   $|\IR{i}|$ rounds are required to reach all nodes of the interval
%   from $i$.
% \item ${1}\over{\blmin(\IR{i})}$ is the rate of the bottleneck of the
%   interval.  If we were to send only $o(s)$ bits through that
%   bottleneck, then the interval could have been shortened not to
%   include that edge, and we could have still sent $s$ bits using the
%   shortened interval, in the same time up to a constant factor. Thus at
%   least $\Omega(s)$ bits should pass through there, thus requiring
%   $\Omega({{s}\over{\blmin(\IR{i})}})$ rounds.
% %In order to use nodes that are after this bottleneck, at least
% %$\Omega(s)$ bits should pass through there, thus requiring
% %$\Omega({{s}\over{\blmin(\IR{i})}})$ rounds. 
% %Otherwise, these nodes are not necessary and that edge should not be
% %in the interval. 
% \item $\bc(\IR{i})$ is the number of bits that can be sent to the
%   cloud in a single round by the nodes of $\IR{i}$. Thus, at least
%   ${s}\over{\bc(\IR{i})}$ rounds are required to upload an $s$-bits
%   message.
% \end{compactitem}
% }

\begin{theorem}
	\label{theorem:one_sided_LB}
	Any algorithm for $\CW_i$
	which does not use link $({i\tm 1}, i)$ requires $\Omega(\ZR{i})$ rounds.
\end{theorem}
\Proof
We show that each term
of $\ZR{i}$ is a lower bound on the running time of any algorithm
solving $\CW_i$. The theorem follows from \lemmaref{lemma:interval_length}, \lemmaref{lemma:interval_BN} and \lemmaref{lemma-phi}.
\QED

Similarly to \corollaryref{cor-ub}, we have the following corollary
for the uniform wheel.
\begin{corollary}\label{cor-lb}
	In the uniform wheel topology with cloud bandwidth $\bc$ and local
	link bandwidth $\bl$, any algorithm for \CW requires at least
	$\Omega\left({s\over\bl}+\min(\sqrt{s\over\bc},{\bl\over\bc})\right)$
	rounds if $\bl\ge\bc$, and $\Omega({s\over\bc})$ otherwise.
\end{corollary}
%
%
\ignore{
	\begin{figure}[t]
		\centering
		\scalebox{.7}{
			\begin{tikzpicture}
				\node[draw, circle, fill=yellow!90!black, minimum size=1cm] at (0,0) (mid) {$i$};
				\node[draw, circle, inner color=white, minimum size=1cm] at (-2,0) (l) {$i-1$};
				\node[draw, circle, inner color=white, minimum size=1cm] at (2,0) (r) {$i+1$};
				\node [cloud, draw,cloud puffs=17,cloud puff arc=120, aspect=4.5, inner ysep=1em]
				at 	(0, 2.5)
				{\emph{$v_c$}};
				\draw [-] (mid) -- (l)
				node [above,text width=3cm,text centered,midway] {$0$};
				\draw [-] (mid) -- (r)
				node [above,text width=3cm,text centered,midway] {$0$};
				\draw [->] (mid) -- (0, 1.5)
				node [right,text width=0cm,text centered,midway] {$\bc(i)$};
				\draw [->] (r) -- (2, 1.5)
				node [right,text width=0cm,text centered,midway] {$0$};
				\draw [->] (l) -- (-2, 1.5)
				node [right,text width=0cm,text centered,midway] {$0$};
			\end{tikzpicture}
			\hspace{8mm}
			\begin{tikzpicture}
				\node[draw, circle, fill=yellow!90!black, minimum size=1cm] at (0,0) (mid) {$i$};
				\node[draw, circle, inner color=white, minimum size=1cm] at (-2,0) (l) {$i-1$};
				\node[draw, circle, inner color=white, minimum size=1cm] at (2,0) (r) {$i+1$};
				\node [cloud, draw,cloud puffs=17,cloud puff arc=120, aspect=4.5, inner ysep=1em]
				at 	(0, 2.5)
				{\emph{$v_c$}};
				\draw [-] (mid) -- (l)
				node [above,text width=3cm,text centered,midway] {$0$};
				\draw [-] (mid) -- (r)
				node [above,text width=3cm,text centered,midway] {$w$};
				\draw [->] (mid) -- (0, 1.5)
				node [right,text width=0cm,text centered,midway] {$0$};
				\draw [->] (r) -- (2, 1.5)
				node [right,text width=0cm,text centered,midway] {$\infty$};
				\draw [->] (l) -- (-2, 1.5)
				node [right,text width=0cm,text centered,midway] {$0$};
			\end{tikzpicture}
			\hspace{8mm}
			\begin{tikzpicture}
				\node[draw, circle, fill=yellow!90!black, minimum size=1cm] at (0,0) (mid) {$i$};
				\node[draw, circle, inner color=white, minimum size=1cm] at (-2,0) (l) {$i-1$};
				\node[draw, circle, inner color=white, minimum size=1cm] at (3,0) (r) {};
				\node[draw, circle, inner color=white, minimum size=1cm] at (5,0) (rfar) {$i+k$};
				\node at ($(mid)!.5!(r)$) (dots) {\ldots};
				
				\node [cloud, draw,cloud puffs=23,cloud puff arc=120, aspect=7, inner ysep=1em]
				at 	(1.6, 2.5)
				{\emph{$v_c$}};
				
				\draw [-] (mid) -- (l)
				node [above,text width=3cm,text centered,midway] {$0$};
				\draw [-] (mid) -- (dots)
				node [above,text width=3cm,text centered,midway] {$\infty$};
				\draw [-] (r) -- (dots)
				node [above,text width=3cm,text centered,midway] {$\infty$};
				\draw [-] (r) -- (rfar)
				node [above,text width=3cm,text centered,midway] {$\infty$};
				\draw [->] (mid) -- (0, 1.45)
				node [right,text width=0cm,text centered,midway] {$0$};
				\draw [->] (r) -- (3, 1.45)
				node [right,text width=0cm,text centered,midway] {$0$};
				\draw [->] (l) -- (-2, 1.45)
				node [right,text width=0cm,text centered,midway] {$0$};
				\draw [->] (rfar) -- (5, 1.45)
				node [right,text width=0cm,text centered,midway] {$\infty$};
			\end{tikzpicture}
		}
		\caption{ \em
			The lower bound at a glance. Labels near edges indicate
			their bandwidth.
			Left: $\IR{i}=\Set{i}$, and $Z_i\ge s/\bc(i)$.
			Middle: $\IR{i}=\Set{i,i\tp1}$, $\phi(\IR{i})=w$, so $Z_i\ge s/w$.
			Right: $\IR{i}=\Set{i,\ldots,i+k}$, so $Z_i\ge k$.
		}
		\label{fig-Z-explanation}
	\end{figure}
}

\begin{lemma}
	\label{lemma:interval_length}
	Any algorithm for $\CW_i$
	that does not use edge $({i\tm 1}, i)$ requires 
	$\Omega \left( |\IR{i}|\right) = \Omega \left( \kR{i}\right)$
	rounds.
\end{lemma}
\Proof Let $A$ be an algorithm for $\CW_i$
that does not use link $({i\tm 1}, i)$ and runs in $t_A$ rounds.
If $t_A \ge n$ then $t_A \ge \kR{i}$ and we are done. Otherwise,
we count the number of bits of $S$ that can get to the cloud in $t_A$
rounds. %\yehuda{by when?}.
% Once a bit
% gets to the cloud, we do not count it again if some other node reads
% it and writes it again. 
% We also assume that all bits of the message
% are written to the cloud as they are, without any manipulation. This
% assumption is justified, as we can assume that the input can't be
% compressed as there are $2^s$ inputs that are distributed uniformly.
%
Since $S$ is initially stored in $i$, and since link $({i\tm 1},
i)$ is not used, 
in round $t$  only the nodes in
$\interval{i}{i\tp t\tm1}$ can write to the cloud
parts of $S$.
It follows that in a given round $t$,
at most $\bc([i,i\tp t\tm1])$ bits of
information are sent to the cloud and therefore, overall $A$
writes to the cloud at most
$\sum_{t=1}^{t_A}\bc([i,i\tp t\tm1]) \le t_A\cdot\bc([i,i\tp t_A\tm1])$
bits. Hence, by assumption that  $A$ solves $\CW_i$,
we must have $t_A\cdot\bc([i,i\tp t_A\tm1]) \ge s$. Since by definition,
$\kCR{i}$ is the minimal 
integer%
\footnote{
	$\kCR{i}$ may be $n$ if no such integer exists, but $t_A$ is an integer
	that satisfies the $\kCR{i}$ formula so this is not the case.
}
$\ell$ such that
$(\ell \tp 1)\sum_{j=i}^{i+\ell} \bC{j} \ge s$, we get that
$t_A \tm 1 \ge \kCR{i} \ge \kR{i}$ and the lemma follows. \QED


\begin{lemma}
	\label{lemma:interval_BN}
	Any algorithm for $\CW_i$
	which does not use edge $({i\tm 1}, i)$ requires 
	$\Omega({s}/{\blmin(\IR{i})})$ rounds.
\end{lemma}
\Proof
If $\kR{i}=0$, $\blmin(\IR{i})=\infty$ and the claim is trivial.
Otherwise, let $(j,j\tp 1)\in E$ be any link in
$\IR{i}$ with $\bL{j}{j\tp 1} = \bLminR{i}$.
Note that $j-i<\kR{i}$ because $j+1\in I_i$.
% $r = \argmin\Set{\bL{i\tp j}{i\tp j\tp 1}
%   \mid 0 \le j \le \kR{i}\!\! - \!\!1}$ (ties broken arbitrarily),
% % $r = \argmin\Set{\bL{i\!\!+\!\!j}{i\!\!+\!\!j\!\!+\!\!1}
% %   \mid 0 \le j \le \kR{i}\!\! - \!\!1}$.
% % the link $(i\tp r, i\tp r\tp 1)$ has the least bandwidth in $\IR{i}$,
% % meaning
% which implies that $\bL{i\tp r}{i\tp r\tp 1} = \bLminR{i}$.
%
Consider the total bandwidth of links emanating from the interval
$I' \DEF \interval{i}{j} $. Since we assume that
the link $(i\tm1,i)$ is not used, the number of bits that can leave
$I'$  in $t$ rounds is at most
$t\cdot\left(\bc(I')+ \bL{j}{j\tp 1}\right)$. 
Notice that % $s$ bits of the file originate at node $i$ and are written
% to the cloud, and thus
at least $s$ bits have to leave $I'$.

Observe that $\bc(I') \le \bL{j}{j\tp 1}$, because otherwise we would have
$\kLR{i}=j-i$, contradicting the fact that $k(i)>j-i$.
Therefore, any
algorithm $A$ that solves $\CW_i$ in $t_A$ rounds satisfies
$$
s~\le~t_A\cdot\left(\bc(I') + \bL{j}{j\tp 1} \right)
~\le~ 2t_A\cdot \bL{j}{j\tp 1}
~=~ 2t_A\cdot \bLminR{i} ~,
$$
and the lemma follows. \QED

\begin{lemma}\label{lemma-phi}
	Any algorithm for $\CW_i$
	which does not use edge $({i\tm 1}, i)$ requires 
	$\Omega \left({s}/{\bC{\IR{i}}} \right)$ rounds.
\end{lemma}

\Proof Let $A$ be any algorithm that solves $\CW_i$ in $t_A$ rounds.
Recall that $\kR{i} = \min(\kCR{i}, \kLR{i})$.  If $\kR{i}=n$ then
$\IR{i}$ contains all processor nodes $V_p$, and the claim is obvious, as no more
than $\bC{V_p}$ bits can be written to the cloud in a single round.
Otherwise, we consider the two cases: If $\kR{i} = \kCR{i}$, then
$\kR{i} \ge {s}/{\bC{\IR{i}}} - 1$ by definition, and we are done
since $t_A = \Omega(\kR{i})$ by \lemmaref{lemma:interval_length}.
Otherwise, $\kR{i} = \kLR{i}$. Let us denote $w_R=\bL{i\tp
	\kR{i}}{i\tp \kR{i}\tp1}$. In this case we have
$w_R < \bc(\IR{i})$.  We count how many
bits can leave $\IR{i}$.  Similarly to \lemmaref{lemma:interval_BN},
in a single round, at most $\bC{\IR{i}}$ bits can leave through the
cloud links, and at most $w_R$ bits can leave through
the local links. Since $A$ solves $\CW_i$, we must have
$
s
~\le~t_A\cdot\left(\bC{\IR{i}} +w_R\right)
~\le~ 2t_A \cdot \bC{\IR{i}} ~,$
and hence $t_A = \Omega\left({s}/{\bC{\IR{i}}} \right)$.
\QED




% \subsection{Using Links From Both Directions}
% \label{ssec:write_two_sided}
Given \theoremref{theorem:one_sided_LB} and its corresponding lower
bound for counterclockwise intervals, we can prove the lower bound for
two-sided intervals, under some reasonable assumptions.
%
%Recall that 
%Without loss of generality,
We consider algorithms that
do not manipulate bits, i.e., the only representation of a bit string
(and substrings) is by explicit listing of its content, where the
length is proportional to the number of bits.
We also assume that the algorithms are oblivious to contents: the algorithm execution is independent of the actual bit values in the file, its operation depends only on the network parameters and $s$, the number of bits to be transferred. 
% we only consider algorithms that operate in the same manner for every
% input size $s$, i.e., each node sends and receives the same amount
% of bits through its incident links in every round,
% regardless of the actual content of the input message.

\begin{lemma}\label{lem-oneway-lb}
	Let $Z_\ell$ denote the minimal number of rounds required by an
	algorithm for $\CW_i$ which does not use link
	$({i},{i\tp 1})$, and similarly let $Z_r$ the minimal number of
	rounds for an algorithm which does not use $({i\tm 1},{i})$.  Then
	any oblivious algorithm for $\CW_i$ (which uses all links) requires
	$\Omega(\min(Z_\ell,Z_r))$ rounds.
\end{lemma}

\Sketch Let $A$ be an algorithm by which node $i$ writes an $s$-bits file to the cloud 
in $t_A$ rounds. % $A$ may use nodes on both sides of $i$ to
% write its file.
We make a few assumptions on $A$ and show how to relax them without
affecting $A$'s running time.
%We start with a few simplifying assumptions on $A$,
%and prove that $A$ can be adjusted to allow these assumptions,
%while only improving on the its runtime.

%	\emph{$A$ is oblivious to the content of the message
%		(i.e the value of the bits).}
%	This assumption is legitimized by the aforementioned assumption that the algorithm
%	does not manipulate the message, and the existence of an incompressible input string.
%	
First, we assume that no message is sent from either node $i \tp 1$ or
$i \tm 1$ to node $i$.
We assume that node $i$ is the only node that has information (the $s$-bits file)
prior to the execution of $A$,
and also that $A$ and all bandwidths in $G$ are known to all nodes.
Hence, node $i$ can locally simulate the execution of $A$,
and calculate in advance all messages that it receives through links
$(i, i\tm 1)$ and $(i \tp 1, i)$. Therefore $A$ can operate in the exact same manner,
without sending information through these links to node $i$.

Next, we assume that during the run of $A$, no node reads from $v_c$.
Since we assume that message contents is not manipulated, and that $A$
is oblivious to the content of the file, for any node $j$ that reads a bit string
from the cloud there are two options for the content it reads:
\begin{compactitem}
	\item Part of the file of node $i$. In this case, the destination of these bits
	is eventually the cloud, and thus the node(s) that wrote these bits to the cloud
	could have written them directly to their destination, and the read operation
	is redundant.
	\item Information that was sent from other node(s),
	which is not part of the file of node $i$.
	In that case, since $A$ is oblivious to the content of
	the file, node $j$ could have simulated locally the run of $A$ on some
	arbitrary input, and discover this message by itself without reading it
	from the cloud.
\end{compactitem}

In light of these simplifying assumptions on $A$,
let $s_r$ be the number of bits that were sent to
$v_c$ from nodes $\interval{i\tp 1}{i\tp t_A}$,
let $s_\ell$ be the number of bits that were sent to
$v_c$ from nodes $\interval{i\tm t_A}{i\tm 1}$,
and let $s'$ be the number of bits that were sent to
$v_c$ from node $i$.
Let $s'_r=s_r + s'$, $s'_\ell=s_\ell + s'$.

$A$ sends $s$ bits to the cloud, and thus we get that
$s \le s'+s_r+s_\ell \le s'_r + s'_\ell$,
from which we get that either $s'_r \ge s/2$ or $s'_\ell \ge s/2$.
Assume \WLOG the former.
By the assumptions on $A$, %one can see that 
the $s'_r$
bits sent by $\interval{i}{i+t_A}$ are independent of the operations
performed by nodes $\interval{i\tm t_A}{i\tm 1}$.

We can now construct an algorithm $A'$ that sends $s$ bits of
information originating in node $i$ to the cloud, without using the
link $(i\tm 1, i)$:
We run $A$, without sending any information through edge $({i\tm 1}, i)$,
and by that send $s'_r$ bits of the file to the cloud.
Once $A$ finishes, we run $A$ again in the same manner, now sending
the remaining $s-s'_r$ bits.
$A'$ requires $2t_A$ rounds, and by the definition of $Z_r$ we get
that $2t \in \Omega(Z_r)$. \QED



\ignore{
	\begin{definition}\label{def-Ii-2-sided}
		Let $\IR{i}^r$ and $\IR{i}^\ell$ be the intervals received in \defref{def-Ii}
		for the cases that do not use
		edge $(i \tm 1, i)$, and do not use edge $(i, i\tp 1)$, respectively. Let
		$\ZR{i}^r$ and $\ZR{i}^\ell$ be the lower bounds that were
		defined in \defref{def-Ii}
		%received from \theoremref{theorem:one_sided_LB}
		for these intervals, respectively.
		
		We define the (\emph{not one-sided}) cloud interval $\IR{i}$ and timespan $\ZR{i}$
		of node $i$
		to be $\IR{i}^r$ and $\ZR{i}^r$
		respectively, if $\ZR{i}^r < \ZR{i}^\ell$. Otherwise, we define
		$\IR{i}$ and $\ZR{i}$ to be $\IR{i}^\ell$ and $\ZR{i}^\ell$
		respectively.
	\end{definition}
}

Combining %\lemmaref{lem-oneway-ub} with \theoremref{theorem:one_sided_UB}
%and 
\lemmaref{lem-oneway-lb} with \theoremref{theorem:one_sided_LB},
we obtain the following results.


\begin{theorem} \label{theorem:two_sided_LB} 
	Let $Z_i^\ell$ and $Z_i^r$ denote the timespans of the counterclockwise and the clockwise cloud intervals of $i$, respectively. Then any oblivious algorithm
	for $\CW_i$ requires $\Omega(\min(Z_i^\ell,Z_i^r))$ rounds.
	% Any algorithm that
	%  writes an $s$-bits message originating from node $i$ to the cloud,
	%  requires at least $\Omega(\ZR{i})$ rounds.
\end{theorem}


\subsection{\CR:  Upper and Lower Bounds}
\label{ssec:CR}
%%%%%%%%%%%%%%%%%%%%%
We now consider $\CR_i$% , under the assumption that link bandwidth is symmetric, the same in both directions
. 
We claim that it is essentially the same as
$\CW_i$---reversed:
% Note that since we require that an invocation of $\CW_i$
% requires a ``done'' response at $i$, read and
% write are essentially the same task, reversed: 
Given an
execution of $\CW_i$, consider running it  backwards. The
acknowledgements sent in $\CW_i$, run backwards, turn into ``start''
message sent by $i$,
and writes to the cloud by nodes of $\IR{i}$ in $\CW_i$ turn into reads from
the cloud in $\CR_i$. Finally, instead for $i$ sending $S$ to $\IR{i}$, in
$\CW_i$, in $\CR_i$ we have that the nodes of $\IR{i}$ send pieces of
$S$ to $i$, which assembles them to the complete $S$ and
halts. Pseudocode is presented in
\algref{alg:cr-hi}. We summarize as follows.


\begin{algorithm}[t]%[H]\small
	\caption{$\CR_i$}
	\label{alg:cr-hi}
	\begin{algorithmic}[1]
		\STATE{
			Node $i$ sends a ``start'' message to all nodes in $\IR{i}$,
			telling them when to start reading from the cloud.}
		\label{cr-alg-start}
		\FOR{ all $j\in\IR{i}$  in parallel}
		\STATE{
			Node $j$ reads from the cloud
			the part of the message starting at
			$s\cdot{\bc([i,j])\over\bC{I{i}}}$ and extending for
			$s\cdot{\bc(j)\over\bC{I{i}}}$ bits,
			by reading $\bC{j}$ bits in every round.
		}
		\label{cr-alg-node-read}
		\STATE {
			Node $j$ sends the part of $S$ it read through the local
			links to $i$.
		}
		\label{cr-alg-send-local}
		\ENDFOR    
		\STATE{ When all $s$ bits of the message are
			received at node $i$, \CR is done.
		}
		\label{cr-alg-end}
	\end{algorithmic}
\end{algorithm}

\begin{theorem}\label{theorem:CR_UB}
	Let $Z_i^\ell$ and $Z_i^r$ denote the timespans of the counterclockwise and the clockwise cloud intervals of $i$, respectively. Then 
	$\CR_i$ can be executed in  $O(\min(Z_i^\ell,Z_i^r))$ rounds.
\end{theorem}

% \Proof Taking the algorithm received in \theoremref{theorem:two_sided_UB},
% and reversing it as mentioned will result with an algorithm that reads $s$ bits from the cloud and sends them to node $i$, as required.

% To be more explicit, the reversed algorithm for \algref{alg:cw-hi}
% is described in high level in \algref{alg:cr-hi}.
% Note that this algorithm is described for the \emph{right} cloud interval of $i$,
% but the claim can be extended to both directions using a
% similar lemma to \lemmaref{lem-oneway-ub}.

% Similarly to the upper bound of \CW, one can see that
% step \ref{cr-alg-start} requires $O(|\IR{i}|)$ rounds,
% step \ref{cr-alg-node-read} requires $O\left({s}/{\bC{\IR{i}}} \right)$ rounds,
% and step \ref{cr-alg-send-local} requires
% $O\left(|\IR{i}| + {{s}\over{\bLminR{i}}} \right)$ rounds,
% which sums up to $O(\ZR{i})$ rounds in total.

Using arguments as for $\CW_i$, we also have the following lower bound.

\begin{theorem} \label{theorem:CR_LB}
	Let $Z_i^\ell$ and $Z_i^r$ denote the timespans of the counterclockwise and the clockwise cloud intervals of $i$, respectively. Then any oblivious algorithm
	for $\CR_i$ requires $\Omega(\min(Z_i^\ell,Z_i^r))$ rounds.
\end{theorem}

% \Proof Any such algorithm, can be ``reversed'' as described above,
% to get an algorithm that contradicts \theoremref{theorem:two_sided_LB}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cwc"
%%% End:




==> solution-details.tex <==
\section{Solution-Details}
\label{sec:solution-details}

\ignore{%%%
\paragraph{Background}
}%%%

\subsection{Packet Structure}
%\label{sec:}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Explain the Packet structure between the Resolvers and the AS
Details of the selected fields to a backward compatible solution
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{DNSUD - Update Process}
%\label{sec:}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DNSUD's database stores list of DNS records that are outdated .

\begin{figure}[h]
    \centering
    \includegraphics[width=8cm]{db}
    \caption{DNSUD database structure}
    \label{fig:dnsud}
\end{figure}

Figure 7 shows us the structure of a record inside the database: \newline
* Timestamp - Time of entry the domain entered the database. \newline 
* Including Subdomains - Indicates update that applys to subdomains. \newline 
* Domain - The domain that is outdated. \newline
* Value - IP update for the record (for "Save Updates Extension"). \newline
* Sign - Sign for the record (required for "Save Updates Extension"). \newline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

UpDNS request includes the last timestamp for the resolver. Then, DNSUD finds all updated domains and sends the relevant records back to the resolver. As a result, it is possible to keep the database sorted by timestamp. \newline
For a resolver, find the domains from its local cache that need updating is quite simple.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "cwc"
%%% End:


==> ttls.tex <==
\section{Increasing the TTL values}
\label{sec:increase-ttl}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ignore{%%%%%%%%%%%%%%%%%%%%%
\DNSUD{} enables Internet services to significantly increase the TTL values associated with their domain names, on top of the benefits described in Section \ref{sec:solution}.
TTL increasing is possible due to the short period from the time an authoritative sends an InsertDomain request to the \UpdateDB{} until any client gets the updated record information in response to its DNS request (around one minute), see Section \ref{sec:recovery-time}.}%%%%%%%%%%

The motivation to use short TTL values in the current DNS system stems from the need to keep the recovery time (undo time) short.  Since \DNSUD{} decouples the dependency of the recovery time on the TTL value, and provides a fast recovery time, there is no more a reason not to use much larger TTL values. Therefore, we add a second TTL value, called \DNSUD-TTL, to the records of domains that use \DNSUD.
\ignore{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DNSUD{} enables Internet services to significantly increase the TTL values associated with their domain names, on top of the benefits described in Section \ref{sec:solution} due to the short recovery time (around one minute) achieved by \DNSUD, see Section \ref{sec:recovery-time}.}%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Backward compatibility of the \DNSUD{}}
\label{sec:new-ttl}
The only conflict between the \DNSUD{} and the standard DNS system is in the new TTL value that the resolver may use for domain names in its cache.
Notice however that resolvers and authoritative servers using \DNSUD{} still need to maintain also the traditional shorter TTL for the communication with their clients. In addition, resolvers should send the same DNS queries as before to communicate with authoritative servers that do not use the method. 
\ignore{%%%%%%%%%%%%%%%%%%%%
Thus, we need to find a way for an authoritative server to send a different TTL value for the resolvers that use the \DNSUD{} method without influencing resolvers and clients that still do not use the service.
To enable backward compatibility with the current DNS system, we should describe how some of the resolvers can use the \DNSUD{} service while the others operate as usual.} %%%%%%%%%%%%%%%%%%

To add the \DNSUD-TTL value while maintaining the traditional TTL value in the authoritative responses, in a backward compatible way, the optional ADDITIONAL section \cite{rfc1035} is used for the \DNSUD-TTL value.
Inside the ADDITIONAL section, a new record with the new TTL value - the "\DNSUD-TTL" is added. Its maximal possible value is $2,147,483,647$ seconds \cite{rfc1034}, which is more than $68$ years.

An example of a possible DNS answer sent by an authoritative server for Google is: \\
\textbf{ANSWER section:} \newline
google.com {} {} {} {} $600$ {} {} {} {} IN {} {} {} {} A {} {} {} {} $172.253.115.100$ \newline
\textbf{ADDITIONAL section:} \newline
\DNSUD.google.com $2,147,483,647$ {} IN A {} $172.253.115.100$ \\

Clients and resolvers that are not yet using the \DNSUD{} ignore the ADDITIONAL section and use the traditional TTL from the ANSWER section (e.g., $600$ for google.com), while resolvers that use \DNSUD{} take the "\DNSUD-TTL" for the domain from the ADDITIONAL section (e.g., $2147483647$ for google.com). Internet service owners add the "\DNSUD-TTL" in their DNS zone file \cite{zone-file}. 
Thus, an authoritative server that uses the \DNSUD{} can communicate with resolvers that do or do not, implement the method. Alternative implementations may be considered by the DNS community.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

